Graph Relations and Constrained Homomorphism Partial Orders

We consider constrained variants of graph homomorphisms such as embeddings, monomorphisms, full homomorphisms, surjective homomorpshims, and locally constrained homomorphisms. We also introduce a new variation on this theme which derives from relations between graphs and is related to multihomomorphisms. This gives a generalization of surjective homomorphisms and naturally leads to notions of R-retractions, R-cores, and R-cocores of graphs. Both R-cores and R-cocores of graphs are unique up to isomorphism and can be computed in polynomial time. The theory of the graph homomorphism order is well developed, and from it we consider analogous notions defined for orders induced by constrained homomorphisms. We identify corresponding cores, prove or disprove universality, characterize gaps and dualities. We give a new and significantly easier proof of the universality of the homomorphism order by showing that even the class of oriented cycles is universal. We provide a systematic approach to simplify the proofs of several earlier results in this area. We explore in greater detail locally injective homomorphisms on connected graphs, characterize gaps and show universality. We also prove that for every $d\geq 3$ the homomorphism order on the class of line graphs of graphs with maximum degree $d$ is universal.

==> Chapter2/chapter2_beforeAndrew.tex <==
\chapter[Homomorphisms and Constrained Homomorphisms]{\fontsize{35}{10}\selectfont Homo\-morphisms and\\ Constrained Homomorphisms}
\label{ch:homo}
\ifpdf
    \graphicspath{{Chapter2/Chapter2Figs/PNG/}{Chapter2/Chapter2Figs/PDF/}{Chapter2/Chapter2Figs/}}
\else
    \graphicspath{{Chapter2/Chapter2Figs/EPS/}{Chapter2/Chapter2Figs/}}
\fi

%\markboth{\MakeUppercase{\thechapter. Constrained Graph homomorphism }}

%Several variants of graph homomorphism also have been studied.
 

%For the sake of completeness, we also give a brief summary of computational complexity of problems related to constrained homomorphism.

%\section{Bijective, injective, surjective}

%\markboth{\MakeUppercase{\thechapter. Constrained Graph homomorphism }}


The topic of this chapter are graph homomorphisms and several common variants of graph homomorphisms. The theory of graph homomorphisms, which can be seen as the foundation of this thesis, has developed from a well know graph-theoretical problem `graph colouring'. 
Meanwhile, many graph-theoretical problems can be generalized to the notions of special homomorphisms, which we call \emph{constrained homomorphisms}\index{constrained homomorphisms}.
This chapter can be divided into four parts. In the first 3 sections we overview the existing structural results: We first recall the basic properties of ordinary graph homomorphisms in Section~\ref{sec:homo}. Later, in Section~\ref{sec:glo} we review several types of \emph{globally constrained homomorphisms}\index{globally constrained homomorphisms} such as monomorphism, embedding, surjective homomorphism, full homomorphism and compaction. In Section~\ref{sec:loc}
we discuss three kinds of \emph{locally constrained homomorphisms}\index{locally constrained homomorphisms}: locally injective, locally bijective and locally surjective. In the last section we introduce a new notion we call `relation' which can be viewed as a generalization of surjective homomorphism. We developed the basic properties of `relation', as a preparation of a deeper investigation in Chapter~\ref{ch:relation}.



\section{Graph homomorphisms} \label{sec:homo}



Graph colouring is one of the most well-known problems in the field of graph theory. As an example, the four colour conjecture, which is postulated by Francis Guthrie while trying to colour a map of the counties of England, stating that four colours were sufficient to colour the map so that no regions sharing a common border receive the same colour. In terms of graph theory: all planar graphs can be coloured by 4 colours. As a generalization of graph colouring,  the study of graph homomorphisms dates from 1960s. It was pioneered by G.\ Sabidussi~\cite{Sabidussi1961}, and by Z.\ Hedrl\' in and A.\ Pultr~\cite{Hedrlin1964}, and rapidly developed by P.\ Hell and J.\ Ne\v{s}et\v{r}il~\cite{Hell2004}. In this section we give a brief summary of the main concepts and results in this area. For more details please refer to the recent monograph~\cite{Hell2004}.

\begin{defi}
Let $G=(V_G,E_G)$ and $H=(V_H,E_H)$ be two directed graphs,
a \emph{homomorphism}\index{homomorphism} of $G$ to $H$,
is a mapping $f:V_G\rightarrow V_H$ such that $(f(u),f(v))\in E_H$
whenever $(u,v)\in E_G$. 
\end{defi}

A homomorphism of $G$ to $H$ is also called an \emph{$H$-colouring of G}\index{$H$-colouring}.
If there exists a homomorphism $f:G\rightarrow H$ we write, $G\rightarrow H$\index{$\rightarrow$}, and $G\nrightarrow H$\index{$\nrightarrow$} means there is no such homomorphisms.


Let $f$ be a homomorphism of graph $G=(V_G,E_G)$ to graph $H=(V_H,E_H)$, and $S$ a subset of $V_G$, $M$ a subset of $V_H$,
we define $f(S):=\{v\in V_H\mid \exists x\in S \text{ s.t.\ } f(x)=v\}$ as the \emph{image of $S$}\index{image},
$f^{-1}(M):=\{x\in V_G\mid \exists u\in M \text{ s.t. } f(x)=u\}$ as the \emph{domain of $M$}\index{domain}.
Moreover, the \emph{image of homomorphism $f$}\index{image of a homomorphism}, denoted by $I(f)$\index{$I(f)$}, is defined as the image of $V_G$, and the \emph{domain of $f$}\index{domain of a homomorphism}, denoted by $D(f)$\index{$D(f)$}, is defined as the domain of $V_H$. 
Note that since $f$ is a mapping, the domain of $f$ is always $V_G$.

%\begin{figure}[!ht]
%\centering
%\begin{tabular}{c c m{5cm}} 
%\begin{minipage}{4cm}
%\centering
%\includegraphics[height=4cm]{Frucht.eps}
%\end{minipage}
%&
%\begin{minipage}{2.5cm}
%\centering
%\includegraphics[height=2cm]{K_3.eps}
%\end{minipage}
%&
%\begin{minipage}{4cm}
%\begin{itemize}
 %\item[]
 %$f(1)$ = Red
 %\item[]
 %$f(2)$ = Blue
 %\item[]
 %$f(3)$ = Red
 %\item[]
 %$f(4)$ = Green
 %\item[]
 %$f(5)$ = Blue
 %\item[]
 %$f(6)$ = Green
 %\item[]
 %$f(7)$ = Blue
 %\item[]
 %$f(8)$ = Red
 %\item[]
 %$f(9)$ = Blue
 %\item[]
 %$f(10)$ = Blue
 %\item[]
 %$f(11)$ = Red
%\item[]
 %$f(12)$ = Green
%\end{itemize}
%\end{minipage}\\
%Frucht graph & Graph $K_3$ & An homomorphism from Frucht graph to $K_3$
%\end{tabular}
%\caption{Graph homomorphism.}
%\label{tab:FtoK3}
%\end{figure}


%\noindent
\begin{table}
\centering
\begin{tabular}{|c|c|c|}
    \hline
    Frucht graph & Graph $K_3$ & \begin{tabular}{c}An homomorphism from\\Frucht graph to $K_3$\end{tabular}
    \\[8pt]
    \hline
     \lower1.8cm\hbox{\includegraphics[width=4cm]{Frucht.eps}}
    &
     \lower1cm\hbox{\includegraphics[height=2.5cm]{K_3.eps}} 
    &
    \begin{tabular}{l}
     \\[-6pt]
     $  f(1) = \color{Red}  \text{Red}  $\\
     $  f(2) = \color{Blue} \text{Blue} $\\ 
     $  f(3) = \color{Red}  \text{Red}  $\\ 
     $  f(4) = \color{Green}\text{Green}$\\ 
     $  f(5) = \color{Blue} \text{Blue} $\\ 
     $  f(6) = \color{Green}\text{Green}$\\ 
     $  f(7) = \color{Blue} \text{Blue} $\\ 
     $  f(8) = \color{Red}  \text{Red}  $\\ 
     $  f(9) = \color{Blue} \text{Blue} $\\
     $ f(10) = \color{Blue} \text{Blue} $\\
     $ f(11) = \color{Red}  \text{Red}  $\\
     $ f(12) = \color{Green}\text{Green}$\\[6pt]  
     \end{tabular}
    \\
    \hline
\end{tabular}
\caption{Graph homomorphism.}
   \label{tab:FtoK3} 
   \end{table}


%\begin{table}[t]
 %\centering
%\bgroup
%\def\arraystretch{1.4}
%\begin{tabular}{|c|c|c|} \hline
%\parbox{3cm}{Frucht graph} &
%\parbox{3cm}{Graph $K_3$}&
%\parbox{5cm}{An homomorphism \\from Frucht graph to $K_3$}\\ \hline
%%\begin{tabular}{|c|c|c|}
 %   \hline
 %   Frucht graph & Graph $K_3$ & \begin{tabular}{c}An homomorphism from\\Frucht graph to $K_3$\end{tabular}
  %  \begin{tabular}{|c|c|c|} \hline
%\multirow{12}{*}{\includegraphics[height=4cm]{Frucht.eps}} & \multirow{12}{*}{\includegraphics[height=2.5cm]{K_3.eps}} &  $f(1)$ = Red\\
%&&$f(2)$ = Blue\\ 
%&&$f(3)$ = Red\\ 
%&&$f(4)$ = Green\\ 
%&&$f(5)$ = Blue\\ 
%&&$f(6)$ = Green\\ 
%&&$f(7)$ = Blue\\ 
%&&$f(8)$ = Red\\ 
%&&$f(9)$=Blue\\
%&&$f(10)$=Blue\\
%&&$f(11)$=Red \\
%&&$f(12)$=Green\\ \hline
%\end{tabular}
%\egroup
%\caption{Graph isomorphism.}
%\label{tab:FtoK3}
%\end{table}

\begin{example}
In order to build intuition about the existence of graph homomorphisms, we give some examples :
\begin{enumerate}
 \item If graph $G$ is a subgraph of graph $H$, then the subgraph structure induces a homomorphism from $G$ to $H$
(Figure~\ref{fig:subg}). However, there may have other homomorphisms of $G$ to $H$ which are not induced by subgraph structure. 
 \item There is a homomorphism of Frucht graph to complete graph $K_3$ as in Fig.~\ref{tab:FtoK3}. Because $K_3$ is a subgraph of Frucht graph, there is a homomorphism of $K_3$ to Frucht graph.
 \item $P_2\to K_3$, since $P_2$ is a subgraph of $H_3$. However $K_3\nrightarrow P_2$, that is because the size of $K_3$ is larger than $P_2$, then there are at least two vertices of $K_3$ which must be mapped to the same vertex of $P_2$, this would induce a loop. However $P_2$ is loop-free.
\end{enumerate}
\end{example}


It is an easy fact that the composition of homomorphisms are still homomorphisms. Moreover, homomorphisms are also associative.
Let $f:V_G\rightarrow V_H$ be a homomorphism of $G$ to $H$, if the mapping $f$ is injective, we call it a \emph{injective homomorphism}\index{injective homomorphism}. Homomorphism $f$ naturally induces an edge mapping of $E_G$ to $E_H$, if $f$ and the induced edge mapping are both surjective, we call it is a \emph{surjective homomorphism}\index{surjective homomorphism}.
The following proposition shows that a homomorphism can be decomposed, as a surjective homomorphism and an injective homomorphism.



\begin{pro}[\textbf{Decomposition law}~\cite{Hell2004}] 
Let $G$ and $H$ be any directed graphs. Every homomorphism $f:G\rightarrow H$ can be written as $f=i\circ s$ where $s$ is a surjective homomorphism and $i$ is an injective homomorphism.
\end{pro}

We leave the proof to the section of surjective graph on Page~\pageref{decomp}. 

\begin{pro} \label{pro:colouring}
A homomorphism $f:G\rightarrow K_k$ is precisely a $k$-colouring of graph $G$.
\end{pro}

\begin{proof}
For $1\leq i\leq k$, we colour the vertices of graph $G$ in the set $f^{-1}(i)$ by colour $i$. Clearly for distinct $i$ and $j$, $f^{-1}(i)\cap f^{-1}(j)=\emptyset$. And for any $i$, $f^{-1}(i)$ is an independent set, otherwise there is a loop on vertex $i$ of $K_k$. Hence homomorphism $f$ is a proper $k$-colouring of graph $G$.
\end{proof}

Proposition~\ref{pro:colouring} explains the reason that a homomorphism from $G$ to $H$ is also called $H$-colouring: actually a graph homomorphism can be seen as a generalization of a graph colouring.

\subsection*{Homomorphisms preserve adjacency}
The fact that homomorphisms preserve vertex adjacency has interesting implications, the following propositions are derived from the adjacency preservations.

\begin{pro}
A mapping $f: V_{P_k}\rightarrow V_G$ is a homomorphism of $P_k$ to graph $G$ if and only if the sequence $f(1),f(2),\dots,f(k)$ is
a walk in graph $G$.
\end{pro}

Consequently, we can get the following useful corollary.

\begin{cor}
If $f:G\rightarrow H$ is a homomorphism, then for any two vertices $u,v$ of graph $G$, the distance of $f(u)$ and $f(v)$ in graph $H$ is at most the distance of $u$ and $v$ in $G$.
\end{cor}

\begin{rem}
Even though the existence of homomorphisms is monotone with respect to the distance, it is not monotone with radius and diameter. For example, $P_2\to K_3$ and $P_2\to P_5$, but the diameter as well as radius of $P_2$ is between $K_3$ and $P_5$. In contrast, we will see an analogous structure which is monotone with respect to diameter as well in Corollary~\ref{rad} on Page~\pageref{rad}. 
\end{rem}

Similar to paths, we have the following result of homomorphisms from cycle graphs.

\begin{pro}
A mapping $f: V_{C_k}\rightarrow V_G$ is a homomorphism of $C_k$ to $G$ if and only if the sequence $f(0),f(1),\dots,f(k-1)$ is a closed walk in $G$.
\end{pro}

\begin{cor}
$C_{2k+1}\rightarrow C_{2l+1}$ if and only if $l\leq k$.
\end{cor}




\subsection*{Homomorphism equivalence}
\label{sec:hom-equ}
In the last section, we know that the existence of homomorphisms is monotone with respect to chromatic number, so that if two directed graphs $G$ and $H$ have different chromatic numbers, then $G\to H$ and $H\to G$ do not hold at the same time. Two directed graphs $G$ and $H$ such that each is homomorphic to the other are called \emph{homomorphically equivalent}\index{homomorphically equivalent}, and denoted by $G\sim H$\index{$G\sim H$}. Homomorphic equivalence is indeed an equivalence relation. To see this, let $G$, $H$ and $K$ be directed graphs. Since every directed graph is homomorphically equivalent to itself (self-adjoint); $G\sim H$ implies $H\sim G$ (symmetric); If $G\sim H$ and $H\sim K$, then follows from the fact that homomorphisms are closed for composition, $G\sim K$ (transitive). We immediately gets that the homomorphically equivalent directed graphs have the same chromatic number. In this section we focus on the question of how to characterize homomorphism equivalent directed graphs.


\begin{defi}
A \emph{retraction}\index{retraction} of directed graph $G$ to its subgraph $H$ is a homomorphism
$r:G\rightarrow H$ such that $r(x)=x$ for all $x\in V_H$.
\end{defi}

If there is a retraction of $G$ to $H$, we call $H$ is a \emph{retracted graph}\index{retracted graph} of $G$.
Recall that the a subgraph has a homomorphism to its original graph, so a graph and (any of) its retracted graph are homomorphism equivalent. Figure~\ref{fig:Retr} shows a series of retractions. 
  

\begin{figure}[!ht]
\centering
\begin{minipage}[c]{0.22\textwidth}
  \includegraphics[width=1\textwidth]{dicore1.eps}
\end{minipage}
$\rightarrow$
\begin{minipage}[c]{0.22\textwidth}
 \centering
 \includegraphics[width=1\textwidth]{dicore2.eps}
\end{minipage}
$\rightarrow$
\begin{minipage}[c]{0.22\textwidth}
 \centering
\includegraphics[width=0.8\textwidth]{dicore3.eps}
\end{minipage}
$\rightarrow$
\begin{minipage}[t][][b]{0.15\textwidth}
 \centering
\includegraphics[width=0.8\textwidth]{dicore4.eps}
\end{minipage}
\caption{A series of retractions.}
\label{fig:Retr}
\end{figure}


The most natural idea is to find the smallest directed graph (in the sense of size) in an equivalent class as the representative. 
Firstly, given a graph $G$, we can try to find the smallest subgraph which $G$ has a retraction to. This leads an important concept which was independently discovered and was given different names such as \emph{minimal graphs}\index{minimal graph} and \emph{unretractive graphs}\index{unretractive graph}~\cite{Fellner1982,Hell1992,Nowakowski1979}.

\begin{defi}
A \emph{core of (directed) graph $G$}\index{core of a graph} is the smallest graph (in the sense of size) which $G$ admits a retraction to.
A (directed) graph is a \emph{core}\index{core} if it does not retract to a proper subgraph.
\end{defi}

It is easy to see that every directed graph is homomorphically equivalent to a (up to isomorphism) unique core.
Thus we can denote the core of a given graph $G$ by $G_\text{core}$\index{$G_\text{core}$}.
For example, the core of first three directed graphs in Figure~\ref{fig:Retr} is the fourth directed graph.

Two graphs are homomorphically equivalent if and only of their cores are isomorphic, therefore we can use core to be the
representative in an equivalent class. However, the computational complexity of determining a core is NP-hard. As we know, 3-colouring problem, i.e., testing whether a graph has a homomorphism to triangle $K_3$, is NP-complete. Given a graph $G$, consider $G'$ to be the disjoint union of $G$ and $K_3$. If we can determine the core of $G'$, then it is easy to decide whether $G$ is 3-colourable or not. If the core of $G'$ is $K_3$, then $G$ is 3-colourable, otherwise $G$ is not 3-colourable.

\subsection*{H-colouring problem}
In this section we introduce the main results of the existence of homomorphisms from an algorithmic perspective.

Let $H$ be a fixed directed graph. The \emph{homomorphism problem for $H$}\index{homomorphism problem for $H$} asks whether or not an input
directed graph $G$ admits a homomorphism to $H$. Recall that a homomorphism of $G$ to $H$ is also called an
$H$-colouring of $G$. Thus the homomorphism problem for $H$ is also called the \emph{$H$-colouring problem}\index{$H$-colouring problem},
and denoted by $\COL$\index{$\COL$}.


The $H$-colouring problem can be analogously stated for any general relational system $H$, in this case the problem is also known as \emph{constraint satisfaction problem}\index{constraint satisfaction problem} (or \emph{CSP}\index{CSP}) with a template $H$, and denoted as $\CSP$\index{$\CSP$}~\cite{Hell2004}. Many studies are done regarding to constraint satisfaction problem, there is an introduction book by E. Tsang~\cite{Tsang1993}.

We first consider the $H$-colouring problem for graphs (instead of digraphs). Clearly all graphs which have a loop have core $O$, the graph with one vertex and a loop.
The problem of $O$-colourablity is trivial.

Recall that the usual $k$-colouring problem for simple graphs is polynomial time solvable when $k\leq 2$ and is NP-complete for $k>2$.
Such a classification result implies that we have a \emph{dichotomy}\index{dichotomy} of possibilities ---
each $k$-colouring problem is polynomial time solvable or NP-complete. Analogously, $H$-clouring has also dichotomy of possibilities.

\begin{thm}
 Let $H$ be a graph. If $H$ is bipartite or contains a loop, then the $H$-colouring problem has a polynomial time algorithm.
 Otherwise the $H$-colouring problem is NP-complete.
\end{thm}

This theorem was first proved in~\cite{Hell1990} by Hell and Ne\v{s}et\v{r}il.
There is a new proof by Bulatov~\cite{Bulatov} which follows the same idea but uses an algebraic approach.

The $H$-colouring problem for directed graphs has received much attention, and yet no graph-theoretic classification has been obtained, or conjectured~\cite{Hell2004}. Note that even the following dichotomy conjecture is still open.

\begin{con}
 Let $H$ be a directed graph, the $H$-colouring problem is polynomial time solvable or NP-complete.
\end{con}

There is a nice conjectured dichotomy classification for directed graphs with positive indegree and outdegree in each vertex.
The conjecture is still open though many special cases of the conjecture have been verifies~\cite{Hahn2002}.

\begin{con}[Bang-Jensen, Hell~\cite{Bang1990}]
Suppose $H$ is a connected directed graph in which each vertex has positive indegree and outdegree.
If the core of $H$ is a directed cycle, then $H$-colouring problem is polynomial.
Otherwise it is NP-complete.
\end{con}




\section[Globally constrained homomorphisms]{\fontsize{20}{10}\selectfont Globally constrained homomorphisms}\label{sec:glo}


We consider several types of (globally) constrained homomorphisms.

\begin{enumerate}
\item A homomorphism $f:G\to H$ is {\em a monomorphism}\index{monomorphism}\footnote{The name `monomorphism' is from category theory.}, (also called \emph{injective homomorphism}\index{injective homomorphism}~\cite{Hell2004} or {\em \MonoHomo}\index{\MonoHomo}) if it is injective.
\item A homomorphism $f:G\to H$ is {\em a full homomorphism}\index{full homomorphism}, or {\em \FullHomo}\index{\FullHomo}, if $(f(u),f(v))\in E_H$ implies $(u,v)\in E_G$.
\item A homomorphism $f:G\to H$ is {\em an embedding}\index{embedding}, or {\em \EmbedHomo}\index{\EmbedHomo} if it is both a monomorphism and a full homomorphism.
\item A homomorphism $f:G\to H$ is {\em a vertex surjective homomorphism}\index{vertex surjective homomorphism}, or {\em \VSurHomo}\index{\VSurHomo}, if $f(V_G)=V_H$. A homomorphism $f:G\to H$ is {\em a surjective homomorphism}\index{surjective homomorphism}, or {\em \SurHomo}\index{\SurHomo}, if it is vertex surjective and moreover for every $(u,v)\in E_H$ there is $(u',v')\in E_G$ such that $f(u')=u$ and $f(v')=v$.
\end{enumerate}


%Vertex mapping $f$ induces an edge mapping $f'$ by mapping edge $(x,y)$ of graph $G$ to $f'((x,y))=(f(x),f(y))$, which is an edge of $H$ by definition of %graph homomorphism. A homomorphism $f:G\to H$ is {\em an edge surjective homomorphism}\index{edge surjective homomorphism}
%if the mapping $f'$ is surjective, i.e.\ for every $(u,v)\in E_H$ there is $(x,y)\in E_G$ such that $f(x)=u$ and $f(y)=v$.
%A homomorphism $f:G\to H$ is {\em a surjective homomorphism}\index{surjective homomorphism}, or {\em \SurHomo}\index{\SurHomo}, if it is vertex surjective 5and edge surjective.


\begin{figure}[!ht]
 \centering
 \includegraphics[width=0.55\textwidth]{global.eps}
 \caption{Monomorphism, surjective homomorphism, embedding.}
 \label{fig:glo}
\end{figure}


Figure~\ref{fig:glo} shows a monomorphism ($G_m$ to $H$), a surjective homomorphism ($G_s$ to $H$) and an embedding ($G_e$ to $H$). 


Let $G$ and $H$ be directed graphs, there is a monomorphism from
$G$ to $H$ if and only if $G$ is a subgraph of $H$, there is an embedding from $G$ to $H$ if and only if $G$
is an induced subgraph of $H$. Examples can be found in Section~\ref{subsec:sub} on Page~\pageref{subsec:sub}.

%Note that there is an embedding or a monomorphism from directed graph $G$ to directed $H$ implies that the order of $G$ is no less than the order of $H$.



\subsection*{Surjective homomorphisms} \label{sec:mono}




%the computational complexity of monomorphism problem, also called subgraph isomorphism problem, is NP

\begin{example} 
There are some examples of vertex or edge surjective homomorphisms.
\begin{enumerate}
\item The mapping from Frucht graph to $K_3$ shown in Figure~\ref{tab:FtoK3} is a surjective homomorphism;
\item The homomorphism from $P_3$ (Figure~\ref{fig:iplus})to $K_3$ by mapping $f(x_i)=v_i$ for $i=1,2,3$ is vertex surjective but not edge surjective (because the preimage of edge $(v_2,v_3)$ is empty);
\item The homomorphism from to $P_3$ to $G$ shown in Figure~\ref{fig:iplus} by mapping $f(x_1)=v_2$, $f(x_2)=v_3$ and $f(x_3)=v_2$ is edge surjective bot not vertex surjective (because the preimage of $v_1$ is empty).
\end{enumerate}
\end{example}



%\begin{wrapfigure}{r}{4.5cm}
\begin{figure}[!ht]
 \centering
 \includegraphics[width=0.65\textwidth]{iplusP2.eps}
 \caption{Example of an edge surjective but not vertex surjective homomorphism.}
 \label{fig:iplus}
\end{figure}
%\end{wrapfigure}



Note that a homomorphism that is vertex injective is also edge injective (but not conversely), and, as long as the resulting graph has no isolated vertices, a homomorphism that is edge surjective is also vertex surjective (but not conversely).
In other words, injective homomorphisms are the same as vertex injective homomorphisms, while surjective homomorphisms are, in the absence of isolated vertices, the same as edge surjective homomorphisms~\cite{Hell2004}.



\subsubsection*{Quotient graphs and homomorphic image}

Recall that given an arbitrary partition $P$ of $V_G$, with nonempty parts $V_i$, $i\in I$, we define the quotient graph \index{quotient graph} of $G$ induced by partition $P$ to be the graph $G/P$ with vertex set $\{V_i\mid i\in I\}$, in which there is a loop $(V_i,V_i)\in E_{G/P}$ if $V_i$ contains some $u,v$ with $(u,v)\in E_G$, and in which $(V_i,V_j)\in E_{G/P}$ if some $(u,v)\in E_G$ has $u\in V_i$, $v\in V_j$. Then the canonical mapping that assigns to each $u\in V_G$ the unique $i$ such that $u\in V_i$ is a homomorphism $f:G\rightarrow G/P$, it is actually surjective.


For example, if we take the partition $P=\{V_1,V_2,V_3\}$ by different colours of Frucht graph in Figure~\ref{fig:quo}, i.e.\ $V_1=\{1,3,8,11\}$ (red vertices), $V_2=\{2,5,7,9,10\}$ (blue vertices), $V_3=\{4,6,12\}$ (green vertices), then the quotient graph of Frucht graph induced by $P$ is $K_3$.


Similar as quotient graph, there is another concept `homomorphic image' which is also close connected to surjective homomorphisms. Let $G$ and $H$ be directed graphs, and $f$ is a homomorphism of directed graph $G$ to directed graph $H$.
We define the \emph{homomorphic image of $G$ under $f$}\index{homomorphic image}, denote $f(G)$\index{$f(G)$},
as a directed graph with vertices $\{f(v)\mid v\in V_G\}$, and there is an edge $(f(v),f(w))$ if and only if $v,w\in E_G$.

Note that $f(G)$ is a subgraph of $H$, and that $f:G\rightarrow f(G)$ is a surjective homomorphism.
Conversely, if $f:G\rightarrow H$ is a surjective homomorphism, then $H=f(G)$.



There is a one-to-one correspondence in between quotient graphs and homomorphic images.

\begin{pro}
 Every quotient of $G$ is a homomorphic image of $G$, and conversely, every homomorphic image of $G$ is isomorphic to a
 quotient of $G$.
\end{pro}

\begin{proof}
 Suppose $G/P$ is a quotient graph of $G$ with partition $P=\{V_1,V_2,\dots,V_k\}$, then we assign the canonical mapping that assigns to each vertex $u \in V_G$ the unique $i\in \{1,2,\dots,k\}$ such that $u\in V_i$, $G/P=f(G)$.

For a homomorphic image $f(G)$, we assign an equivalence class by $u\sim v$ if $f(u)=f(v)$ for any $u,v\in V_G$. It is easily seen that
for the partition $P$ induced by $\sim$, $G/P$ is isomorphic to $f(G)$.
\end{proof}


Now we can come to the proof of the decomposition law.


\begin{pro}[Hell, Ne\v set\v ril~\cite{Hell2004}] \label{decomp}
Let $G$ and $H$ be any directed graphs. Every homomorphism $f:G\rightarrow H$ can be written as $f=i\circ s$ where $s$ is a surjective homomorphism and $i$ is an injective homomorphism.
\end{pro}

\begin{proof}
 Recall that the image graph $f(G)$ is a graph with vertex set $f(V_G)$ and $u,v\in f(V_G)$ is an edge in $f(G)$ if and only if there exist $x,y\in V_G$ and $f(x)=u$, $f(y)=v$. $f(G)$ is a subgraph of $H$, thus there is a natural injective homomorphism $i$ from $f(G)$ to $H$. On the other hand, $f$ induces a quotient of $G$ with respect to partition $\theta_f$. Thus we can take $s$ to be canonical surjective homomorphism of $G$ onto $G/\theta_f = f(G)$, and $i$ the inclusion homomorphism of $f(G)$ in $H$.
\end{proof}


\subsection*{Full homomorphisms} \label{sec:full}
Consider the surjective homomorphism from Frucht graph to $K_3$ shown in Table~\ref{tab:FtoK3}. There is no edge for example between vertices 1 and 7 in Frucht graph, but there is an edge between their images Red and Blue in $K_3$. That is because surjective homomorphism does not necessarily preserve non-adjacency relation. In this part we discuss full homomorphisms which preserve both edge and non-edge.

\begin{figure}[!ht]
\centering
\subfloat[$G$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[height=0.75\textwidth]{ex3.1.2.eps}
\end{minipage}}
\subfloat[$H$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[height=0.75\textwidth]{ex3.1.3.eps}
\end{minipage}}
     \caption{A full homomorphism from $G$ to $H$.}
    \label{fig:fige4}
\end{figure}




%\begin{figure}[!ht]
  %\centering
%\begin{tabular}{ccc}
  %  \includegraphics[height=0.22\textwidth]{ex3.1.2.eps} &
%\qquad \qquad \qquad
    %\includegraphics[height=0.22\textwidth]{ex3.1.3.eps} \\
  %  $G$ & \qquad \qquad \qquad $H$\\
%\end{tabular}
  %   \caption{A full homomorphism from $G$ to $H$.}
 %   \label{fig:fige4}
%\end{figure}

\begin{example}
 There is a full homomorphism from $G$ to $H$ as in Figure~\ref{fig:fige4}, by mapping the vertices in graph $G$ to the vertex in the corresponding colour in graph $H$.
\end{example}

To our knowledge, the concept of full homomorphisms first appeared in 1966 in~\cite{Hedetniemi1966}. It has close connection to other variants of graph homomorphisms, for example,
a full homomorphism is a surjective homomorphism in the sense of absence of isolated vertices in $H$. A homomorphism is an embedding if it is both a monomorphism and a full homomorphism. 



\begin{obser}[\cite{Hell2004}]
There are some easy facts regarding to full homomorphisms:
\begin{enumerate}
 \item If $G$ is an induced subgraph of $H$ then the inclusion mapping $i:G\rightarrow H$ is a full injective homomorphism.
 \item Full injective homomorphisms are embeddings.
 \item There exists a full homomorphism $f:G\rightarrow H$ if and only if the vertices of $G$ can be partitioned into
independent sets $S_x$, $x\in V_H$, such that if $xy\notin E_H$ then no edge of $G$ joins the set $S_x$ to the set $S_u$,
and if $xy\in E_H$ then all vertices of $S_x$ are joined in $G$ to all vertices of $S_y$. 
\end{enumerate}
\end{obser}

Recall that graph homomorphism is a generalization of colouring, while full homomorphism is close connected to another colour relatied concept `the achromatic numbers'~\cite{Hell1976}.

\subsubsection*{Point-determining graphs}
Full homomorphism is closely related to point-determining graph, which was introduced by D. Sumner~\cite{Sumner1973} and others in 70s. 

\begin{definition}
{\em Point-determining graphs}\index{point-determining graph} (also known as {\em mating-type graphs}\index{mating-type graphs}, {\em mating graphs}\index{mating graphs}, {\em M-graph}\index{M-graph} or {\em thin graphs}\index{thin graphs}~\cite{Hammack2011}) are graphs in which no two vertices have the same open neighborhood. 
\end{definition}

\begin{example}
 In Fig.~\ref{fig:fige4}, the left graph is not a point-determining graph while the right graph is a point-determining graph. Moreover, there is a full homomorphism from the left graph to the right graph. 
\end{example}



\begin{definition}
  The \emph{thinness relation}\index{thinness relation} $S$ of $G$ is the equivalence relation on
  $V_G$ defined by $(x,y)\in S$ if and only if $N_G(x)=N_G(y)$.
  We denote by $\mathcal{S}$ the corresponding partition of $V_G$, and write
  $R_S\subseteq V_G\times\mathcal{S}$ that associates each vertex with its
  $S$-equivalence class, i.e., $(x,\beta)\in R_S$ if and only if $x\in\beta$.

  The \emph{point-determining graph of $G$}\index{point-determining graph of $G$}, (also called \emph{thin graph of $G$}\index{thin graph of a graph}), denoted by $G_{\mathrm{pd}}$\index{$G_{\mathrm{pd}}$}, is a graph with vertex
  $\mathcal{S}$, two equivalence classes $\sigma$ and
  $\tau$ of $S$ are adjacent in $G_{\mathrm{pd}}$ if and only if $(x,y)$ is an edge of
  $G$ with $x\in\sigma$ and $y\in\tau$.
\end{definition}

Note that $R_S$ is a full homomorphism of $G$ to $G_{\mathrm{pd}}$
\cite{Feder2008}. Also $G_{\mathrm{pd}}$ is indeed a point-determining graph~\cite{Hammack2011}.
We observe that $G$ is obtained from $G_{\mathrm{pd}}$
by vertex duplication. Thinness and the quotients w.r.t.\ the thinness
relation play a role in particular in the context of product graphs, see
\cite{Imrich2000}. In this context it is well known that $G$ can
be reconstructed from $G_{\mathrm{pd}}$ and the knowledge of the $S$-equivalence
classes.


If there is a full homomorphism from graph $G$ to graph $H$, then there is a point-determining graph $K$ such that both $G$ and $H$
has a full homomorphism to $K$.
The correspondence between full homomorphisms and point-determining graphs is explored in greater detail in~\cite{Feder2008}.
In the following we summaries the results of point-determining graph in~\cite{Sumner1973}.

\begin{lemma}[Sumner~\cite{Sumner1973}] \label{lem:pd}
Let $G$ be point-determining. If $N_G(a)=N_G(b)-c$ with $a\neq b$ and $N_G(d)=N_G(e)-a$ with $d\neq e$, then $d=c$.
\end{lemma}

\begin{proof}
Suppose that $d\neq c$. Since $N_G(d)=N_G(e)-a$ we have $e$ and $a$ are adjacent, because $N_G(a)=N_G(b)-c$, then $e\in N_G(a)\subset N_G(b)$. Hence $b\in N_G(e)-\{a\} = N_G(d)$. Since $d\neq c$, $d\in N_G(b)-\{c\}=N(a)$. So $a\in N_G(d)=N_G(e)-\{a\}$, a contradiction.
\end{proof}


\begin{pro} [Sumner~\cite{Sumner1973}]
If $G$ is nontrivial and point-determining, then there exists a vertex $x\in G$ such that $G-\{x\}$ is point-determining.
\end{pro}

\begin{proof}
Suppose no such point exists. Let $x\in G$ be the vertex with largest degree. Then since graph $G-\{x\}$ is not point-determining,
there exist vertices $p,q\in G-\{x\}$ with $p\neq q$ and $N_G(p)=N_G(q)-\{x\}$. Similarly there exist vertices $r,s\in G-\{p\}$ with $r\neq s$
such that $N_G(r)=N_G(q)-\{x\}$, by Lemma~\ref{lem:pd}, $r=x$, so $N_G(x)=N_G(s)-\{p\}$ and thus $d(x)=d(s)-1$, so that $d(s)>d(x)$, which is a contradiction.
\end{proof}




\section{Locally constrained homomorphisms}\label{sec:loc}
%\markboth{\MakeUppercase{\thechapter. Constrained Graph homomorphism }}

In this section we introduce three kinds of locally constrained homomorphisms: locally injective, surjective and bijective homomorphism. Locally constrained homomorphisms play a crucial rule in many application area. There is a comprehensive survey~\cite{Fiala2008} which summaries the important results of locally constrained homomorphisms in structural, algorithmic and applicational aspects.

\begin{definition}
For undirected graphs,
\begin{enumerate}
\item A homomorphism $f:G\to H$ is a {\em locally injective homomorphism}\index{locally injective homomorphism}, or {\em \LocInHomo}\index{\LocInHomo}, if for all $v\in V_G$, the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is injective.
\item A homomorphism $f:G\to H$ is a {\em locally surjective homomorphism}\index{locally surjective homomorphism}, or {\em \LocSurHomo}\index{\LocSurHomo}, if for all $v\in V_G$, the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is surjective.
\item A homomorphism $f:G\to H$ is a {\em locally bijective homomorphism}\index{locally bijective homomorphism}, or {\em \LocBiHomo}\index{\LocBiHomo}, if it is both a locally surjective and locally bijective homomorphism. That is if the restrictions on neighborhoods are bijections.
\end{enumerate}
\end{definition}


There is an alternative and quite natural definition shown in~\cite{Fiala2005}:

\begin{enumerate}
\item A homomorphism $f:G\to H$ is a {\em locally injective homomorphism}\index{locally injective homomorphism}, if for every edge $(u,v)$ of $H$, the subgraph
of $G$ induced by $f^{-1}(u)\cup f^{-1}(v)$ is a matching.
\item A homomorphism $f:G\to H$ is a {\em locally surjective homomorphism}\index{locally surjective homomorphism}, if for every edge $(u,v)$ of $H$, the subgraph
of $G$ induced by $f^{-1}(u)\cup f^{-1}(v)$ is a bipartite graph without isolated vertices.
\item A homomorphism $f:G\to H$ is a {\em locally bijective homomorphism}\index{locally bijective homomorphism}, if For every edge $(u,v)$ of $H$, the subgraph
of $G$ induced by $f^{-1}(u)\cup f^{-1}(v)$ is a perfect matching.
\end{enumerate}
%Let $f: G\rightarrow H$ be a graph homomorphism. For every edge $(u,v)$ of $H$, the subgraph
%of $G$ induced by $f^{-1}(u)\cup f^{-1}(v)$ is a
%perfect matching if and only if $f$ is locally bijective,
%matching if and only if $f$ is locally injective,
%bipartite graph without isolated vertices if and only if $f$ is locally surjective.

In accordance with the notation used for ordinary graph homomorphisms we write $G\LocInHom H$, $G\LocSurHom H$, $G\LocBiHom H$ for the existence of locally injective, surjective and bijective homomorphisms.

Compare to global homomorphisms, locally homomorphisms have its own interesting properties and applications.
Figure~\ref{fig:loc} shows examples of locally injective ($G_i$ to $H$), locally bijective ($G_b$ to $H$), locally surjective homomorphism ($G_s$ to $H$).
It is easily seem that a locally injective (locally bijective) homomorphism is not necessarily an injective (bijective) homomorphism, but a locally surjective homomorphism between two connected graph is a surjective homomorphism.


\begin{figure}[!ht]
\centering
\includegraphics[width=0.55\textwidth]{local.eps} 
\caption{Locally injective, bijective, surjective homomorphisms~\cite{Fiala2008}.}
\label{fig:loc}
\end{figure}


Locally surjective homomorphisms were firstly introduced by Everett and Borgatti, who called them \emph{role colourings}\index{role colouring}~\cite{Everett1991}. It is originated in the theory of social behaviour. The source graph $G$ represents relations between particular individuals of some group. The target graph $H$ is called the role graph. The task is to assign roles to individuals so that each person given a particular role has, among its neighbors, every role prescribed by the role graph at least once, while no other roles may appear in the neighborhood~\cite{Fiala2008}.
where individuals of the same social role relate to other individuals in the same way~\cite{Fiala2008}.
In this thesis, the other two kinds of locally constrained homomorphisms are more of our interest, we thus introduce them in greater detail.


\subsubsection*{Locally injective homomorphism} \label{sec:li}
Locally injective homomorphism, sometimes called \emph{local monomorphism}\index{local monomorphism}~\cite{Nesetril1971}
or \emph{partial covering projection}\index{partial covering projection}~\cite{Fiala2001}, has an interesting history and a wide application. It has very close connection to the frequency assignment problem, which is a highly practical problem of interference-free frequency assignment for wireless networks~\cite{Fiala2008}.
Locally injective homomorphisms (also called local epimorphisms or partial covers) are also used in distance constrained labelings of graphs~\cite{Fiala2001}
and as indicators of the existence of homomorphisms of derivative graphs (line graphs)~\cite{Nesetril1971}.

Observe that if there is a locally injective homomorphism from graph $G$ to graph $H$, then for any vertex $v\in V_G$,
$|N(v)|\leq |N(f(v))|$. 
Consequently, locally injective homomorphism from a graph to itself preserves the degrees, i.e.,
if $f$ is a locally injective homomorphism from graph $G$ to itself, then for any vertex $v\in V_G$,
$d(v)=d(f(v))$. There is a classical result about locally injective homomorphisms from a graph to itself which was shown in 1971:


\begin{thm}[Ne\v{s}et\v{r}il~\cite{Nesetril1971}] \label{thm:locin-auto}
 Let $G$ be a connected finite graph. Then every locally injective homomorphism of $G$ into itself
 is an automorphism.
\end{thm}

\begin{proof}
 We prove the statement by induction on $|G|$.
 It is easily seen that for $|G|=2$ the proposition holds. Let $|G|>2$, suppose that the statement
 of the proposition holds for all connected graphs $H$ with $|H|<|G|$. We assume there is a locally
 injective homomorphism $f$ from $G$ to itself which is not an automorphism, then $f(V_G) \subset V_G$ and the homomorphic image $f(G)$ is a connected graph.
 Take a vertex $v\in V_G \setminus f(V_G)$, consider the graph $G-v$. Let $G^1,\dots,G^n$ be the disjoint connected components of $G-v$, because $G$ is a connected graph, for each $G^i$, there exists a vertex $v^i$ which is connected to $v$. Suppose the image of $v$ is in $G^j$ where $1\leq j\leq n$, then from the properties of locally injective homomorphism, for all $i$, $f(v^i)\in G^j$. Because of the connectivity,  $f(G^i)\subset G^j$ for any $i$. It is easily seen that the restriction of $f$ to $G^j$
 is also a locally injective homomorphism, from the induction hypothesis it is an automorphism.
 Consider any vertex $w$ in the set of $N_G(v)\cap G^j$, then $f(N_{G^j}(w))=N_{G^i}(w)$. But $v\in V_G(w)$ and $v\notin f(N_G(w))$, then $f$ is not a locally injective homomorphism of $G$ to itself, which is a contradiction.
\end{proof}

\subsubsection*{Locally bijective homomorphisms} \label{sec:lb}

A locally bijective homomorphism is also locally injective and locally surjective. Hence,
any result valid for locally injective or locally surjective homomorphism is also valid for locally bijective
homomorphisms. Locally bijective homomorphisms (also known as \emph{local isomorphisms}\index{local isomorphisms} or \emph{full covering projection}\index{full covering projection}~\cite{Fiala2001}) have important
applications in many areas, for example distributed computing, recognizing graphs by networks of
processors or constructing highly transitive regular graphs~\cite{Fiala2005}. 

For locally bijective homomorphisms the preimage classes of all vertices have the same size
and for locally surjective homomorphisms all the preimage classes have size at least one.
If there is a locally bijective homomorphism from graph $G$ to graph $H$, then either $|V_G|>|V_H|$
or else $G$ and $H$ are isomorphic.

Just like graph isomorphisms, a locally bijective homomorphism maintains vertex degrees and degrees
of neighbours and degrees of neighbours of neighbours and so on.
The existence of such a mapping from $G$ to $H$ therefore implies equality of the so-called
\emph{degree refinement matrices}\index{degree refinement matrices} of $G$ and $H$.

\subsubsection*{Degree decomposition matrix}
\label{sec:DRM}
Consider a locally bijective homomorphism $f:G\LocBiHom H$. By definition, for every vertex $x$, $f$ induces an isomorphism from the neighbourhood of $x$, $N_G(x)$, to the neighbourhood of $f(x)$, $N_H(f(x))$. In particular $x$ and $f(x)$ have the same degree. (For every vertex $x'\in N_G(x)$ the neighbourhood of $x'$ must be isomorphic to the neighbourhood of $f(x')$ that itself lies in the neighbourhood of $f(x)$.) It follows that locally bijective homomorphisms preserve not only the degrees of vertices, but also the degrees of neighbourhood vertices and so on. This property is well captured by the notion of degree refinement matrices~\cite{Fiala2005}.

A partition of the vertex set of a graph $G$ into disjoint classes is an {\em equitable partition}\index{equitable partition} if the vertices in the same class have the same numbers of neighbours in all classes of the partition.

The relation `being finer' defines a lattice on the set of all equitable partitions of a fixed graph.
Every finite graph admits a unique minimal equitable partition~\cite{Everett1991}.

Any equitable partition is characterized by the associated {\em degree decomposition matrix}\index{degree decomposition matrix} whose rows and columns are indexed by the blocks of the partition, and the entry in the $i$-th row and $j$-th column describes how many neighbors a vertex from the $i$-th block has in the $j$-th block.

Every finite graph $G$ admits a unique minimal equitable partition. In this case a canonical ordering can be imposed on the blocks, so the corresponding degree matrix, called the {\em degree refinement matrix}, $\drm(G)$, is also defined uniquely.

We put $G\Matrixeq H$ if and only if $\drm(G)=\drm(H)$. The relation $\Matrixeq$ is an equivalence relation on the class of finite connected graphs, $\ConnGraph$.

It is easy to observe that given a pair of graphs $(G,H)$ with $\drm(G)\neq \drm(H)$ there is no locally bijective homomorphism $G\LocBiHom H$.
Consequently the relation $\LocBiHom$ is a sub-relation of $\Matrixeq$.
The connections between $\Matrixeq$ and all three variants of locally constrained homomorphisms is captured by the following so called Cantor-Bernstein type theorems.

\begin{thm}[Fiala, Kratochv\'{\i}l~\cite{Fiala2001}]
\label{thm:degeq1}
 If two graphs $G$ and $H$ share the same degree refinement matrix, then every locally injective homomorphism from $G$ to $H$ is locally bijective.
\end{thm}

\begin{thm}[Kristiansen, Telle~\cite{Kristiansen2000}]
\label{thm:degeq2}
 If two graphs $G$ and $H$ share the same degree refinement  matrix, then every locally surjective homomorphism from $G$ to $H$ is locally bijective.
\end{thm}

It is not necessary to have locally bijective homomorphisms between two graphs with the same degree refinement matrix, for example, $C_3,C_4$ and $C_5$ share the same degree refinement matrix $\{2\}$, but they are independent in locally bijective homomorphism.


Because the degree refinement matrix is easy to compute, 
for many pair of graphs $(G,H)$ we can easily determine that a locally
bijective homomorphism from $G$ to $H$ does not exist.

\subsubsection*{Universal cover}
The notion of \emph{universal cover}\index{universal cover} is well established in topology of
continuous spaces. 
 One requirement of universal cover is simply connected, which translates in terms of graph theory to be a requirement of being acyclic and connected, that is a tree. In the discrete case, formally, the \emph{universal covering graph}\index{universal covering graph} (or \emph{universal cover}\index{universal cover}) of a graph $H$ is the only (possibly infinite) tree $T_H$ that allows a
locally bijective homomorphism to $H$.


If $G$ is a tree, then $G$ itself is the universal covering graph of $G$.
The universal covering graph of other connected graph is a countably infinite (but locally finite) tree. 


The universal covering graph $T_G$ of a connected graph $G$ can be constructed as follows\footnote{This construction is from \textit{Covering graph. (2012, September 3). In Wikipedia, The Free Encyclopedia. Retrieved 09:51, February 20, 2014, from \url{http://en.wikipedia.org/w/index.php?title=Covering_graph&oldid=510586814}}.}. Choose an arbitrary vertex $r$ of $G$ as a starting point. Each vertex of $T_G$ is a non-backtracking walk that begins from $r$, that is, a sequence $w = (r, v_1, v_2, ..., v_n)$ of vertices of $G$ such that
$v_i$ and $v_{i+1}$ are adjacent in $G$ and $v_{i-1} \neq v_{i+1}$ for all $i$.
Then, two vertices of $T_G$ are adjacent if one is a simple extension of another: the vertex $(r, v_1, v_2, ..., v_n)$ is adjacent to the vertex $(r, v_1, v_2, ..., v_{n-1})$. Up to isomorphism, the same tree $T_G$ is constructed regardless of the choice of the starting point $r$. Thus the universal covering graph is unique up to isomorphism.

The covering map $f$ maps the vertex $(r)$ in $T_G$ to the vertex $r$ in $G$, and a vertex $(r, v_1, v_2, ..., v_n)$ in $T$ to the vertex $v_n$ in $G$.

Figure~\ref{fig:cover} gives an example of universal covering graph.

\begin{figure}[!ht]
\centering
\includegraphics{Covering.eps} 
\caption{$H$ and its universal covering graph.}
\label{fig:cover}
\end{figure}



Suppose $f$ is a homomorphism from graph $G$ to graph $H$. 
If $f$ is locally injective, then the tree $T_G$ is a subtree of $T_H$;
if $f$ is locally surjective, then $T_H$ is a subtree of $T_G$;
if $f$ is locally bijective, then $T_G$ and $T_H$ are isomorphic.

The following theorem shows the connection between degree refinement matrix and universal cover.

\begin{thm}[Leighton~\cite{Leighton1982}]
Two graphs $G$ and $H$ share the same degree refinement matrix if and only if their universal covers are
isomorphic.
\end{thm}


\section{Relations}
In next chapter we will discuss the theory of relations in more detail.

\begin{definition}\label{def:muls}
  Let $G=(V_G,E_G)$ be a graph, $B$ a finite set, and $R\subseteq V\times
  B$ a binary relation, where for every element $b\in B$, we can find an
  element $v \in V_G$ such that $(v,b)\in R$. Then the graph $G\muls R$\index{$G\muls R$} has
  vertex set $B$ and edge set
\begin{equation*}
  E_{G\muls R} = \left\{ (u,v)\in B\times B \mid \textrm{ there is }
  (x,y)\in E_G \textrm{ and } (x,u),(y,v)\in R \right\}.
\end{equation*}
\end{definition}

Graphs with loops are not always a natural model, however, so that
it may appear more appealing to consider the slightly modified definition.
\begin{definition}\label{def:mulw}
Let $G=(V_G,E_G)$ be a simple graph, $B$ a finite set, $R$ a binary relation,
where for every element $b\in B$, we can find an element $v \in V_G$ such that
$(v,b)\in R$. Then the (simple) graph $G\mulw R$\index{$G\mulw R$} has vertex set $B$ and edge
set
\begin{equation*}
  E_{G\mulw R} = \left\{ (u,v)\in B\times B \mid u\ne v \textrm{ and there is }
  (x,y)\in E_G \textrm{ and } (x,u),(y,v)\in R \right\}.
\end{equation*}
\end{definition}

We remark that the definitions remain meaningful for directed graphs,
weighted graphs (where the weight of edge is a sum of weights of its
pre-images) as well as relational structures. For simplicity, we restrict
ourselves to undirected graphs (with loops). Most of the results can be
directly generalized.

Graphs can be regarded as representations of symmetric binary
relations. Using the same symbol for the graph and the relation it
represents, we may re-interpret definition~\ref{def:muls} as a conjugation
of relations. $R^+$ is the \emph{transpose}\index{transpose} of $R$, i.e., $(u,x)\in R^+$
if and only if $(x,u)\in R$. The double composition $R^+\circ G\circ R$
contains the pair $(u,v)$ in $B\times B$ if and only if there are $x$ and
$y$ such that $(u,x)\in R^+$, $(y,v)\in R$, and $(x,y)\in E_G$. Thus
\begin{equation*}
  G\muls R = R^+\circ G\circ R.
\end{equation*}

Simple graphs, analogously, correspond to the irreflexive symmetric
relations. For any relation $R$, let $R^\iota$\index{$R^\iota$} denote its irreflexive
part, also known as the \emph{reflexive reduction}\index{reflexive reduction} of $R$. Since
definition~\ref{def:mulw} explicitly excludes the diagonals, it can be
written in the form
\begin{equation*}
  G\mulw R = (R^+\circ G\circ R)^{\iota}.
\end{equation*}
We have $G\mulw R = (G\muls R)^{\iota}$, and hence $E_{G\mulw R}\subseteq
E_{G\muls R}$. The composition $G\muls R$ is of particular interest when
$G$ is also a simple graph, i.e., $G=G^{\iota}$.

If there is an $R$ such that $G\muls R=H$ holds, we say there is a \emph{relation}\index{relation} from $G$ to $H$.
If there is an $R$ such that $G\mulw R=H$ holds, we say there is a \emph{weak relation}\index{weak relation} from $G$ to $H$.

The main part of this contribution will be concerned with the solutions of
the equation $G\muls R=H$. The weak version, $G\mulw R=H$, will turn out
to have much less convenient properties, and will be discussed only briefly
in Section~\ref{sect:weak}.

\vspace{10pt}
Throughout this thesis we use the following standard notations and terms.


For relation $R\subseteq X\times Y$ we define by
$R(x)=\{p\in Y\mid (x,p)\in R\}$\index{$R(x)$} the \emph{image of $x$ under $R$}\index{image under relation} and
$R^{-1}(p)=\{x\in X\mid (x,p)\in R\}$\index{$R^{-1}(p)$} the
\emph{pre-image of $p$ under $R$}\index{pre-image under relation}.


The \emph{domain}\index{domain} of $R$ is defined by $\domain{R}=\{x\in
X\mid \exists p\in Y\text{ s.t. }(x,p)\in R\}$\index{$\domain{R}$}, and the \emph{image}\index{image} of
$R$ is defined by $\image{R}=\{p\in Y\mid \exists x\in X\text{
  s.t. }(x,p)\in R\}$\index{$\image{R}$}. We say that the \emph{domain of $R$ is full}\index{domain is full} if for
any $x\in X$ we have $R(x)\ne\emptyset$. Analogously, the \emph{image is
full}\index{image is full} if for any $p\in Y$ we have $R^{-1}(p)\ne\emptyset$.

Let $R\subseteq X\times Y$ is a binary relation, then $R$ is
\emph{injective}\index{injective}, if for all $x$ and $z$ in $X$ and $y$ in
$Y$ it holds that if $(x,y)\in R$ and $(z,y)\in R$ then $x = z$.
$R$ is \emph{functional}\index{functional}, if for all $x$ in $X$, and $y$ and
$z$ in $Y$ it holds that if $(x,y)\in R$ and $(x,z)\in R$ then
$y = z$.

We denote by $I_G$\index{$I_G$}\index{$I_G$} the \emph{identity map on $G$}\index{identity map,identity}, i.e.,
$\{(x,x)\mid x\in V_G\}$.


\subsection*{Matrix multiplication}
The operation $\muls$ can also be formulated in terms of matrix
multiplication. To see this, consider the following variant of the
operation on weighted graphs.
\begin{definition}\label{mult_w}
If $G$ is a weighted graph, we use $w(x,y)$\index{$w(x,y)$} to denote the weight between
$x$ and $y$. Given a finite set $B$ and a binary relation $R\subseteq
V_G\times B$, $G\mulm R$ is defined as a weighted graph $H$ with vertex set
$B$, for any $u,v\in B$, $w(u,v)=\sum_{(x,u)\in R,(y,v)\in R} w(x,y)$.
\end{definition}
Ignoring the weights, operations $\muls$ and $\mulm$ are equivalent.

Using the language of matrices, $G\mulm
 R=H$ can be interpreted as
matrix multiplication:
\begin{equation*}
  \textbf{W}_{G\mulm R} = \mathbf{R}^+ \mathbf{W}_G \mathbf{R}
\end{equation*}
where $\mathbf{R}$ is the matrix representation of the relation $R$,
i.e., $\mathbf{R}_{xu}=1$ if and only if $(x,u)\in R$, otherwise
$\mathbf{R}_{xu}=0$, $\mathbf{R}^+$\index{$\mathbf{R}^+$} denotes the transpose of
$\mathbf{R}$, and $\mathbf{W}_G$ is the matrix of edge weights of
$G$.

\subsection*{Homomorphisms and multihomomorphisms}

The notion of relations between graphs is in many ways similar (but not
equivalent) to the well studied notion of graph homomorphisms. The majority
of our results focus on similarities and differences between those two
concepts. 

Recall that a \emph{(strong) homomorphism}\index{strong homomorphism}\index{homomorphism} from a graph $G$ to a graph $H$ is a mapping
$f:V_G\to V_H$ such that for every edge $(x,y)$ of $G$, $(f(x), f(y))$ is
an edge of $H$. Note that strong homomorphisms require loops in $H$
whenever $(x,y)\in E_G$ and $f(x)=f(y)$. In contrast, we define $f$ is a \emph{weak
  homomorphism}\index{week homomorphism} if $(x,y)\in E_G$ implies that either $f(x)=f(y)$ or
$(f(x),f(y))\in E_H$. Every strong homomorphism from $G$ to $H$ induces
also a weak homomorphism, but not conversely. Weak homomorphisms play an important role in graph product, see~\cite{Imrich2000}.


A map $f:V_G\to V_H$ is, of course, a special case of a relation. This is
seen by setting $F=\{(x,f(x))\mid x\in V_G\}$. Hence, there is a strong
surjective homomorphism from $G$ to $H$ if and only if there is a
functional relation $F$ such that $G\muls F=H$. Another important connection to
the graph homomorphisms is the following simple lemma.
\begin{lemma} \label{reho}
  If $G\muls R = H$, and the domain of $R$ is full, then there is a
  homomorphism $f$ from $G$ to $H$ contained in $R$.
\end{lemma}

\begin{proof}
  If $G\muls R = H$, then take any functional relation $f\subseteq R$, we
  have $G\muls f \subseteq H$, where $f$ is a homomorphism from $G$ to $H$.
\end{proof}

Analogously, there is a \emph{weak surjective homomorphism}\index{weak surjective homomorphism} from $G$ to
$H$ if and only if there is a functional relation $F$ such that $G\mulw F=H$,
and there is a weak homomorphism from $G$ to $H$ if there is a functional
relation $F\subseteq V_G\times V_H$ such that $G\mulw F$ is a subgraph of
$H$. The existence of relations between graphs thus can be seen as a proper
generalization of weak or strong graph homomorphisms, respectively.


Relations between graphs can be regarded also as a variant of
multihomomorphisms. Multihomomorphisms are building blocks of
Hom-complexes, introduced by Lov{\'a}sz, and are related to recent exciting
developments in topological combinatorics~\cite{Matousek2003}, in particular
to deep results involved in proof of the Lov{\'a}sz hypothesis~\cite{Babson2006}.

A \emph{multihomomorphism}\index{multihomomorphism} $G\rightarrow H$ is a mapping $f:
V_G\rightarrow 2^{V_H} \setminus \{ \emptyset \}$ (i.e., associating a
nonempty subset of vertices of $H$ with every vertex of $G$) such that
whenever $\{ u_1,u_2\}$ is an edge of $G$, we have $(v_1,v_2)\in E_H$ for
every $v_1\in f(u_1)$ and every $v_2\in f(u_2)$.

The functions from vertices to sets can be seen as representation of
relations. A relation with full domain thus can be regarded as
\emph{surjective multihomomorphism}\index{surjective multihomomorphism}, a multihomomorphism such that
pre-image of every vertex in $H$ is non-empty and for every edge $(u,v)$ in
$H$ we can find an edge $(x,y)$ in $G$ satisfying $u\in f(x)$, $v\in f(y)$.

\subsection*{Examples}

Similarly to graph homomorphisms, the equation $G\muls R=H$ (or $G\mulw R=H$
respectively) may have multiple solutions for some pairs of graphs $(G,H)$,
while there may be no solution at all for other pairs.

As an example, consider $K_2$ (two vertices $x,y$ connected by an edge) and
$C_3$ (a cycle of three vertices $u,v,w$). Denote $R_1=\{(u,x),(v,y)\}$,
$R_2=\{(v,x),(w,y)\}$, $R_3=\{(w,x),(u,y)\}$, then it is easily seen that
$C_3\muls R_i=K_2$ for each $1\leq i\leq 3$, i.e., the equation $C_3\muls
R=K_2$ has more than one solution.

On the other hand, there is no relation $R$ such that $K_2\muls R=C_3$.
Otherwise, each vertex of $C_3$ is related to at most one vertex of $K_2$,
since $C_3$ is loop free; hence there exists a vertex in $K_2$ which has no
relations to at least two vertices in $C_3$, w.l.o.g., one can assume
$(x,u), (x,v)\notin R$; then the definition of $\muls$ implies that there
is no edge between $u$ and $v$, which causes a contradiction.

Because relations do not need to have full domain (unlike graph
homomorphisms), there is always a relation from a graph $G$ to its induced
subgraph $G[W]$.

Relations with full domain are not restricted to surjective
homomorphisms. As a simple example, consider paths $P_1$ with vertex set
$\{x,y\}$ and $P_2$ with vertex set $\{u,v,w\}$, respectively, and set
$R=\{(x,u),(x,w),(y,v)\}$. One can easily verify $P_1\muls R=P_2$ by direct
computation. Here, $R$ is not functional since $x$ has two images.

Note that, quite surprisingly, there is no relation $R$ satisfying
$P_2\muls R=P_3$. In fact $(P_1,P_2)$ is the only pair of paths such that
there is a relation from one to another and vice versa. This will be further
explained in Section~\ref{sub:dist}.



% ------------------------------------------------------------------------

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> Chapter3/chapter3_beforeAndrew.tex <==
\chapter[R-Homomorphisms (relations)]{\fontsize{32}{12}\selectfont R-Homomorphisms (relations)}
\label{ch:relation}
\ifpdf
    \graphicspath{{Chapter3/Chapter3Figs/PNG/}{Chapter3/Chapter3Figs/PDF/}{Chapter3/Chapter3Figs/}}
\else
    \graphicspath{{Chapter3/Chapter3Figs/EPS/}{Chapter3/Chapter3Figs/}}
\fi

%\section{Outline and main results}
%\markboth{\MakeUppercase{\thechapter. R-Homomorphism }}{\thechapter. R-Homomorphism} %Chaptial LETTER DAXIE


%\subsection*{Outline and Main Results}

This chapter is organized as follows:

In Section~\ref{sect:basic} the basic properties of the strong relations
between graphs are compiled. It is shown that relations compose and every
relation can be decomposed in a standard way into a surjective and an
injective relation (Corollary~\ref{DeCo}). We discuss some structural
properties of graphs preserved by relations.

Equivalence on the class of graphs induced by the existence of relations
between graphs is the topic of section~\ref{sect:retract}. We consider two
forms: the strong relational equivalence, where relations are required to
be reversible, and weak relational equivalence. Equivalent classes of
strong relational equivalence are characterized in Theorem~\ref{thm:equi}.
To describe equivalence classes of the weak relational equivalence we
introduce the notion of an R-core of a graph and show that it is in many
ways similar to the more familiar construction of the graph core
(Theorem~\ref{thm:Rcore}). We explore in particular the differences between
core and R-core and provide an effective algorithm to compute the R-cores of
given graphs.

Section~\ref{sect:poset} is concerned with the partial order induced on
relations between two fixed graphs $G$ and $H$ by inclusion. Focusing on the special
case $G=H$, we describe the minimal elements of this partial order. In
Theorem~\ref{thm:auto1} we give a, perhaps surprisingly simple,
characterization of those graphs whose relations to
themselves are automorphisms.

R-retractions are defined in Section~\ref{sect:retraction} in analogy to
retractions. It naturally gives rise to a notion of R-reduced graphs that
we show to coincide with the concept of graph cores. By reversing the
direction of relations, however, we obtain the concept of a cocore of a
graph, which does not have a non-trivial counterpart in the world of
ordinary graph homomorphisms, and we explore its properties. Finally, we give
a full list of the inclusion relation of these notions
and give examples to distinguish them.

The computational complexity of testing for the existence of a relation
between two graphs is briefly discussed in Section~\ref{sect:complexity}.
In Theorem~\ref{thm:complex} we describe the reduction of this problem to
the surjective homomorphism problem.

Finally, in Section~\ref{sect:weak} we briefly summarize the most important
similarities and differences between weak and strong relational
compositions.




\section{Basic properties}
\label{sect:basic}



\subsection*{Composition}

Recall that the composition of binary relations is associative, i.e.,
suppose $R\subseteq W\times X$, $S\subseteq X\times Y$, and $T\subseteq
Y\times Z$. Then $R\circ(S\circ T)=(R\circ S)\circ T$. Furthermore, the
transposition of relations satisfies $(R\circ S)^+ = S^+ \circ
R^+$. Interpreting a graph $G$ as a relation on its vertex set, we easily
derive the following identities.

\begin{lemma}[Composition law]\label{lem:compo}
  $(G\muls R)\muls S = G\muls(R\circ S)$.
\end{lemma}
\begin{proof}
\abovedisplayskip=-12pt
\belowdisplayskip=-12pt
\begin{equation*}
\begin{split}
(G\muls R)\muls S
 & = S^+\circ(R^+\circ G\circ R)\circ S =(S^+\circ R^+)\circ G\circ (R\circ S)\\
 & =(R\circ S)^+ \circ G\circ (R\circ S) = G\muls(R\circ S).
\end{split}
\end{equation*} 
\end{proof}

Now we show that every relation $R$ can be decomposed, in a standard way,
to a relation $R_D$ duplicating vertices and a relation $R_C$ contracting
vertices.

\begin{lemma} \label{dec}
  Let $R\subseteq X\times Y$ be a relation. Then there exists a subset $A$ of
  $X$, a set $B$, an
  injective relation with full domain $R_D\subseteq A\times B$ and a
  functional relation $R_C\subseteq B\times Y$, such that $R=I_A\circ
  R_D\circ R_C$, where $I_A$ is the identity on $X$ restricted to $A$.
\end{lemma}
\begin{proof}
  Put $A=\domain{R}$.
  Then the relation $I_A$ removes
  vertices in $X\setminus\domain{R}$. Therefore, it remains
  to show, that any relation $R\subseteq X\times Y$ with full
  domain can be decomposed into an injective relation
  $R_D\subseteq X\times B$ and a
  functional relation $R_C\subseteq B\times
  Y$. To see this, set $B=R$ and declare $(x,\alpha)\in R_D$ if and only if
  $\alpha=(x,p)\in R$ for some $p\in Y$, and $(\beta,q)\in R_C$ if and only if
  $\beta=(y,q)\in R$ for some $y\in X$. By construction $R_D$ is injective
  and $R_C$ is functional. Furthermore, $(x_0,p_0)\in R_D\circ R_C$ if and
  only if there is an $\alpha\in R$ that is simultaneously of the form
  $(x_0,p)$ and $(x,p_0)$, i.e., $x=x_0$ and $p=p_0$. Hence $(x_0,p_0)\in
  R$.
\end{proof}

Note that this decomposition is not unique. For instance, we could
construct $B$ from multiple copies of $R$. More precisely, let $B=R\times
\{1,2,\dots,k\}$, then we would set $\big(x,(\alpha,i)\big)\in R_D$
($1\leq i\leq k$) if and only if $\alpha=(x,p)\in R$ for some $p\in Y$,
etc.

The set $B$ as constructed in the proof of Lemma~\ref{dec} has
minimal size. To see this, it suffices to show that, given $B$ there
is a mapping from $B$ onto $R$. Since $R_D$ is injective and $R_C$ is
functional we may set
$$\alpha\in B\mapsto (R_D^{-1}(\alpha),R_C(\alpha)).$$
Since $R=I_A\circ R_D\circ R_C$ we conclude that the mapping is
surjective, and hence $|B|\geq |R|$.

According to Lemma~\ref{lem:compo}, the decomposition of $R$ in
Lemma~\ref{dec} can be restated as follows:
\begin{cor} \label{DeCo}
Suppose $G\muls R=H$. Then there is a set $B$, an injective relation
$R_D\subseteq \domain R\times B$ with full domain, and a surjective relation
$R_C\subseteq B\times \image R$ such that
$G[\domain R]\muls R_D\muls R_C=H$.
\end{cor}

In diagram form, this is expressed as
  \begin{figure}[!ht]
  \centering
  \includegraphics[width=0.25\textwidth]{comum.eps} 
\caption{Commutative diagram.}
\label{fig:comum}
\end{figure}   

We will remark that from the fact the relations compose it follows that
the existence of a relation implies a quasi-order on graphs that is related
to the homomorphism order. This order is studied more deeply in~\cite{Fiala2012}.

\subsection*{Structural properties preserved by relations}

In this subsection we investigate structural properties of $H$ that can be
derived from knowledge about certain properties of $G$ and the fact that
there is some relation $R$ such that $G\muls R=H$.

\subsubsection*{Connected components}

\begin{pro}\label{ccs}
  Let $G\muls R=H$ and denote by $H_1,\dots,H_k$ the (non-empty) connected components
  of $H$. Then there are relations $R_i\subseteq V_G\times V_{H_i}$ such
  that $G\muls R_i=H_i$ for each $1\leq i\leq k$ and $R=\bigcup_{i=1}^k
  R_i$. Furthermore, set $G_i=G[R^{-1}(V_{H_i})]$, then there are no edges
  between $G_i$ and $G_j$ for arbitrary $i\neq j$.
\end{pro}

\begin{proof}
  Define the restriction of $R$ to the connected components of $H$ as
  $R_i=\{(x,y)\in R\mid y\in V_{H_i}\}$. Clearly, $R$ is the disjoint union of
  $R_i$ and $G\muls R_i\subseteq H_i$. The definition of $\muls$
  implies $H=G\muls R= \left(\bigcup_i R_i\right)^+ \circ G\circ
  \left(\bigcup_j R_j\right) = \bigcup_i\bigcup_j R_i^+ \circ G\circ R_j$.
  Since for $i\neq j$, $R_i$ and $R_j$ relate vertices of $G$ to different connected
  components of $H$, we have $R_i^+ \circ G\circ R_j=\emptyset$. It follows
  that $H=\bigcup_i\bigcup_j R_i^+\circ G\circ R_j = \bigcup_i R_i^+\circ
  G\circ R_i = \bigcup_i G\muls R_i$. Hence $G\muls R_i=H_i$.

  Any edge between $G_i$ and $G_j$ would generate edges between $H_i$ and
  $H_j$, which causes a contradiction to our assumptions.
\end{proof}

Denote by $b_0(G)$ the number of connected components of $G$, then from
Proposition~\ref{ccs} we arrive at:
\begin{cor}\label{cor:concomp}
  Suppose both $G$ and $H$ do not have isolated vertices. If $G\muls R=H$
  and $R$ has full domain, then $b_0(G)\geq b_0(H)$.
\end{cor}
\begin{proof}
  Our notation is the same as in Proposition~\ref{ccs}. We claim for arbitrary
  connected component $C$ of graph $G$, there exists a unique $i$, such that
  $C$ is a connected component of $G_i$. Otherwise one can find two
  vertices $x,y\in C$, $x$ and $y$ adjacent,
  such that $x\in V_{G_i}$ and $y\in V_{G_j}$, since $G$ has no isolated
  vertices, which contradicts
  $E(G_i,G_j)=\emptyset$. Thus it follows $b_0(G)\geq b_0(H)$.
\end{proof}

From Corollary~\ref{cor:concomp}, we know that $H$ is connected whenever $G$
is connected. Conversely, the connectedness of $G$, however, cannot be deduced from the
connectedness of $H$. For example, consider $G=P_1\cup P_1$ with vertex set
$\{x_1,x_2,x_3,x_4\}$ and edges $\{x_1,x_2\}$ and $\{x_3,x_4\}$, and
$H=P_2$ with vertex set $\{v_1,v_2,v_3\}$. Set
$R=\{(x_1,v_1),(x_2,v_2),(x_3,v_2),(x_4,v_3)\}$. One can easily verify that
$G\muls R=H$. On the other hand, $H$ is connected but $G$ has 2 connected
components. The point here is, of course, that $R$ is not injective.

\subsubsection*{Colorings}
Graph homomorphisms of simple graphs can be seen as generalizations of
colourings. Thus, if $R$ is a
functional relation describing a vertex colouring, then $G\muls R\subseteq
K_k$. Conversely, if $G\muls R\subseteq K_k$, where $R$ has full domain,
then from Lemma~\ref{reho}, there exists a homomorphism from $G$ to
$K_k$, which is a colouring of $G$.
\begin{lemma} \label{colour} If $G$ is a simple graph and $R$ has full
  domain, then $\chi(G)\leq \chi(G\muls R)$.
\end{lemma}

\begin{proof}
  Suppose $G\muls R=H$ and the domain of $R$ is full, from Lemma~\ref{reho}
  we know $G\rightarrow H$, so $\chi(G)\leq \chi(G\muls R)$.
\end{proof}

\subsubsection*{Distances} \label{sub:dist}
\begin{obser} \label{path} If $P_k\muls R=G$, $G$ is a simple graph and the
  domain of $R$ is full, $P_k$ with the vertex set ${0,1,\dots,k}$, then
  there is a walk $[v_0,v_1,\dots,v_k]$ in $G$, where $(i,v_i)\in R$ for
  $0\leq i\leq k$.
\end{obser}

\begin{obser} \label{cycle} If $C_k\muls R=G$, $G$ is a simple graph and
  the domain of $R$ is full, then there is a closed walk
  $[v_0,v_1,\dots,v_{k-1}]$ in $G$, where $(i,v_i)\in R$ for $0\leq i\leq
  k-1$.
\end{obser}

Recall that $d_G(x,y)$ denote the \emph{(canonical) distance}\emph{(canonical) distance}\index{canonical distance, distance} on graph $G$, i.e.,
$d_G(x,y)$ is the minimal length of a path in graph $G$ that connects
vertices $x$ and $y$; if there is no path that connects vertices $x$ and $y$,
then the distance is infinite.

\begin{lemma}
  Suppose there exists a relation $R$ with full domain s.t.\ $G\muls R=H$,
  $x,y\in V_G$, $u,v\in V_H$ and $(x,u)\in R, (y,v)\in R$. If $x\neq y$,
  then $d_H(u,v)\leq d_G(x,y)$; If $x=y$ and $x$ is not an isolated vertex,
  then $d_H(u,v)\leq 2$.
\end{lemma}
\begin{proof}
  If $x=y$ and $x$ is not isolated, pick a vertex $z$ of graph $G$ which is
  adjacent to vertex $x$, and find a vertex $w\in H$ satisfying $(z,w)\in
  R$. Then $(w,u)\in E_H$ and similarly $(w,v)\in E_H$. So $d_H(u,v)\leq
  2$.

  If $x\neq y$, choose the shortest path $P=x,x_1,x_2,\dots, x_k,y$
  between $x$ and $y$, and find corresponding vertices
  $u_1,u_2,\dots,u_k\in H$ such that$(x_i,u_i)\in R$ for any $1\leq i\leq
  k-1$, it is easily seen that $(u,u_1)\in E_H$, $(u_i,u_{i+1})\in E_H$ and
  $(u_k,v)\in E_H$, then $d(u,v)\leq d(x,y)$.
\end{proof}

Hence we immediately get the following corollary about radius.

\begin{cor} \label{rad} Suppose $G\muls R=H$, $G$ and $H$ are connected
graphs, and $R$ has full domain, then $rad(H)\leq \max\{rad(G),2\}$.
\end{cor}
An analogous result holds for the diameters. In particular, if $G$
is not a complete graph, then $diam(G)\geq diam(G\muls R)$. As a result,
$k<l$ and $k\neq 1$ implies there is no relation from $P_k$ to $P_l$.
Also, as we state in the example section, $(P_1,P_2)$ is the only pair of paths
such that there is a relation from one to another and vice versa.

\label{subs:complete}

%The \emph{complement graph $\overline{H}$} of a simple graph $H$ has the
%same vertex set as $H$, and two vertices are connected in $\overline{H}$ if
%and only if they are not connected in $H$.
\subsubsection*{Complete graphs} 
Note that in this subsection we do not require that the domain of $R$ is
full.


\begin{pro}\label{prop:complete}

  Let $H$ be a simple graph. Then there exists a relation $R$ such that
  $K_k\muls R=H$ if and only if $H$ is a complete $m$-partite graph, where
  $m\leq k$.

\end{pro}

\begin{proof}
 We denote the vertices of $K_k$ by $1,\dots,k$.

 If $H$ is a complete $m$-partite graph, let $R=\{(i,u)\mid i=1,\dots,m,u\in U_i\}\}$, then
 for each $1\leq i\leq m$, all the vertices
  in $U_i$ are independent in $H$, and $u$ is adjacent to $v$ whenever
  $u\in U_i$ and $v\in U_j$ for distinct $i,j$. Hence it is easily
  seen that $K_k\muls R=H$.

   Conversely, if $K_k\muls R=H$, assume $\domain R=\{1,\dots,m\}$. We claim that $R$ is
  injective, otherwise $H$ would have loops. Thus $V_H$ is the disjoint union
  of $R(1),\dots,R(m)$. For any
  two distinct vertices $u,v$ in $R(i)$, $u$ and $v$ are independent in $H$,
  then $H$ is a $m$-partite graph.
  For distinct $i$ and $j$ every vertex in $R(i)$ are adjacent with every
  vertex in $R(j)$ whenever $R(i)\neq \emptyset$, which means $H$ is a complete $m$-partite graph.
\end{proof}


%\begin{pro}
%  Let $H$ be a simple graph. Then there exists a relation $R$ such that
%  $K_k\muls R=H$ if and only if $\overline{H}$ is the disjoint union
%  of at most $k$ complete graphs.
%\end{pro}

\subsubsection*{Subgraphs} \label{sect:subgraph}
Relations between graphs intuitively imply relations between local
subgraphs. In this section we make this concept more precise. Recall $N_G[x]$ was denoted to be
the \emph{closed neighbourhood}\index{closed neighbourhood} of $x$ in $G$ ($N_G[x]=N_G(x)\cup \{x\}$) and
$\overbar{N_G[x]}:= V_G\setminus N_G[x]$\index{$\overbar{N_G[x]}$} be the set of vertices that are
not adjacent (or identical) to $x$ in $G$. Furthermore,
$\overbar{G_x}:=G-N_G[x]$\index{$\overbar{G_x}$}, which is the induced subgraph of $G$
obtained by removing the closed neighbourhood of a vertex $x$.
Analogously, for a subset $S\subseteq V_G$, $\overbar S$ is the induced subgraph obtained by removing all vertices in $S$ and their neighbours.

Then we have the following result about relations between local subgraphs.



\begin{pro} Suppose $G\muls R=H$ and $(x,u)\in R$. Suppose there is no isolated vertex in $G$. If there is no loop in
  $x$, then $\overbar{G_x}\muls \widetilde{R} = \overbar{G_u}$ where
  $\widetilde{R}\subseteq \overbar{N_G[x]}\times\overbar{N_H[u]}$ is the
  restriction of $R$.
\end{pro}

\begin{proof}
  We claim that the pre-image of any vertex in $\overbar H_u$ is not
    in $N_G(x)$. Otherwise, there is a vertex $v\in \overbar H_u$ and a
    vertex $y\in N_G(x)$ such that $(y,v)\in R$; from $(x,u)\in R$ we deduce
    that $v$ and $u$ are adjacent, which contradicts to $v\in \overbar
    H_u$. Next we claim that there is no vertex in $\overbar H_u$ whose
    pre-image is $x$. Suppose $v\in \overbar H_u$ and $R^{-1}(v)=\{x\}$.
    Since $v$ is not isolated in $\overbar H_u$, there exists a
    vertex $v'$ which is adjacent with $v$ in $\overbar H_u$. Thus
    $R^{-1}(v')\cap N(x)\neq \emptyset$, a contradiction. Hence
    for any edge $(v,v')$ in $\overbar H_u$, we can find
    an edge $(y,y')$ in $\overbar G_x$ such that $(y,v),(y',v')\in
    R$. Thus $\overbar G_x\muls \widetilde{R}=\overbar{G_y}$.
\end{proof}

%$(x,u)\in R$
%\TODO{
%if the vertex $x$ is isolated and $x$ duplicated.
%1.1 $u$ is also isolated, $u$ has only one preimage. then there is an isolated vertex
%after deleting. may have problem(if $G$ have no other isolated vertex, eg. two isolated vertex
%to two isolated vertex)

%1.2 $u$ is also isolated, and $x$ contracts.
%may have problem.



%1. if the vertex $x$ is isolated and been duplicated,

%1.1. if $u$ has only one preimage on $G$, then after deleting, there is a isolated vertex in %$H$.

%1.2. if it has more than one preimages, no impact.
%}

\begin{example}
Let us see an example. Let $G$ and $H$ be graphs as Figure~\ref{fige5}.
For a relation from $G$ to $H$, we consider the pre-image of
vertex $u$, because the domain of $R$ is full, and the symmetry of $P_4$, at least
either $(1,u)\in R$ or $(2,u)\in R$ holds. If $(1, u)\in R$, from the
above theorem, we know that there is an induced relation from $P_2$ to
$P_4$, but it is impossible. If $(2,u)\in R$ holds, also from above
theorem, there is an induced relation from $P_1$ to $P_4$, which is impossible.

\begin{figure}[!ht]
\centering
\subfloat[$G$]{
%\label{fig:improved_subfig_a}
\begin{minipage}[c]{0.4\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{dupl1.eps}
\end{minipage}
}
\subfloat[$H$]{
%\label{fig:improved_subfig_b}
\begin{minipage}[c]{0.4\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{ex3.eps}
\end{minipage}
}
 \caption{There is no relation from $G$ to $H$.}
    \label{fige5}
\end{figure}
\end{example}


Note that from Corollary~\ref{rad}, the radius of $H$ is smaller than the radius of $G$, so there is no relation $R$ such that
$H\muls R=G$. Therefore there is neither a relation from $G$ to $H$, nor one from $H$ to $G$. Note that the two solutions can be different.



\begin{pro} \label{pro:subgraph}
  Suppose $G\muls R=H$ and $S$ and $D$ are subsets of $V_G$ and $V_H$,
  respectively, such that
  \begin{enumerate}
   \item $G[S] \muls R|_{(S\times D)}=H[D]$;
   \item $R|_{(S\times D)}$ has full domain on $S$;
   \item there is no isolated vertex in $\overbar D$.
  \end{enumerate}

  Then $\overbar S\muls\widetilde{R}=\overbar D$,
  where $\widetilde{R} = R|_{(\overbar S\times \overbar D)}$ is the
  corresponding restriction of $R$.
\end{pro}

\begin{proof}
  Obviously, $\overbar S\muls\widetilde{R}$ is an induced subgraph of $\overbar
  D$. We need to show the reverse inclusion. Given $u\in V_{\overbar{D}}$
  and $x\in R^{-1}(u)$, we first show that there are two possibilities:
  \begin{enumerate}
  \item $x$ is a vertex of $\overline{S}$.
  \item $x$ is an isolated vertex of $S$.
  \end{enumerate}
  Assume, to the contrary, $x$ is either a non-isolated vertex of $S$ or $x$ is in the
  neighbourhood of some vertex of $S$. In both cases there is $y\in S$
  connected by an edge to $x$. Consequently there is a vertex $v\in D$, such
  that $v\in R(y)$, and $v$ is connected by an edge to $u$. It follows
  $u\notin V_{\overbar{D}}$, a contradiction.

  Now consider an arbitrary edge $(u,v)\in E_{\overbar{D}}$. We have
  $(x,y)\in E_G$ such that $u\in R(x)$ and $v\in R(y)$.
  If any of $x$ and $y$, say $x$, is an isolated vertex in $S$, then $y$ is not in $S$.
  Thus $y$ is in the neighbourhood of $S$, which contradicts the two possibilities.
  So both $x$ and $y$ are not isolated in $S$, from the above deduction $x,y$ are in the case 1, i.e.,
  they are vertices of $\overline{S}$.
  Consequently $\overbar S\muls\widetilde{R}$ has precisely the same edges
  as $\overbar D$. Because $\overbar{D}$ has no isolated vertices and
  thus every vertex is an endpoint of some edge, we know that the vertex set
  of $\overbar S\muls\widetilde{R}$ is same as the vertex set of $\overbar D$. Hence
  $\overbar S\muls\widetilde{R}=\overbar D$.
\end{proof}
This result is of particular practical use in the special case where $S$
and $D$ consist of a single vertex. When looking for a relation $R$ such
that $G\muls R=H$ one can remove a vertex including its neighborhood from
$G$ as well as the prospective image including the neighborhood from $H$
and then solve the problem on the subgraphs.



\section{Relational equivalence}
\label{sect:retract}
Recall that in Section~\ref{sec:hom-equ} we define graphs $G$ and $H$ are \emph{homomorphism equivalent}\index{homomorphism equivalent} (or
\emph{hom-equivalent}\index{hom-equivalent}) if there exists homomorphisms $G\to H$ and $H\to
G$. It is well known that every equivalence class of the homomorphism order
contains a minimal representative that is unique up to isomorphism: the
\emph{graph core}\index{graph core}~\cite{Hell2004}.

We define similar equivalences implied by the existence of
(special) relations between graphs. In this section, we require all
relations to have full domain unless explicitly stated otherwise. With
this condition we will show that these equivalences produce a rich structure
closely related to but distinct from the structure of homomorphism
equivalences.

This may come as a surprise: the equivalence implied by the existence of
surjective homomorphisms is not interesting. Consider two graphs $G$ and
$H$ and suppose there are surjective homomorphisms $f:G\to H$ and $g:H\to
G$. Since every vertex in $V_G$ has at most one image under $f$, we have
$|V_G|\geq |V_H|$. Analogously $|V_H|\geq |V_G|$, and hence
$|V_G|=|V_H|$. Thus $f$ and $g$ are both bijective, and $G$ is isomorphic
to $H$.

\subsection*{Reversible relations} \label{revers}

\begin{definition}
  A relation $R$ is \emph{reversible with respect to a graph $G$}\index{reversible} if
  $(G\muls R)\muls R^+=G$.
\end{definition}

Recall that in Proposition~\ref{dec} we proved that $R$ can be decomposed.
Suppose $R=R_D\circ R_C$, where $R_D$ and $R_C$
are constructed as in the proof of Proposition~\ref{dec}. $R_C$ is a functional relation and $R_D$ is an injective
relation with full domain.
Then we can get the following result with respect to reversible relation.

\begin{pro} \label{reve}   
$R$ is reversible with respect to $G$ if and only if for every $\alpha$ and $\beta$
  satisfying $R_C(\alpha)=R_C(\beta)$ we have
  $N_{G\muls R_D}(\alpha)= N_{G\muls R_D}(\beta)$.
\end{pro}
\begin{proof}
  We set $G_1=G\muls R_D$, If $R_C(\alpha)=R_C(\beta)$ implies
  $N_{G_1}(\alpha)= N_{G_1}(\beta)$, then $H\muls R_C^+=G_1$.
  Therefore,
  \begin{align*}
     G\muls R\muls R^+ & = H\muls R^+ = H\muls (R_D\muls R_C)^+\\
                       & = H\muls R_C^+\muls R_D^+ = G_1\muls R_D^+ = G.
   \end{align*}

  The first equation is by assumption, the second is by Proposition~\ref{dec}, the third one
  is by the property of transpose, the fourth is from Lemma~\ref{lem:compo},
  the last equation is because $R_D$ is injective.
  Thus by definition, $R$ is reversible.

  Conversely, since $R$ is
  reversible, i.e., $H\muls R^+=G$, setting $G_2 = H\muls R_C^+$ gives
  $G_2\muls R_D^+=G$. Hence $G_1\muls R_C\muls R_C^+=G_2$ and $G_2\muls
  R_D^+\muls R_D=G_1$. From $I_{G_1}\subseteq R_C\muls R_C^+$ we conclude
  $G_1\subseteq G_2$, and similarly $I_{G_2}\subseteq R_D^+\muls R_D$ yields
  $G_1\supseteq G_2$. Hence $G_1=G_2$. $R_C^+$ is injective, hence
  $\alpha,\beta\in V_{G_2}=V_{G_1}$ has the same open neighbourhood whenever
  the pre-image of $\alpha$ and $\beta$ under $R_C^+$ coincide,
  i.e. $R_C(\alpha)=R_C(\beta)$.
\end{proof}

$R_D$ is an injective relation, hence one can easily get
$N_{G\muls R_D}(\alpha)=R_D(N_G(x))$ provided that $(x,\alpha)\in R_D$. On the
other hand, if we define $R$ to be the image of $R_D$ as in the proof of
Proposition~\ref{dec}, then $R_C(\alpha)=R_C(\beta)$ implies there are two
distinct vertices $x,y\in V_G$, s.t. $(x,u),(y,u)\in R$, where
$u=R_C(\alpha)=R_C(\beta)$, and verse visa. Using Proposition~\ref{reve}
we thus obtain
\begin{pro}
  A relation $R$ is reversible with respect to $G$ if and only if for every
  two vertices $x$ and $y$ such that $R(x)\cap R(y) \neq \emptyset$ we have
  $N_G(x)=N_G(y)$.
\end{pro}

\subsection*{Strong relational equivalence}

\begin{definition}
  Two graphs $G$ and $H$ are \emph{strongly relationally equivalent}\index{strong relationally equivalent}, denoted by $G
  \backsim_s H$\index{$\backsim_s$}, if there is a relation $R$ such that $G\muls R=H$ and
  $H\muls R^+=G$.
\end{definition}

\begin{lemma}
  Relational equivalence is an equivalent relation on graphs.
\end{lemma}
\begin{proof}
  By definition $\backsim_s$ is symmetric. Because $G\muls I_G=G$, relation
  $\backsim_s$ is reflexive. Suppose $G\backsim_s G'$ and $G'\backsim_s
  G''$. Thus there are relations $R$, $S$, such that
  $G'=G\muls R$, $G''=G'\muls S$, $G=G'\muls R^+$, and $G'=G''\muls S^+$. By
  the composition law (Lemma~\ref{lem:compo}) it follows that
  $G''=G\muls(R\circ S)$ and $G=G''\muls(S^+\circ R^+)=G''\muls(R\circ S)^+$, i.e, $G\backsim_s
  G''$. Hence $\backsim_s$ is transitive.
\end{proof}


Recall that the \emph{thinness relation}\index{thinness relation} $S$ of $G$ is the equivalent relation on
  $V_G$ defined by $(x,y)\in S$ if and only if $N_G(x)=N_G(y)$.
  We denote by $\mathcal{S}$ the corresponding partition of $V_G$, and write
  $R_S\subseteq V_G\times\mathcal{S}$ that associates each vertex with its
  $S$-equivalence class, i.e., $(x,\beta)\in R_S$ if and only if $x\in\beta$.
In this context it is well known that $G$ can
be reconstructed from $G_{pd}$ (the point-determining graph of $G$) and the knowledge of the $S$-equivalence
classes. In fact, we have
\begin{equation}
\label{eq:thin-1}
  G_{pd}\muls R^+_S=G.
\end{equation}




\begin{thm} \label{thm:equi}
  $G$ and $H$ are in the same equivalence class w.r.t.\ $\backsim_s$ if and
  only if their point-determining graphs are isomorphic.
\end{thm}
\begin{proof}
  Assume $G\backsim_s H$. From Equation(\ref{eq:thin-1}) we know that
  $G\backsim_s G_{pd}$, $H\backsim_s H_{pd}$, so $G_{pd}\backsim_s
  H_{pd}$.
  Now we claim that $G_{pd}$ and $H_{pd}$ are isomorphic.
  Suppose $G_{pd}\muls R=H_{pd}$, then the pre-image of $R$ is unique.
  Otherwise, there exist distinct vertices $x,y\in V_{G_{pd}}$ such that
  $R(x)=R(y)$, then $N_{G_{pd}}(x)=N_{G_{pd}}(y)$, contradicting
  thinness. Likewise, the pre-image of $R^{+}$ is unique, i.e., the image
  of $R$ is unique. Hence $R$ is one-to-one.
\end{proof}

\begin{figure}[!ht]
\centering
\subfloat[$G$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
 \includegraphics[height=0.7\textwidth]{ex3.1.1.eps}
\end{minipage}}
\subfloat[$H$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
 \includegraphics[height=0.7\textwidth]{ex3.1.2.eps}
\end{minipage}}
\subfloat[$G_{pd}=H_{pd}$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
 \includegraphics[height=0.7\textwidth]{ex3.1.3.eps}
\end{minipage}}
\caption{Non-isomorphic graphs $G$ and $H$ with isomorphic point-determining graphs.}
\label{fig:thin}
\end{figure}

%\begin{figure}
%\begin{center}
 % \begin{tabular}{ccc}
  %  \includegraphics[height=0.2\textwidth]{ex3.1.1.eps} &
   % \includegraphics[height=0.2\textwidth]{ex3.1.2.eps} &
    %\includegraphics[height=0.2\textwidth]{ex3.1.3.eps} \\
    %$G$ & $H$ & $G_{thin}=H_{thin}$\\
  %\end{tabular}
%\end{center}
%\caption{Non-isomorphic graphs $G$ and $H$ with isomorphic thin graphs.}
%\label{fig:thin}
%\end{figure}

The example in Fig.~\ref{fig:thin} shows that point-determining graphs can be isomorphic
while $G$ and $H$ themselves are not isomorphic. Relational equivalence
thus is coarser than graph isomorphism (surjective homomorphic equivalence)
but stronger than homomorphic equivalence.

\subsection*{Weak relational equivalence} \label{sec:weakeq}

\begin{definition}
  Two graphs $G$ and $H$ are \emph{(weak) relationally equivalent}\index{weak relationally equivalent, relationally equivalent}, denoted by $G
  \backsim_w H$\index{$\backsim_w$}, if there are relations $R$ and $S$ such that $G\muls R=H$
  and $H\muls S=G$.
\end{definition}

Note that $\backsim_w$ is the same as $\Releq$ in Chapter~\ref{Ch:order}.


\begin{lemma}
  Weak relational equivalence is an equivalent relation on graphs.
\end{lemma}
\begin{proof}
  By definition $\backsim_w$ is symmetric. Because $G\muls I_G=G$, relation
  $\backsim_w$ is reflexive. Suppose $G\backsim_w G'$ and $G'\backsim_w
  G''$. Thus there are relations $R$, $S$, $R'$, and $S'$, such that
  $G'=G\muls R$, $G''=G'\muls R'$, $G=G'\muls S$, and $G'=G''\muls S'$. By
  the composition law (Lemma~\ref{lem:compo}) it follows that
  $G''=G\muls(R\circ R')$ and $G=G''\muls(S'\circ S)$, i.e, $G\backsim_w
  G''$. Hence $\backsim_w$ is transitive.
\end{proof}

Strong relational equivalence implies weak relational equivalence. To see
this, simply observe that the definition of the weak form is obtained from
the strong one by setting $S=R^+$.

\begin{figure}[!ht]
\centering
\subfloat[$G$]{\label{figa:weak}
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{weak_nonstrong.eps}
\end{minipage}}
\subfloat[$H$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{weak_nonstrong2.eps}
\end{minipage}}
\caption{$G$ and $H$ are weakly relationally equivalent but have
  non-isomorphic  graphs.}
\label{fig:weak}
\end{figure}


%\begin{figure}[!ht]
%\begin{center}
 % \begin{tabular}{ccc}
  %  \includegraphics[height=0.25\textwidth]{weak_nonstrong.eps} &\qquad
   % \includegraphics[height=0.25\textwidth]{weak_nonstrong2.eps}\\
    %    $G$ & \qquad $H$ 
  %\end{tabular}
%\end{center}
%\caption{$G$ and $H$ are weakly relationally equivalent but have
 % non-isomorphic thin graphs.}
%\label{fig:weak}
%\end{figure}

The converse is not true, as shown by the graphs $G$ and $H$ in
Fig.~\ref{fig:weak}: It is easy to see that their point-determining graphs are different
and thus $G$ and $H$ are not strongly relationally equivalent. However,
they are relationally equivalent. To get relation from $G$ to $H$ contract
vertices 2 and 3 and keep other vertices on place, i.e.,
$$R=\{(1,1),(2,2),(3,2),(4,4),(5,5),(6,6),(7,7)\}.$$ To get relation
from $H$ to $G$, duplicate 5 and 7 and contract them together to 3,
$$S=\{(1,1),(2,2),(4,4),(5,5),(6,6),(7,7),(5,3),(7,3)\}.$$
Consequently, weak relational equivalence is coarser than strong relational
equivalence.

\subsection*{R-cores}
\label{subsec:R-core}

A graph is an \emph{R-core}\index{R-core}, if it is the minimal graph (in the number of
vertices) in its equivalence class of $\backsim_w$.

This notion is analogous to the definition of graph cores. In this section
we show properties of R-cores that are similar to the properties of graph
cores. To this end we first need to develop a simple characterization of
R-cores.

Again we start from a decomposition of relations. Consider a relation
$R$ such that $G\muls R = H$. We seek for pair of relations $R_1$ and
$R_2$ such that $R=R_1\circ R_2$. In contrast to Lemma~\ref{dec}, however,
we now look for a decomposition so that the graph $G'=G\muls R_1$ is
smaller (in the number of vertices) than $G$.
%\begin{equation}
%\xymatrix{
%G \ar[dr]_{R_1}  \ar@{->}[rr]^{R=R_1\circ R_2} & & H \\
%  & G' \ar[ur]_{R_2} &
%}
%\end{equation}
  \begin{figure}[!ht]
  \centering
  \includegraphics[width=0.25\textwidth]{comum.eps} 
\caption{Communted diagram.}
\label{fig:comum2}
\end{figure}   

The existence of such a decomposition follows from a translation of
the well-known Hall Marriage Theorem~\cite{Schrijver2003} to the language of
relations. We say that the relation $R\subseteq A\times B$ satisfies the
\emph{Hall condition}, if for every $S\subseteq A$ we have $|S|\leq |R(S)|$.

We have already proved Hall's marriage theorem in~\ref{thm:hallo}. Here we restate it in terms of relations.

\begin{thm}[Hall's marriage theorem] \label{thm:hall}
  If $G\muls R = H$ and $R$ satisfies the Hall condition, then $R$
  contains a monomorphism $f:G\rightarrow H$.
\end{thm}


\begin{lemma} \label{lem:nohall} If $G\muls R = H$ and relation $R$ does
  not satisfy the Hall condition, then there are relations $R_1$ and $R_2$
  such that $R=R_1\circ R_2$, and the number of vertices of graph
  $G'=G\muls R_1$ is strictly smaller than the number of vertices of $G$.
\end{lemma}
\begin{proof}
  Without loss of generality assume that $V_G\cap V_H=\emptyset$. If $R$
  does not satisfy the Hall condition, then there exists a vertex set $S\subset
  V_G$ such that $|S|>|R(S)|$. Now we define relations $R_1$ and $R_2$ as
  follows:
  \begin{equation*}
    R_1(x)=
    \begin{cases} R(x) \text{   for $x\in S$,}\\
      x \text{   otherwise,}
    \end{cases}
\qquad\qquad\qquad
    R_2(x)=
    \begin{cases} x \text{   for $x\in R(S)$,}\\
      R(x) \text{   otherwise.}
    \end{cases}
  \end{equation*}
Obviously $R_1\circ R_2 = R$ and $|V_{G'}|=|V_G|-(|S|-|R(S)|)<|V_G|$.
\end{proof}

This immediately gives a necessary, but in general not sufficient,
condition for a graph to be an R-core.

\begin{cor}\label{cor:nohall2}
  If $G$ is an R-core, then every relation $R$ such that $G\muls R=G$
  satisfies the Hall condition and thus contains a monomorphism.
\end{cor}
\begin{proof}
  Assume that there is a relation $R$ that does not satisfy the Hall
  condition. Then there is a graph $G'$, $|V_{G'}|<|V_G|$, and relations
  $R_1$ and $R_2$ such that $G\muls R_1=G'$ and $G'\muls
  R_2=G$. Consequently $G'$ is a smaller representative of the equivalence
  class of $\backsim_w$, a contradiction with $G$ being R-core.
\end{proof}

To see that the condition of Corollary~\ref{cor:nohall2} is not sufficient,
consider a graph $G$ consisting of two independent vertices. It is not an R-core,
because it can retract to an isolated vertex. However, the relation is required
to be full, any relation from $G$ to itself satisfies the Hall condition.

Next we show that R-cores are, up to isomorphism, unique representatives of
the equivalence classes of $\backsim_w$.


  \begin{figure}[!ht]
  \centering
  \includegraphics[width=0.35\textwidth]{rcore.eps} 
\caption{Construction of an embedding from $G_\text{R-core}$ to $G$.}
\label{fig:rcore}
\end{figure}   

\begin{pro}\label{pro:iso}
  If both $G$ and $H$ are R-cores in the same equivalence class of
  $\backsim_w$, then $G$ and $H$ are isomorphic.
\end{pro}

\begin{proof}
  Because both $G$ and $H$ are R-cores, we know that $|V_G|=|V_H|$.

  Consider relations $R_1$ and $R_2$ such that $G\muls R_1=H$ and $H\muls
  R_2=G$. Applying Lemma~\ref{lem:nohall} we know that $R_1$ satisfies the
  Hall condition. Otherwise there would be a graph $G'$ with $|V_{G'}|<
  |V_G|$ so that $G'$ is relationally equivalent to both $G$ and $H$
  which contradicts the fact that $G$ and $H$ are R-cores. Similarly, we can
  show that $R_2$ also satisfies the Hall condition.

  From Theorem~\ref{thm:hall} we know that there is a monomorphism $f$ from
  $G$ to $H$, and monomorphism $g$ from $H$ to $G$. It follows that number
  of edges of $G$ is not larger than the number of edges of $H$ and
  vice versa. Because $G$ and $H$ have the same number of edges and
  same number of vertices, $G$ and $H$ must be isomorphisms.
\end{proof}

It thus makes sense to define a construction analogous to the core of a graph.
\begin{definition}
  $H$ is an \emph{R-core of a graph $G$}\index{R-core} if $H$ is an R-core and $H\backsim_w
  G$.
\end{definition}

All R-cores of graph $G$ are isomorphic as an immediate consequence of
Proposition~\ref{pro:iso}. We denote the (up to isomorphism) unique R-core
of graph $G$ by $G_{\text{R-core}}$\index{$G_{\text{R-core}}$}..

\begin{lemma}
  $G_{\text{R-core}}$ is isomorphic to a (not necessarily induced) subgraph
  of $G$.
\end{lemma}

\begin{proof}
  Take any relation $R$ such that $G_{\text{R-core}}\muls R=G$. By the same
  argument as in Corollary~\ref{cor:nohall2}, there is a monomorphism
  $f:G_{\text{R-core}}\rightarrow G$ contained in $R$. Consider the image
  of $f$ on $G$.
\end{proof}

\begin{thm}
  \label{thm:Rcore}
  $G_{\text{R-core}}$ is isomorphic to an induced subgraph of $G$.
\end{thm}

\begin{proof}
%  We firstly prove that $G_{\text{R-core}}$ is isomorphic to a subgraph of $G$, i.e.,
%  there exists a mapping which maps every edge of $G_{\text{R-core}}$ to an edge of
%  $G$. We construct this mapping as follows:
  Fix $R_1$ and $R_2$ such that $G_{\text{R-core}}\muls R_1=G$ and
  $G\muls R_2=G_{\text{R-core}}$.

  $R=R_1\circ R_2$ is a relation such that $G_{\text{R-core}}\muls
  R=G_{\text{R-core}}$. By Corollary~\ref{cor:nohall2}, $R$ contains a
  monomorphism $f:G_{\text{R-core}}\rightarrow G_{\text{R-core}}$. Because
  such a monomorphism is a permutation, there exists an $n$ such that $f^n$ is
  identity.

  Put $R_1'=R^{n-1}\circ R_1$. Because $R^{n}$ contains the identity and
  $R^{n}=R_1'\circ R_2$, it follows that for every
  $x\in V_{G_{\text{R-core}}}$, there is a vertex
  $I(x)\in V_G$ such that $I(x)\in R'_1(x)$ and $x\in R_2(I(x))$.
  In other words, $(x,I(x))\in R'_1(x)$ and $(I(x),x)\in R_2$.
  It is easily seen that $I$ is a mapping from vertex set of $G_{\text{R-core}}$
  to vertex set of $G$. We take the induced subgraph of $G$ induced by the image of $I$,
  denoted by $G'$, and claim that $I$ is an isomorphism of $G_{\text{R-core}}$ to $G'$.

  We first show that for two vertices $x\neq y$, we have $I(x)\neq I(y)$ and
  thus $I$ is vertex injective (thus both vertex and edge injective). Assume, to the contrary, that there are two vertices $x\neq y$ such that $I(x)=I(y)$.
  Consider an arbitrary vertex $z$ in the neighbourhood of $x$. It follows
  that $I(z)$ must be in the neighbourhood of $I(x)$ and consequently
  $z$ is in the neighbourhood of $y$. Thus the neighbourhoods of $x$ and $y$
  are the same. By Theorem~\ref{thm:equi}, however, we know that the
  R-core is a point-determining graph (because weak relational equivalence is coarser
  than strong relational equivalence), a contradiction.

  Then we claim that, $I$ is a homomorphism of $G_{\text{R-core}}$ to $G'$, i.e.,
  for every edge $(x,y)\in E_{G_{\text{R-core}}}$ we also have edge
  $(I(x),I(y))\in E_G$. This is because $I\subset R'_1$, then
  $G_{\text{R-core}}=G_{\text{R-core}}\muls I\subset G_{\text{R-core}}\muls R'_1=G$.
%  Hence we proved that $G_{\text{R-core}}$ is isomorphic to a subgraph of $G$.

  By the construction, $I$ is vertex surjective.
  Finally we prove that $I$ is also a edge surjective homomorphism by claiming
  $I^{-1}$ is a homomorphism of $G'$ to $G_{\text{R-core}}$.
  We see $I^{-1}\subset R_2$ by observing $x \in R_2(I(x))$ implies $(I(x),x)\in R_2$ for all $x\in$
  vertex set of $G_{\text{R-core}}$. Because $I$ as well as $I^{-1}$ is one-to-one,
  $G'=G'\muls I^{-1}\subset G'\muls R_2=G_{\text{R-core}}$.
  $(I(x),I(y))\in G'$ corresponds to an edge $(x,y)\in
  G_{\text{R-core}}$.

  Hence we proved $I$ is bijective (both edge and vertex) homomorphism, thus $I$ is an isomorphism.
\end{proof}

We close the section with an algorithm for computing the R-core of a graph. In
contrast to graph cores, where the computation is known to be NP-complete,
there is a simple polynomial algorithm for R-cores.

Observe that the R-core of a graph containing isolated vertices is isomorphic
to the disjoint union of the R-core of the same graph with the isolated
vertices removed and a single isolated vertex. The R-core of a graph without
isolated vertices can be computed by Algorithm~\ref{alg:Rcore}.

\begin{algorithm}[htb]
\caption{The R-core of a graph}
\label{alg:Rcore}
%\newcommand{\AND}{ $\wedge$ }
\begin{algorithmic}[1]
  \REQUIRE ~~\newline
  Graph $G$ with loops allowed and without isolated vertices,
  vertex set denoted by $V$, neighbourhoods $N_G(i)$, $i\in V$.
  \FOR {$i\in V$}
  \STATE $W(i)= \emptyset$
  \STATE found = FALSE
  \FOR {$j\in V\setminus \{i\}$}
  \IF {$N(j)\subseteq N(i)$}
  \STATE  $W(i):= W(i)\cup N(j)$
  \ENDIF
  \IF {$N(i)\subseteq N(j)$}
  \STATE found = TRUE
  \ENDIF
  \ENDFOR
  \IF {$W(i)=N(i)$ \AND found}
  \STATE delete $i$ from $V$
  \STATE $N(i)= \emptyset$
  \ENDIF
  \ENDFOR
\RETURN  The R-core $G[V]$ of $G$.

\end{algorithmic}
\end{algorithm}

The algorithm removes all vertices $v\in G$ such that (1) the neighborhood
of $v$ is union of the neighbourhood of some other vertices $v_1,v_2,\dots, v_n$
and (2) there is vertex $u$ such that $N_G(v)\subseteq N_G(u)$.

It is easy to see that the resulting graph $H$ is relationally equivalent
to $G$. Condition (1) ensures the existence of a relation $R_1$ such that
$H\muls R_1=G$, while condition (2) ensures the existence of a relation
$R_2$ such that $G\muls R_2=H$.

We need to show that $H$ is isomorphic to $G_{\text{R-core}}$. By Theorem
\ref{thm:Rcore} we can assume that $G_{\text{R-core}}$ is an induced
subgraph of $H$ that is constructed as an induced subgraph of $G$.

We also know that there are relations $R_1$ and $R_2$ such that
$G_{\text{R-core}}\muls R_1=H$ and $G\muls R_2=G_{\text{R-core}}$. By the
same argument as in the proof of Theorem~\ref{thm:Rcore} we can assume both
$R_1$ and $R_2$ to contain an (restriction of) identity.

Now assume that there is a vertex $v\in V_H\setminus
V_{G_{\text{R-core}}}$. We can put $u=R_2(v)$ and because $R_2$ contains an
identity we have $N_G(v)\subseteq N_G(u)$. We can also put
$\{v_1,v_2\ldots v_n\}$ to be the set of all vertices such that $v\in
R_1(v_i)$. It follows that the neighbourhood of $v$ is the union of
the neighbourhoods of $v_1,v_2,\ldots, v_n$ and by the construction of $H$ we have $v\notin
V_H$, a contradiction.


\section{The partial order Rel\texorpdfstring{$(G,H)$}{Rel(G,H)}}
\label{sect:poset}

\subsection*{Basic properties}

For fixed graphs $G$ and $H$ we consider the partial order $\mathrm{Rel}(G,H)$.
The vertices of this partial order are all relations $R$ such
that $G\muls R=H$. We put $R_1\leq R_2$ if and only if $R_1\subseteq R_2$.

This definition is motivated by Hom-complexes, see~\cite{Matousek2003}. In
this section we show the basic properties of this partial order and
concentrate on minimal elements in the special case of $\mathrm{Rel}(G,G)$.

\begin{pro}
  Suppose $G\muls R'=H$, $G\muls R''=H$ and $R'\subseteq R''$, then any
  relation $R$ with $R'\subseteq R\subseteq R''$ also satisfies $G\muls
  R=H$.
\end{pro}
\begin{proof}
  From $R'\subseteq R\subseteq R''$ we conclude $G\muls R'\subseteq G\muls
  R\subseteq G\muls R''$. Hence $G\muls R'=G\muls R''$ implies $G\muls
  R=H$.
\end{proof}

Hence it is possible to describe the partial order $\mathrm{Rel}(G,H)$ by
listing minimal and maximal solutions $R$ of $G\muls R=H$ w.r.t.\ set
inclusion.

For example, if $G$ is $P_3$ with vertices $v_0,v_1,v_2,v_3$ and $H$ is
$P_1$ with vertices $x_0,x_1$, it is easily seen that
$R''=\{(v_0,x_0),(v_2,x_0),(v_1,x_1),(v_3,x_1)\}$ is a maximal solution of
$G\muls R=H$ and $R'=\{(v_0,x_0),(v_1,x_1)\}$ is a minimal solution,
because $R'\subset R''$, then all the relations $R$ with $R'\subseteq
R\subseteq R''$ satisfy $G\muls R=H$. We note that minimal and maximal
solutions need not be unique.


\subsection*{Solutions of \texorpdfstring{$G\muls R = G$}{G* R = G}}


For simplicity, we say that a relation $R$ is an \emph{automorphism}\index{automorphism} of $G$
if it is of the form $R=\{(x,f(x))\mid x\in V_G\}$ and $f:V_G\to V_G$
is an automorphism of $G$.


We will see that conditions related to thinness again play a major role in
this context. Recall that $G$ is point-determining if no two vertices have the same
neighborhood, in other words, $N_G(x)=N_G(y)$ implies $x=y$. Here we need an even
stronger condition:
\begin{definition}
  A graph $G$ satisfies \emph{condition N}\index{condition N} if $N_G(x)\subseteq N_G(y)$
  implies $x= y$.
\end{definition}
In particular, graphs satisfying condition N are point-determining.

\begin{pro}
  For a given graph $G$, the set $\mathrm{Rel}(G,G)$ of all relations
  satisfying $G\muls R = G$ forms a monoid.
\end{pro}
\begin{proof}
  Firstly, $R,S\in \mathrm{Rel}(G,G)$ implies $G\muls R=G$ and
  $G\muls S=G$ and thus $G\muls (R\circ S)=G$, so that $R\circ S\in
  \mathrm{Rel}(G,G)$. Furthermore, for any $R,S,T\in \mathrm{Rel}(G,G)$ we have $(R\circ S)\circ T=R\circ(S\circ T)$.
Finally, the identity relation $I_G$ is a left and right
  identity for relational composition: $I_G\circ R=R\circ I_G=R$.
\end{proof}

A relation $R\subset V_G\times V_G$ can be interpreted as a directed graph
$\vec R$ with vertex set $V_G$ and a directed edge $u\rightarrow v$ if and
only if $(u,v)\in R$. Note that $\vec R$ may have loops. We say that $v\in
V_G$ is \emph{recurrent}\index{recurrent} if and only if there exists a walk (of length at
least 1) from $v$ to itself. Let $S_G$ be the set of all the recurrent
vertices. Furthermore, we define an equivalent relation $\xi$ on $S_G$ by
setting $(u,v)\in\xi$ if there are both a walk in $\vec R$ from $u$ to $v$
and from $v$ to $u$. The equivalence classes w.r.t.\ $\xi$ are denoted by
$\vec R/\xi=\{D_1,D_2,\dots,D_m\}$. We furthermore define a binary
relation $\geq$ over $\vec R/\xi$ as follows: if there is a walk from a
vertex $u$ in $D_i$ to a vertex $v$ in $D_j$, then we say $u\geq v$. It is
easily seen that $\geq$ is reflexive, antisymmetric, and transitive, hence
$(\vec R/\xi,\geq)$ is a partially ordered set. W.l.o.g.\ we can assume
$\{D_1, D_2,\dots,D_s\}$ are the maximal elements w.r.t.\ $\geq$. Now let
$G_r=G[D_1\cup\dots\cup D_s]$ be the subgraph of $G$ induced by these
maximal elements.

\begin{lemma}\label{lem:aut1}
For arbitrary $x\in V_G$, there exist an $l\in \mathbb{N}$ and a
recurrent vertex $v$ such that $(v,x)\in R^l$, where $R^l$ is $l$-times
composition of relation $R$.
\end{lemma}
\begin{proof}
Set $x_0=x$ and choose $x_i\in R^{-1}(x_{i-1})$ for all $i\ge1$. Since
$|V_G|<\infty$, there are indices  $j,k\in \mathbb{N}$, $j<k$,
$x_j=x_k$. Then $x_j$ is a recurrent vertex. The lemma follows by setting
$l=j$ and $v=x_i$.
\end{proof}

\begin{lemma}\label{lem:aut2}
For every $v\in V_{G_r}$, $R^{-1}(v)\subseteq V_{G_r}$.
\end{lemma}
\begin{proof}
  We prove this by two steps:

  First, we claim that for any $x\in R^{-1}(v)$, $x$ is recurrent.
  Suppose $x\in R^{-1}(v)$ is not recurrent. Lemma~\ref{lem:aut1} implies
  that there is an $l\in \mathbb{N}$ and a recurrent vertex $w$ such that
  $(w,x)\in R^l$. Hence the definitions of $E$ and $\geq$ imply $[w]\geq
  [v]$, where $[v]$\index{$[v]$} denotes the equivalence class (w.r.t.\ $E$) containing
  the vertex $v$. Since $[v]$ is maximal w.r.t.\ $\geq$, we have
  $[v]=[w]$. Consequently, there exists an index $k\in \mathbb{N}$ such
  that $(v,w)\in R^k$. On the other hand, we have $(x,x)=(x,v)\circ
  (v,w)\circ (w,x)\in R^{k+l+1}$. Thus, $x$ is recurrent, a contradiction.
  Therefore, every vertex $x\in R^{-1}(v)$ is recurrent.

  Second, we prove $x$ is a maximal element in the partial order.
  Hence $[x]\geq
  [v]$ together with the maximality of $[v]$ gives $[x]=[v]$, and thus
  $x\in V_{G_r}$.
\end{proof}

\begin{lemma}\label{lem:aut3}
  For every $x\in V_G$, there is $l\in \mathbb{N}$ such that, for arbitrary
  $i\geq l$, there exists $u\in V_{G_r}$ satisfying $(u,x)\in R^i$.
\end{lemma}

\begin{proof}
  From Lemma~\ref{lem:aut1} and Lemma~\ref{lem:aut2} we conclude that it is
  sufficient to show that for an arbitrary recurrent vertex $v$ there is a
  $k\in \mathbb{N}$ and $w\in V_{G_r}$ such that $(w,v)\in R^k$. The lemma
  now follows easily from the finiteness of $V_G$.
\end{proof}


Now we introduce a lemma which connects relation $R$ and the neighborhood of vertex in a graph.
The lemma is simple but very useful.
\begin{lemma}\label{lem:aut4}
 Suppose $G\muls R = H$. For any $u,v\in V_H$, if $R^{-1}(u)\subseteq R^{-1}(v)$, then $N_H(u)\subseteq N_H(v)$.
\end{lemma}

\begin{proof} 
 Suppose there exist $u,v\in V_H$, $R_{-1}(u)\subseteq R_{-1}(v)$ but $N_H(u)\nsubseteq N_H(v)$,
 then there exist a vertex $w$ of $H$, $w\in N_H(u)$ but $w\notin N_H(v)$. Because $(u,w)$ is an edge
 in $H$ and $G\muls R = H$, we can find $x,y\in V_G$ such that $x\in R_{-1}(w), y\in R_{-1}(u)$ and $(x,y)$ is an edge in $G$.
 $R_{-1}(u)\subseteq R_{-1}(v)$ implies $y\in R_{-1}(v)$. We already have $(x,w)\in R$ and $(x,y)$ is an edge in $G$,
 by the definition of $\muls$ we have $(v,w)$ is an edge of $H$, which contradicts to $w\notin N_H(v)$.
\end{proof}

%we need to change the prove for using the lemma.


From these lemmata we can deduce:
\begin{thm} \label{thm:auto1}
All solutions of $G\muls R=G$ are
automorphisms if and only if $G$ has property N.
\end{thm}
\begin{proof}
  Suppose there are distinct vertices $x,y\in V_G$ such that $N_G(x)\subseteq
  N_G(y)$. Then $R=I_G\cup(x,y)$, which is not functional, satisfies $G\muls
  R=G$. Thus $G\muls R=G$ is also solved by relations that are not
  automorphisms of $G$. This proves the `only if' part.

  Conversely, suppose $G$ has property N. \textbf{Claim:} There is a
  $k\in\mathbb{N}$ such that $R^k\cap (V_{G_r}\times V_{G_r})=I_{G_r}$.

  For each $v_i\in V_{G_r}$ there is a walk of length $s_i\ge1$ from $v_i$
  to itself. Hence $(v_i,v_i)\in R^{s_i}$. Let $s$ be the least common
  multiple of all the $s_i$. Then $(v_i,v_i)\in R^s$ for all $v_i\in V_{G_r}$.
  Define $Q:=R^s\cap(V_{G_r}\times V_{G_r})$. Thus $I_{G_r}\subseteq Q$ and
  moreover $Q^j\subseteq Q^{j+1}$ for all $j\in\mathbb{N}$. Since $V_{G_r}$
  is finite, there is an $n\in\mathbb{N}$ such that $Q^{n+1}=Q^{n}$, and
  hence $Q^{2n}=Q^n$. Let us write $R^{-i}(v):=\{u\in V_G\mid (u,v)\in
  R^i\}$. For $v\in V_{G_r}$ we have $R^{-i}(v)\subset V_{G_r}$ (from Lemma~\ref{lem:aut2}) and hence $Q^{-n}(v)=R^{-sn}(v)$ for all $v\in V_{G_r}$.
  If $Q^n\neq I_{G_r}$, then there are two distinct vertices $u,v\in
  V_{G_r}$, such that $(u,v)\in Q^n$. From Lemma~\ref{lem:aut4} $N_G(u)\nsubseteq N_G(v)$ and $G=G\muls
  R^{sn}$ allow us to conclude that $R^{-sn}(u)\nsubseteq R^{-sn}(v)$ and
  $R^{-sn}(v)\nsubseteq R^{-sn}(u)$. Hence, there is a vertex $w$, such
  that $(w,u)\in Q^n$ and $(w,v)\notin Q^n$. From $(u,v)\in Q^n$ and
  $(w,u)\in Q^n$ we conclude $(w,v)\in Q^n\circ Q^n=Q^{2n}$, contradicting
  to $Q^{2n}=Q^n$. Therefore $Q^n=I_{G_r}$. Setting $k=sn$ now implies the
  claim.

  Finally, we show $V_{G_r}=V_G$. For any $v\in V_G\setminus V_{G_r}$,
  Lemma~\ref{lem:aut3} implies the existence of $w\in V_{G_r}$ and $m\in
  \mathbb{N}$ such that $(w,v)\in R^{mk}$. However, we have claimed
  $R^{-k}(w)=\{w\}$, hence $R^{-mk}(w)=\{w\}$. From Lemma~\ref{lem:aut4}, this, however, implies
  $N_G(w)\subseteq N_G(v)$ and thus contradicts property N. Therefore,
  $V_G=V_{G_r}$ and moreover $R^k=I_G$. This $R$ is an automorphism.
\end{proof}

\section{R-Retractions}
\label{sect:retraction}

Recall that an important special case of ordinary graph homomorphisms are
homomorphisms to subgraphs, and in particular so-called retractions: Let
$H$ be a subgraph of $G$, a \emph{retraction}\index{retraction} of $G$ to $H$ is a
homomorphism $r: V_G\rightarrow V_H$ such that $r(x)=x$ for all $x\in
V_H$.

We introduced the graph cores in Section~\ref{sect:retract} as minimal
representatives of the homomorphism equivalence classes. The classical and
equivalent definition is the following: A \emph{(graph) core}\index{core} is a graph
that does not retract to a proper subgraph. Every graph $G$ has a unique
core $H$ (up to isomorphism), hence one can speak of $H$ as \emph{the core
  of}\index{the core} $G$, see~\cite{Hell2004}.

Here, we introduce a similar concept based on relations between graphs.
Again to obtain a structure related to graph homomorphisms, in this section
we require all relations to have full domain unless explicitly stated
otherwise.

\begin{definition}
  Let $H$ be a subgraph of $G$. An \emph{R-retraction}\index{R-retraction} of $G$ to $H$ is a
  relation $R$ such that $G\muls R=H$ and $(x,x)\in R$ for all $x\in
  V_H$. If there is an R-retraction of $G$ to $H$ we say that $H$ is a
  \emph{retract}\index{retract} of $G$.
\end{definition}

\begin{lemma}\label{lem:ret}
  If $H$ is an R-retract of $G$ and $K$ is an R-retract of $H$, then $K$ is
  an R-retract of $G$.
\end{lemma}

\begin{proof}
  Suppose $T$ is an R-retraction of $H$ to $K$ and $S$ is an
  R-retraction of $G$ to $H$. Then $(G\muls S)\muls T=G\muls (S\circ
  T)=K$. Furthermore $(x,x)\in T$ for all $x\in V_K\subseteq V_H$, and
  $(u,u)\in S$ for all $u\in V_H$, hence $(x,x)\in S\circ T$ for all $x\in
  V_k$. Therefore $S\circ T$ is an R-retraction from $G$ to $K$.
\end{proof}

Hence, the following definition is meaningful.
\begin{definition}
  A graph is \emph{R-reduced}\index{R-reduced} if there is no R-retraction to a proper
  subgraph.
\end{definition}
Thus, we can also speak about `the R-reduced graph of a graph $G$' as the
smallest subgraph on which it can be retracted. We will see below that the
R-reduced graph of a graph is always unique up to isomorphism.

We remark that R-reduced graphs differ from R-cores introduced
in Section~\ref{sect:retract}, thus we chose an alternative name used
also in homomorphism setting (cores are also called reduced graphs).

\begin{lemma}
  Let $G$ be a graph with loops and $o$ a vertex of $G$ with a loop on
  it. Then the R-reduced graph of $G$ is the subgraph induced by $\{o\}$.
\end{lemma}

\begin{proof}
  Let $O$ be the graph induced by $\{o\}$, and $R=\{(x,o)\mid x\in V_G\}$, then
  it is easily seen $R$ is an R-retraction of $G$ to $O$. Moreover, since
  $O$ has only one vertex, there is no R-retraction to its
  subgraphs. So $O$ is an R-reduced graph of $G$.

  Conversely, let $H$ be an R-reduced graph of $G$ and denote by $R$ the
  R-retraction from $G$ to $H$. Then a loop of $G$ must generate a loop of
  $H$ via $R$, denote it by $O$\index{$O$}. Similarly to above, we see $O$ is an
  R-retract of $H$, hence it is also an R-retract of $G$ (by Lemma~\ref{lem:ret}).
  Therefore the definition of R-reduced graph implies
  $H=O$.
\end{proof}

In the remainder of this section, therefore, we will only consider graphs
without loops.

\begin{lemma} \label{lem:core}
  If $G$ is R-reduced, then $G$ has property N.
\end{lemma}
\begin{proof}
  Suppose there are two distinct vertices $x,y\in V_G$ with $N_G(x)\subseteq
  N_G(y)$ and consider the induced graph $G/x:=G[V_G\setminus\{x\}]$ obtained
  from $G$ by deleting the vertex $x$ and all edges incident with $x$. The
  relation $R=\left\{(z,z)\mid z\in V_G\setminus\{x\}\right\}\cup\{(x,y)\}$
  satisfies $G\muls R=G/x$: the first part is the identity on $G/x$ and
  already generates all necessary edges in $G/x$. The second part
  transforms edges of the form $(x,z)\in E_G$ to edges $(y,z)$. Since $R$
  has full domain and contains the identity relation restricted to
  $G/x$, it is an R-retraction of graph $G$, and hence $G$ is not R-reduced.
\end{proof}

\begin{pro} \label{pro:core}
  A graph $G$ is R-reduced if and only if it has no relation to a proper
  subgraph.
\end{pro}

\begin{proof}
  The `if' part is trivial. Now we suppose that $H$ is a proper induced
  subgraph of graph $G$ with the minimal number of vertices such that there
  is a relation $R$ satisfying $G\muls R=H$. Then $H$ does not have a
  relation to a proper subgraph of itself. We claim that $H$ has property
  N; otherwise, one can find a vertex $u\in V_H$ and construct a retraction
  from $H$ to $H/{u}$ as in Lemma~\ref{lem:core}, which causes a
  contradiction. Denote $\widetilde{R}=R\cap (V_H\times V_H)$, then
  $K=H\muls\widetilde{R}$ is a subgraph of $H$. From our assumptions on $H$ we
  obtain $K=H$. By virtue of Theorem~\ref{thm:auto1}, $\widetilde{R}$ is
  induced by an automorphism of $H$. Hence $R\circ \widetilde{R}^{+}$ is again
  a relation of $G$ to $H$ that contains the identity on $H$, i.e., it is
  an R-retraction.
\end{proof}

Since graph cores are induced subgraphs and retractions are surjective they
also imply relations. Proposition~\ref{pro:core} is also a consequence of
this fact. We refer to~\cite{Hell2004} for a formal proof.

\begin{figure}[!ht]
\centering
   \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{core.eps} \\
    \hspace{0.85cm}   $G$ \hspace{4cm} $G_\text{core}$
    \end{tabular}
\caption{A graph $G$ and its core.}
\label{fig:core}
\end{figure}

We call $R$ an \emph{minimal R-retraction}\index{minimal R-retraction} if there is no
R-retraction $R'$ such that $R\supset R'\supset I_H$.

\begin{lemma} \label{fun}
  Let $H$ be an R-retract of $G$. Then any minimal
  R-retraction of $G$ to $H$ is functional.
\end{lemma}
\begin{proof}
  Suppose $R$ is a minimal R-retraction of $G$ to $H$. If $R$ is not
  functional, then there exist distinct $x,y\in V_H$ such that
  $(u,x),(u,y)\in R$. Hence we could always pick a vertex from $\{x,y\}$
  which is different of $u$, w.l.o.g.\ suppose it is $x$. Then $R\setminus(u,x)$ is
  an R-retraction, which contradicts minimality. To see this, set
  $R'=R\setminus(u,x)$, then $R\supset R'\supset I_H$ and moreover $H=G\muls I_H
  \subseteq G\muls R'\subseteq G\muls R=H$, and thus $G\muls R'=H$.
\end{proof}


\begin{pro}
  A graph is R-reduced if and only if it is a graph core.
\end{pro}
\begin{proof}
  If $H$ is R-reduced from $G$ there is an R-retraction from $G$ to $H$
  which can be chosen minimal and hence by Lemma~\ref{fun} is functional
  and hence is a homomorphism retraction. Conversely, a homomorphism
  retraction is also an R-retraction. Hence the R-reduced graphs coincide
  with the graph cores.
\end{proof}

\begin{pro}
  Suppose $H$ is the core of graph $G$. If $H\muls R=K$ then there is a
  relation $R'$ such that $G\muls R'=K$. If $K\muls S=G$, then there is a
  relation $S'$ such that $K\muls S'=H$.
\end{pro}
\begin{proof}
  Since $H$ is the core of graph $G$, there is a relation $R_1$ such that
  $G\muls R_1=H$. If $H\muls R=K$ we have $G\muls R_1\muls R=K$ and
  $R'=R_1\circ R$ satisfies $G\muls R'=K$. If $K\muls S=G$ we have
  $K\muls S\muls R_1=H$ and $S'=S\circ R_1$ satisfies $K\circ S'=G$.
\end{proof}

\subsection*{Cocores}

In the classical setting of maps between graphs, one can only consider
retractions from a graph to its subgraphs, since graph homomorphisms of an
induced subgraph to the original graph are just the identity map. In the
setting of relations between graphs, however, it appears natural to
consider relations with identity restriction between a graph and an induced
subgraph. This gives rise to notions of R-coretraction and R-cocore in
analogy with R-retractions and R-reduced graphs.

\begin{definition}
  Let $H$ be a subgraph of graph $G$. An \emph{R-coretraction}\index{R-coretraction} of $H$ to $G$ is
  a relation $R$ such that $H\muls R=G$ and $(x,x)\in R$ for all $x\in
  V_H$. We say that $H$ is an \emph{R-coretract}\index{R-coretract} of $G$.
\end{definition}

\begin{lemma}
  If $H$ is an R-coretract of a graph $G$ and $K$ is an R-coretract of $H$, then
  $K$ is an R-coretract of $G$.
\end{lemma}
\begin{proof}
  Suppose $T$ is an R-coretraction of $K$ to $H$ and $S$ is an
  R-coretraction of $H$ to $G$. Then $(K\muls T)\muls S = K\muls(T\circ
  S)=G$. Furthermore $(x,x)\in T$ for all $x\in V_K\subseteq V_H$, and
  $(v,v)\in S$ for all $v\in V_H$, hence $(x,x)\in T\circ S$ for all $x\in
  V_K$. Therefore $T\circ S$ is an R-coretraction from $K$ to $G$.
\end{proof}

Hence, the following definition is meaningful.
\begin{definition}
  An R-coretract $H$ of a graph $G$ is an \emph{R-cocore of $G$}\index{R-cocore} if $H$
  does not have a proper subgraph that is an R-coretract of $H$ (and hence
  of $G$).
\end{definition}

\begin{figure}[!ht]
\centering
\subfloat[$G$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.7\textwidth]{core1.eps}
\end{minipage}}
\subfloat[$\mathrm{cocore}(G)$ ]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.7\textwidth]{cocore1.eps}
\end{minipage}}
 \caption{A graph and its cocore.}
  \label{fig:cocore}
\end{figure}



Clearly, the reference to $G$ is irrelevant: A graph $G$ is an
\emph{R-cocore}\index{R-cocore} if there is no proper subgraph of $G$ that is an
R-coretract of $G$. Similarly, we call $R$ a \emph{minimal
  R-coretraction}\index{minimal R-coretraction} of $H$ to $G$ if there exists no R-coretraction $R'$,
such that $R'\subset R$.

\begin{lemma}\label{lem:cocore}
  Let $H$ be an R-coretract of graph $G$, and let $R$ be a minimal
  R-coretraction of $H$ to $G$. Then the restriction of $R$ to $H$ equals to
  $I_H$.
\end{lemma}
\begin{proof}
  Suppose $R\cap (V_H\times V_H)\neq I_H$ and define $R_1=R\setminus
  \{(x,y)\in R:x,y\in V_H,x\neq y\}$. Then $H\muls R_1\subseteq H\muls
  R=G$. We claim that $H\muls R_1=H\muls R$ and thus $R_1$ is an
  R-coretraction of $H$ to $R$, contradicting the minimality of $R$.

  To prove this claim, it is sufficient to show that any edge $e\in E_G$ is
  contained in $H\muls R_1$. If $e$ is not incident with any vertex in
  $V_H$ or $e\in E_H$, the conclusion is trivial. So we only need to
  consider $e=(z,u)$ with $z\in E_H$ and $u\in V_G\setminus V_H$. Since
  $G=H\muls R$, one can find $x_1,x_2\in V_H$ such that $(x_1,z),(x_2,u)\in
  R$ and $(x_1,x_2)\in E_H$. Because $H\subseteq H\muls\big(I_H\cup
  (x_1,z)\big)\subset H\muls\big(R\cap (V_H \times V_H)\big)=H$, we get
  $N_H(x_1)\subseteq N_H(z)$. It follows that $(z,x_2)\in E_H$ and
  hence $e=(z,u)\in G\muls R_1$.
\end{proof}

Like R-reduced graphs, R-cocores also satisfy a stringent condition on their
neighbourhood structure.

\begin{definition} \label{nei}
  A graph $G$ satisfies property N* if, for every vertex $x\in V_G$,
  there is no subset $U_x\subseteq V_G\setminus\{x\}$ such that
  \begin{equation*}
    N_G(x)=\bigcup_{y\in U_x} N_G(y)
  \end{equation*}
\end{definition}
In other words, no neighbourhood can be represented as the union of
neighbourhoods of other vertices of graph $G$.

\begin{pro} \label{cocore} $G$ is an R-cocore if and only if $G$ has
  property N*.
\end{pro}
\begin{proof}
  Consider a vertex set $U_x$ as in Definition~\ref{nei} and suppose
  that there is a vertex $x\in V_G$ such that $N_G(x)=\bigcup_{y\in U_x}
  N_G(y)$. Then the relation $R:=I\setminus(x,x)\cup\{(y,x):y\in U_x\}$ is an
  R-coretraction from $G/x$ to $G$. Thus $G$ is not an R-cocore.

  Conversely, suppose that $G$ is not an R-cocore, let $H$ be a coretract
  of $G$, and denote by $R$ a minimal R-coretraction of $H$ to $G$. Then,
  by Lemma~\ref{lem:cocore}, $R\cap (V_H\times V_H)=I_H$. Consider a
  vertex $v\in V_G\setminus V_H$ and set
  $R^{-1}(v)=\{x_1,\dots,x_i\}$. Then $N(v)=\bigcup_i N(x_i)$, contradicting
  property N*.
\end{proof}

\begin{lemma} \label{thin-cocore1}
 An R-cocore of graph $G$ is isomorphic to an R-cocore of $G_{\text{pd}}$.
\end{lemma}
\begin{proof}
 Suppose graph $H$ is an R-cocore of graph $G$, then there exists a coretraction $R$
 such that $H\muls R = G$. By the definition of $G_{\text{pd}}$, we know
 there exists an R-retraction $R'$ such that $G\muls R'=G_{\text{pd}}$.
 Then $H\muls (R\circ R') = G$. It is easily seen that $R\circ R'$ is a coretraction.
 Also $H$ is the smallest subgraph of $G_{\text{pd}}$ which has a coretraction
 to $G_{\text{pd}}$, otherwise, suppose there are smaller graph $K$ such that $K$
 has a coretraction to $G_{\text{pd}}$, then $K$ also has a coretraction to $G$,
 which contradicts to the assumption that $H$ is an R-cocore.
 Therefore, $H$ is an R-cocore of $G_{\text{pd}}$.

 Conversely, if $H$ is an R-cocore of graph $G_{\text{pd}}$, then it is also
 an R-cocore of $G$.
\end{proof}

We call a subset $B$ of $V_G$ a \emph{basis}\index{basis} of graph $G$, if for any $x\in V_G$, there
 exists a subset $U_x$ of $B$ such that $N_G(x)=\bigcup_{y\in U_x} N_G(y)$. Of course
 a basis of a graph always exists, because $V_G$ is a basis of $G$. We call a basis of graph $G$
 with minimal cardinality a \emph{minimal basis}\index{minimal basis}. Because we consider only finite graphs,
 a minimal basis always exists. Now we prove that minimal basis of a point-determining graph $G$ is unique.


\begin{lemma} \label{basis}
 Minimal basis of a point-determining graph $G$ is unique.
\end{lemma}


\begin{proof}
  Assume there are two distinct minimal basis $A,B$. Neither
  contains the other by their minimality. Because $A,B$ are distinct,
  there exists an element $a\in A$ and $a\notin B$.

  Since $B$ is a basis of graph $G$, by the definition, there is a set $U_a\subset B$ such that
  $N_G(a)=\bigcup_{b\in U_a} N_G(b)$, thus $|N_G(a)|\geq |N_G(b)|$
  for all $b\in U_a$. Since $G$ is a point-determining graph, any two vertices of $G$ do not
  have the same neighbourhood, thus $|N_G(a)|>|N_G(b)|$
  for all $b\in U_a$. Because $A$ is also a basis of graph $G$, then for any $b\in U_a$,
  $N_G(b)$ can be represented as the union of the neighbourhood of some elements of $A\setminus\{a\}$,
  $a$ is not contained since $|N_G(a)|>|N_G(b)|$. Thus $N_G(a)=\bigcup_{b\in U_a} N_G(b)$ can
  be represented as the union of the neighbourhood of some elements of $A\setminus\{a\}$, which contradicts
  the minimality of $A$.
\end{proof}


\begin{lemma} \label{thin-cocore2}
 R-cocore of a point-determining graph is unique.
\end{lemma}

\begin{proof}
 %We first construct an R-cocore of a thin graph $G$, and then prove the uniqueness.

 From Lemma~\ref{basis}, we know that the basis of a point-determining graph is unique. We claim that the vertex set of
 any R-cocore of graph $G$ is the minimal basis of $G$. First,
 if $H$ is a R-cocore, then $V_H$ is a basis of graph $G$. Because by the definition of R-cocore,
 there is a coretraction $R$ such that $H\muls R = G$. For any vertex $x\in V_G$, we assign
 $U_x=R^{-1}\subset V_H$, it is easily seen that $N_G(x)=\bigcup_{y\in U_x} N_G(y)$.

 Then we prove $V_H$ is the minimal basis. Suppose there exists a subset $K$ of $V_G$ is a basis,
 and the cardinality of $K$ is smaller than $V_G$. By the definition of basis, for any $x\in V_G$
 we fix the set $U_x$, then there is an R-coretraction from $H$ to $G$, induced by $R(x)=\{y\in V_G\mid x\in U_y\}$.
 That is because for any vertex $x\in K$, we have $U_x=\{x\}$. It contradicts to the assumption that
 $H$ is a cocore.

 Therefore R-cocore of a point-determining graph is unique.
\end{proof}
% Now we prove that the subgraph $H$ induced by the minimal basis $B$ of thin graph $G$ is a R-cocore.
% Fix a set $U_x$ for each $x\in V_G$,
% then there is an R-coretraction from $H$ to $G$, induced by $R(x)=\{y\in V_G|x\in U_y\}$. That is because
% for any vertex $x\in B$, $U_x=\{x\}$. And it is easy to check that $H\muls R = G$.
% We claim $H$ is a minimal subgraph of $G$ which has an R-coretraction to $G$. Otherwise,




Because $G_{\text{pd}}$ is a point-determining graph, it follows from Lemma~\ref{thin-cocore2} that $G_{\text{pd}}$
has unique R-cocore for any graph $G$. And from lemma~\ref{thin-cocore1} we immediately get the
following proposition.

\begin{pro}
  R-cocore of $G$ is unique up to isomorphism.
\end{pro}
\iffalse
\begin{proof}
  We denote by $\mathcal{N}$ the collection of all open neighbourhoods of
  vertices in $G$, i.e.,
  $\mathcal{N}=\{N_G(x_1),N_G(x_2),\dots,N_G(x_k)\}$, where
  $V_G=\{x_1,x_2,\dots,x_k\}$. From the definition of the R-cocore we
  know that the subcollection $\mathcal{M}$ of $\mathcal{N}$ consisting of
  all the open neighbourhoods of vertices in R-cocore is a basis of
  $\mathcal{N}$, i.e., any set in $\mathcal{N}$ can be expressed by the
  union of some sets in $\mathcal{M}$. W.l.o.g., we denote the vertex set
  in an R-cocore $C$ of $G$ is $\{x_1,x_2,\dots,x_m\}$ where ${m\leq k}$,
  then $\mathcal{M}=\{N_G(x_1),N_G(x_2),\dots,N_G(x_m)\}$. We claim that
  any element in $\{N_G(x_1),N_G(x_2),\dots,N_G(x_m)\}$ cannot be
  expressed as the union of other elements, i.e., $\mathcal{M}$ is a
  minimal basis. Otherwise, w.l.o.g., suppose
  ${N_G(x_1)=\bigcup_{x_k}N_G(x_k)}$, ${x_k\in \{x_2,\dots,x_m\}}$. For any $1\leq
  k\leq m$, $N_G(x_k)=N_C(x_k)$ or $N_G(x_k)=N_C(x_k)+{\{x_i\mid (x_i,x_k)\in
  E_G, m+1\leq i\leq n\}}$, so either $N_C(x_1)=\cup_{x_k}N_C(x_k),{x_k\in
  \{x_2,\dots,x_m\}}$ or $N_C(x_1)=\cup_{x_k}N_C(x_k)+\{x_i\mid i\in 1,\dots,
  n\},{x_k\in \{x_2,\dots,x_m\}}$, the former contradicts to Proposition~\ref{cocore},
  which implies any element in
  ${\{N_C(x_1),N_C(x_2),\dots,N_C(x_m)\}}$ cannot be expressed as the union
  of other elements, the latter is impossible because $\{x_i\mid i\in 1,\dots,
  n\}\nsubseteq C$.

  Now we prove that this minimal basis is unique. Note that in
  $\mathcal{N}$ we view any vertex with the same neighbourhood as the same,
  since any vertex in R-cocore has different neighbourhoods. Let us
  consider two minimal sub-collections $\mathcal{A},\mathcal{B}$. Neither
  contains the other by their minimality. Since everything is finite, let
  $A\in \mathcal{A}/\mathcal{B}$ be an element of minimal size. Now
  $A$ can be expressed as a union of elements of $\mathcal{B}$, which all
  need to be of smaller cardinality than $A$ (or same but $A\notin
  \mathcal{B}$), but $\mathcal{A}$ then contains all of them, letting $A$
  be expressed by a union of elements of $\mathcal{A}$ contradicting the
  minimality of $\mathcal{A}$.
\end{proof}
\fi

These results allow us to construct an algorithm that computes the cocore
of given graph $G$ in polynomial time. First observe that the cocore of a
graph $G$ that contains isolated vertices is the disjoint union of the cocore
of the graph $G'$ obtained from $G$ by removing isolated vertices and the
graph consisting of a single isolated vertex. It is thus sufficient to
compute cocores for graphs without isolated vertices in Algorithm
\ref{alg1}.

\begin{algorithm}[htb]
\caption{The cocore of a graph}
\label{alg1}
\begin{algorithmic}[1]
  \REQUIRE ~~\\
  Graph $G$ with loops and without isolated vertices specified by its
  vertex set $V$ and the neighbourhoods $N_G(i)$, $i\in V$.
  \FOR{$i\in V$}
    \STATE $W(i)= \emptyset$
    \FOR {$j\in V\setminus \{i\}$}
      \IF {$N(j)\subseteq N(i)$}
        \STATE  $W(i):= W(i)\cup N(j)$
      \ENDIF
     \ENDFOR
    \IF {$W(i)=N(i)$}
      \STATE delete $i$ from $V$
      \STATE $N(i)= \emptyset$
    \ENDIF
  \ENDFOR
\RETURN $G[V]$, the cocore of $G$.
\end{algorithmic}
\end{algorithm}

\begin{pro}
  Suppose $H$ is a cocore of $G$. If $K\muls R=H$, then there is a relation
  $R'$ such that $K\muls R'=G$. If $G\muls S=K$, then there is a relation
  $S'$ such that $H\muls S'=K$.
\end{pro}
\begin{proof}
  Since $H$ is a cocore of $G$, there exists an R-coretraction $R_1$ such
  that ${H\muls R_1=G}$. If $K\muls R=H$, then letting $R'=R\circ R_1$ implies
  $K\muls R'=G$. If $G\muls S=K$, we have $H\muls R_1\muls S=K$. Let
  $S'=R_1\circ S$, then $H\muls S'=K$.
\end{proof}


We can find a graph which is not an R-core, and meanwhile it does not satisfy the
Hall condition. To see that, consider the graph $G$ in the example of Fig.~\ref{fig:weak}.
Obviously $R=\{(1,1),(2,2),(3,2),(4,4),(6,6),(5,3),(7,3),(5,5),(7,7)\}$
satisfies $G\muls R=G$. For the subset $S=\{2,3\}$ of $V(G)$, $R(S)=\{2\}$,
so $|R(S)|<|S|$, it does not satisfy the Hall condition. But not every graph which
are not R-cores do not satisfy the Hall condition. That means the condition of
Corollary~\ref{cor:nohall2} is not sufficient. To see this, we
consider a graph consisting of two independent isolated vertices.

Note that relations from an R-core or R-cocore to itself also satisfy the Hall condition.

\begin{pro}
If $G$ is an R-core, and $R$ is a relation satisfying $G\muls R = G$,
then any monomorphism $f\subset R$ satisfies $G\muls f = G$.
\end{pro}

\begin{proof}
From corollary~\ref{cor:nohall2} we know that $R$ which is a relation from
an R-core to itself satisfies the Hall condition
thus it contains a monomorphism. Suppose  $G\muls f \neq G$, then $G\muls f \subset G$.
By iteration we have $G\muls f^m \subset G$ for any $m$.
On the other hand, $f$ is a permutation, then there exists a $n$ such that $f^n$ is identity, thus
$G\muls f^n = G$. A contradiction.
\end{proof}

%\begin{pro}
% If $G\muls R = G$, and all solutions satisfy the Hall condition, then either of the two cases happens:
%\begin{enumerate}
 %\item $G$ is an $R$-core;
 %\item There is a solution contains a relation with non-full domain.
%\end{enumerate}
%\end{pro}

%\begin{proof}
%Suppose neither happens, then $G$ is not an $R$-core and all the relations are with full domain.
%Because $G$ is not an $R$-core, from the definition of $R$-core, we can find an induced subgraph $H$ of $G$ such that
%there is a relation $R_1$ satisfying $H\muls R_1 =G$
 % \begin{equation*}
  %  R(x)=
   % \begin{cases} R_1(x) \text{   for $x\in V_H$,}\\
    %  x \text{   otherwise,}
    %\end{cases}
    %\end{equation*}
    %thus $R$ is a non-full domain relation from
%$G$ to itself.

%It is easily seen that $R$ is a relation from $G$ to itself with full domain and it contains $R_1$.
%\end{proof}


Without the constraint of $R$ with full domain, we have:
\begin{pro}
All solutions of $G\muls R =G$ satisfy the Hall condition if and only if
$G$ is an R-cocore.
\end{pro}

\begin{proof}
If $G$ is an R-cocore, then all the solutions of $G\muls R = G$ are with full domain.
Note that $G$ is an R-cocore thus it is also an R-core,
from Corollary~\ref{cor:nohall2} we know that all solutions $R$ satisfy the
Hall condition.

Conversely, if all solutions satisfy the Hall condition, then all the solutions have full domains,
Hence $G$ is an R-cocore, otherwise we can find an induced subgraph $H$ of $G$ and a relation $R$
satisfying $H\muls R =G$. This relation $R$ is also the solution of $G\muls R = G$ in general (without constraint of
full domain) case.
\end{proof}

%Note that in the example(which?????), every relation contains a full relation.

Actually, it is very easy to get the following result which characterize the cases when all the solutions satisfy the Hall condition:
\begin{pro}
 If $G\muls R = G$, and all solutions satisfy the Hall condition, then either of the two cases happens:
\begin{enumerate}
 \item $G$ is an $R$-core;
 \item There is a solution contains a relation with non-full domain.
\end{enumerate}
\end{pro}

\subsection*{Inclusion relation}

Figure~\ref{fig:inclu} shows the inclusion relation of cores, R-cores, R-cocores, graphs with property N and point-determining graphs: the set of cores is a proper subset of the set of graphs with property N, which is a proper subset of R-cocores. The latter is a proper subset of R-cocores, the set of R-cores is a proper subset of the set of point-determining graphs.

  {\floatstyle{plain}\restylefloat{figure}%
   \begin{figure}[ht!]
   \centering
  \includegraphics[width=0.6\textwidth]{conclu.eps} 
\caption{Inclusion digram}
\label{fig:inclu}
   }{\end{figure}}


\begin{example}
We also give a list of examples to illustrate the proper inclusion relations, some of the examples have been already shown or explained before:
\begin{enumerate}
\item $K_3$ is a core, then of course it has property N and is a R-core, R-cocore and point-determining graph.
\item $C_6$ has property N but is not a core. Its core is $P_2$.
\item $P_4$ is an R-cocore but not with property N.
\item The graph $H$ in Figure~\ref{fig:glo} is a R-core but not an R-cocore, its R-cocore is $P_4$.
\item The graph in Figure~\ref{figa:weak} is a point-determining graph but not an R-core.
\end{enumerate}
\end{example}
% 
% 
% \subsection*{Lattice decomposition}
% 
% 
% Recall that a \emph{lattice}\index{lattice} is a partially ordered set in which any two elements have a \emph{supremum}\index{superemums}
% (also called a \emph{least upper bound}\index{least upper bound} or \emph{join}\index{join}) and an \emph{infimum}\index{infimum}
% (also called a \emph{greatest lower bound}\index{greatest lower bound} or \emph{meet}\index{meet}).
% 
% Lattices structures have been well studied in~\cite{Davey2002}. In general the partial order $\mathrm{Rel}(G,H)$ is not a lattice, but in some case it is. In this subsection we will study the
% structures of lattices in the partial order of $\mathrm{Rel}(G,H)$.
% 
% Note that graph homomorphism orders are lattice. And locally constrained homomorphism are semi-lattice.
% 
% \begin{obs}
% There is some observations about $\mathrm{Rel}(G,G)$:
% \begin{enumerate}
% \item If $G$ is a rigid graph, i.e., a graph has identity as the only automorphism, then $\mathrm{Rel}(G,G)$ is a trivial lattice (a lattice with only one vertex).
% \item If $G$ is with property N, then $G$ can be decomposed into $k$ trivial lattices, where $k$ is the number of automorphism of $G$.
% \end{enumerate}
% \end{obs}


\section{Computational complexity}
\label{sect:complexity}

In this section we briefly consider the complexity of computational
problems related to graph homomorphisms.
For the readers who are not familiar with computational complexity,
please refer to Appendix A. The \emph{homomorphism problem}\index{homomorphism problem}
$\Homo(H)$\index{$\Homo(H)$} takes as input some finite $G$ and asks whether there is a
homomorphism from $G$ to $H$. The computational complexity of the
homomorphism problem is fully characterized. It is known that $\Homo(H)$ is
NP-complete if and only if $H$ has no loops and contains odd cycles. All
the other cases are polynomial, see~\cite{Hell2004}.

The analogous problem for relations between graphs can be phrased as
follows: The \emph{(full) relation problem}\index{full relation problem,relation problem} $\FulRel(H)$\index{$\FulRel(H)$} takes as input
some finite $G$ and asks whether there is a relation with full domain from
$G$ and asks whether there is a relation from $G$ to $H$. We show that
this problem can be easily converted to a related problem on surjective
homomorphisms. The \emph{surjective homomorphism problem}\index{surjective homomorphism problem} $\sHom(H)$\index{$\sHom(H)$}
takes as input some finite $G$ and asks whether there is a surjective
homomorphism from $G$ to $H$.

Let $\leq_\text{P}^\text{Tur}$ indicate polynomial time Turing reduction.

\begin{thm} \label{thm:complex}
For finite $H$ our relation problem sits in the following relationship.
\begin{equation}
  \Homo(H)\leq_\text{P}^\text{Tur} \FulRel(H)
  \leq_\text{P}^\text{Tur} \sHom(H)\,.
\end{equation}
\end{thm}

\begin{proof}
  First we show that $\Homo(H)$ is polynomially reducible to $\FulRel(H)$.
  If there is a homomorphism from $G$ to $H$, then there is also a surjective
  homomorphism from $G+H$ to $H$. On the other hand, suppose $G$ has no
  homomorphism to $H$, from Lemma~\ref{reho} we conclude that $G+H$ has no
  relation to $H$ since $G$ has no relation to $H$.

  Now we show that the relation problem $\FulRel(H)$ is polynomially reducible to $\sHom(H)$.
  From Corollary~\ref{DeCo} we know $G\muls R = H$ if and only if there is
  a graph $G'=G\muls R_D$ which has a full homomorphism to $G$ and has a
  surjective homomorphism to $H$.

  We construct $G''$, by duplicating all the vertices of $G$ precisely
  $|V_H|$ times. We claim that $G'$ exists if and only if
  $G''$ has a full homomorphism to $G$. We can put
  $G'=G''$ because the surjective homomorphism can easily undo the
  redundant duplications. This gives the polynomial reduction from $\FulRel(H)$ to
  $\sHom(H)$.
\end{proof}

To our knowledge, $\sHom(H)$ is not fully classified. A recent survey of
the closely related complexity problem concerning the existence of vertex
surjective homomorphisms~\cite{Bodirsky2012} provides some arguments why the
characterization of complexity is likely to be hard. We observe that the
existence of a homomorphism from $G$ to $H$ is equivalent to the existence
of a surjective homomorphism from $G+H$ to $H$. Thus $\sHom(H)$ is clearly
hard for all graphs for which $\Homo(H)$ is hard, i.e., for all loop-less
graphs with odd cycles.

Testing the existence of a homomorphism from a fixed $G$ to $H$ is
polynomial (there is only a polynomial number $|V_H|^{|V_G|}$ of possible
functions from $G$ to $H$). Similarly the existence of a relation from a fixed
$G$ to $H$ is also polynomial. In fact, an effective algorithm exists.
For fixed $G$ there are finitely many point-determining graphs $T$ which $G$ has relation
to. The algorithm thus first constructs the point-determining graph of $H$ and then, using
a decision tree recognizes all isomorphic copies of all point-determining graphs $G$ has
relation to.

\section{Weak relational composition}
\label{sect:weak}

In this section we will briefly discuss the `loop-free' version, i.e.,
equations of the form $G\mulw R=H$.

Most importantly, there is no simple composition law analogous to
Lemma~\ref{lem:compo}. The expression
\begin{equation*}
(G\mulw R)\mulw S = (S^+\circ (R^+\circ G\circ R)^{\iota}\circ S)^\iota
\end{equation*}
does not reduce to relational composition in general. For example, let
$G=K_3$ with vertex set $V=\{x,y,z\}$ and consider the relations
$R=\{(x,1),(z,1),(y,2)\}\subseteq \{x,y,z\}\times\{1,2\}$ and
$S=\{(1,x')(1,z')(2,y')\}\subseteq \{1,2\}\times \{x',y',z'\}$. One can easily
verify
\begin{equation*}
(G\mulw R)\mulw S = P_2 \ne G\mulw(R\circ S)= K_3
\end{equation*}
The most important consequence of the lack of a composition law is that
R-retractions cannot be meaningfully defined for the weak
composition. Similarly, the results related to R-equivalence heavily rely
on the composition law.

Nevertheless, many of the above results, in particular basic properties derived
in Section~\ref{sect:basic}, remain valid for the weak composition
operation. As the proofs are in many cases analogous, we focus here mostly
on those results where strong and weak composition differ, or where we need
different proofs. In particular, Lemma~\ref{dec} also holds for the weak
composition. Thus, we still have a result similar to Corollary~\ref{DeCo},
but the proof is slightly different.

\begin{cor}
Suppose $G\mulw R=H$. Then there is a set $C$, an injective relation
$R_D\subseteq \domain R\times C$, and a surjective relation
$R_C\subseteq C\times \image R$ such that
$G[\domain R]\mulw R_D\mulw R_C=H[\image R]$.
\end{cor}
\begin{proof}
From Proposition~\ref{dec} we know $R=I'\circ R_D\circ R_C\circ I''$.
And we know $G[\domain R]\mulw R_D=G[\domain R]\muls R_D$.
From the properties of $\mulw$, we have
\begin{align*}
G[\domain R]\mulw R &=(R^+\circ G[\domain R]\circ R)^l\\
&=((R_D\circ R_C)^+\circ G[\domain R]\circ R_D\circ R_C)^l\\
&=(R_C^+\circ R_D^+\circ G[\domain R]\circ R_D\circ R_C)^l\\
&=(R_C^+\circ (R_D^+\circ G[\domain R]\circ R_D)\circ R_C)^l\\
&=(R_C^+\circ G[\domain R]\muls R_D\circ R_C)^l\\
&=(R_C^+\circ G[\domain R]\mulw R_D\circ R_C)^l\\
&=G[\domain R]\mulw R_D\mulw R_C\\
&=H[\image R].\qedhere
\end{align*}
\end{proof}

Assume $G\mulw R=H$ and let $H_1,\dots,H_k$ be the connected components of
$H$. From the definition of $\mulw$ and $\muls$, if we denote
$\widetilde{H}=G\muls R$, then $\widetilde{H}$ could be decomposed into the union
of connected components $\widetilde{H}_i$($1\leq i\leq k$), such that
$(\widetilde{H}_i)^\iota=H_i$. Hence the conclusion of the proposition
\ref{ccs} also holds true for weak relations.

Lemma~\ref{colour} does not hold for weak relations. For example, there is a
weak relation of $K_5$ to $K_3$, but $\chi(K_5)=5>\chi(K_3)=3$.

Lemma~\ref{path} and Lemma~\ref{cycle} do not hold for weak relations. For
example, if $G$ is a graph consisting of a single isolated vertex isolated,
then $P_3\mulw R=G$ and $C_3\mulw R=G$, but there are no walk in $G$.

With respect to complete graphs, weak relational composition also behaves
different from strong composition. If $K_k\mulw R=H$ then $R(i)$ can
contain more than one vertex in $V_H$. Comparing to Proposition
\ref{prop:complete}, we also obtain a different result:

\begin{thm}
  There is a relation $R$ such that $K_k\mulw R = H$ if and only if every
  connected component of $\overline{H}$ is a complete graph, and the number
  of connected components of $\overline{H}$ containing at least 2 vertices
  is at most $k$.
\end{thm}

\begin{proof}
  If every connected component of $\overline{H}$ is a complete graph,
  we denote the vertex sets of the connected components containing at least
  $2$ vertices by $H_1,\dots, H_m$, $m\leq k$ and the vertices of $K_k$ by
  $1,\dots,k$. Let $R={\{(i,u)\mid i=1,\dots,k,u\in V_{H_i}\}}\cup
  \{(j,v):1\leq j\leq k,v\in V_H\setminus \bigcup_{i=1}^m V_{H_i}\}$. One
  easily checks that $K_k\mulw R=H$.

  Conversely, let $R$ be a relation satisfying $K_k\mulw R=H$. Consider
  the set $U_i=\{u\in V_H\mid R^{-1}(u)=\{i\}\}$. Then $u$ and $v$ are not
  adjacent for arbitrary $u,v\in U_i$, while $u$ is adjacent to $w$ for
  every $w\in V_H\setminus U_i$. Hence
  $\overbar{H}(U_i)$ is a connected component of $\overbar{H}$, which is
  also a complete graph. Given $w\in V_H\setminus \bigcup_{i=1}^m U_i$,
  $R^{-1}(w)$ must have at least 2 vertices in $K_k$, hence $w$ is adjacent
  to every vertex in $H$ except itself; in other words, $w$ is an
  isolated vertex in $\overbar{H}$. Therefore the number of connected
  components of $\overbar{H}$ containing at least 2 vertices is no more
  than $k$.
\end{proof}

The results in subsection~\ref{revers} also remain true for weak relations.


% ------------------------------------------------------------------------


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> Chapter3/chapter3_old.tex <==
\chapter[R-Homomorphism]{R-Homomorphisms}
\ifpdf
    \graphicspath{{Chapter3/Chapter3Figs/PNG/}{Chapter3/Chapter3Figs/PDF/}{Chapter3/Chapter3Figs/}}
\else
    \graphicspath{{Chapter3/Chapter3Figs/EPS/}{Chapter3/Chapter3Figs/}}
\fi

\section{Outline and main results}
%\markboth{\MakeUppercase{\thechapter. R-Homomorphism }}{\thechapter. R-Homomorphism} %Chaptial LETTER DAXIE


%\subsection*{Outline and Main Results}

This chapter is organized as follows:

In section~\ref{sect:basic} the basic properties of the strong relations
between graphs are compiled. It is shown that relations compose and every
relation can be decomposed in a standard way into a surjective and an
injective relation (Corollary~\ref{DeCo}). We discuss some structural
properties of graph preserved by the relations.

Equivalence on the class of graphs induced by the existence of relations
between graphs is the topic of section~\ref{sect:retract}. We consider two
forms: the strong relational equivalence, where relations are required to
be reversible, and weak relational equivalence. Equivalent classes of
strong relational equivalence are characterized in Theorem~\ref{thm:equi}.
To describe equivalent classes of the weak relational equivalence we
introduce the notion of an R-core of a graph and show that it is in many
ways similar to the more familiar construction of the graph core
(Theorem~\ref{thm:Rcore}). We explore in particular the differences between
core and R-core and provide an effective algorithm to compute the R-core of
given graph.

Section~\ref{sect:poset} is concerned with the partial order induced on
relations between two fixed graphs $G$ and $H$ by inclusion. Focusing on the special
case $G=H$ the minimal elements of this partial order are described. In
Theorem~\ref{thm:auto1} we give a, perhaps surprisingly simple,
characterization of those graphs $G$ for which all relations of $G$ to
itself are automorphisms.

R-retraction is defined in section~\ref{sect:retraction} in analogy to
retractions. It naturally gives rise to a notion of R-reduced graphs that
we show to coincide with the concept of graph cores. By reversing the
direction of relations, however, we obtain the concept of a cocore of a
graph, which does not have a non-trivial counterpart in the world of
ordinary graph homomorphisms, and we explore its properties.

The computational complexity of testing for the existence of a relation
between two graphs is briefly discussed in section~\ref{sect:complexity}.
In Theorem~\ref{thm:complex} we describe the reduction of this problem to
the surjective homomorphism problem.

Finally, in section~\ref{sect:weak} we briefly summarize the most important
similarities and differences between weak and strong relational
composition.




\section{Basic properties}
\label{sect:basic}



\subsection*{Composition}

Recall that the composition of binary relations is associative, i.e.,
suppose $R\subseteq W\times X$, $S\subseteq X\times Y$, and $T\subseteq
Y\times Z$. Then $R\circ(S\circ T)=(R\circ S)\circ T$. Furthermore, the
transposition of relations satisfies $(R\circ S)^+ = S^+ \circ
R^+$. Interpreting the graph $G$ as a relation on its vertex set, we easily
derive the following identities.

\begin{lemma}[Composition law]\label{lem:compo}
  $(G\muls R)\muls S = G\muls(R\circ S)$.
\end{lemma}
\begin{proof}
\abovedisplayskip=-12pt
\belowdisplayskip=-12pt
\begin{equation*}
\begin{split}
(G\muls R)\muls S
 & = S^+\circ(R^+\circ G\circ R)\circ S =(S^+\circ R^+)\circ G\circ (R\circ S)\\
 & =(R\circ S)^+ \circ G\circ (R\circ S) = G\muls(R\circ S).
\end{split}
\end{equation*} 
\end{proof}

Now we show that every relation $R$ can be decomposed, in a standard way,
to a relation $R_D$ duplicating vertices and a relation $R_C$ contracting
vertices.

\begin{lemma} \label{dec}
  Let $R\subseteq X\times Y$ be a relation. Then there exists a subset $A$ of
  $X$, a set $B$, an
  injective relation with full domain $R_D\subseteq A\times B$ and a
  functional relation $R_C\subseteq B\times Y$, such that $R=I_A\circ
  R_D\circ R_C$, where $I_A$ is the identity on $X$ restricted to $A$.
\end{lemma}
\begin{proof}
  Put $A=\domain{R}$.
  Then the relation $I_A$ removes
  vertices in $X\setminus\domain{R}$. It remains
  to show, therefore, that any relation $R\subseteq X\times Y$ with full
  domain can be decomposed into an injective relation
  $R_D\subseteq X\times B$ and a
  functional relation $R_C\subseteq B\times
  Y$. To see this, set $B=R$ and declare $(x,\alpha)\in R_D$ if and only if
  $\alpha=(x,p)\in R$ for some $p\in Y$, and $(\beta,q)\in R_C$ if and only if
  $\beta=(y,q)\in R$ for some $y\in X$. By construction $R_D$ is injective
  and $R_C$ is functional. Furthermore, $(x_0,p_0)\in R_D\circ R_C$ if and
  only if there is $\alpha\in R$ that is simultaneously of the form
  $(x_0,p)$ and $(x,p_0)$, i.e., $x=x_0$ and $p=p_0$. Hence $(x_0,p_0)\in
  R$.
\end{proof}

Note that this decomposition is not unique. For instance, we could
construct $B$ from multiple copies of $R$. More precisely, let $B=R\times
\{1,2,\dots,k\}$, then we would set $\big(x,(\alpha,i)\big)\in R_D$
($1\leq i\leq k$) if and only if $\alpha=(x,p)\in R$ for some $p\in Y$,
etc.

The set $B$ as constructed in the proof of Lemma~\ref{dec} has
minimal size. To see this, it suffices to show that, given $B$ there
is a mapping from $B$ onto $R$. Since $R_D$ is injective and $R_C$ is
functional we may set
$$\alpha\in B\mapsto (R_D^{-1}(\alpha),R_C(\alpha)).$$
Since $R=I_A\circ R_D\circ R_C$ we conclude that the mapping is
surjective, and hence $|B|\geq |R|$.

According to Lemma~\ref{lem:compo}, the decomposition of $R$ in
Lemma~\ref{dec} can be restated as follows:
\begin{cor} \label{DeCo}
Suppose $G\muls R=H$. Then there is a set $B$, an injective relation
$R_D\subseteq \domain R\times B$ with full domain, and a surjective relation
$R_C\subseteq B\times \image R$ such that
$G[\domain R]\muls R_D\muls R_C=H$.
\end{cor}

In diagram form, this is expressed as
  \begin{figure}[!ht]
  \centering
  \includegraphics[width=0.25\textwidth]{comum.eps} 
\caption{Commuted diagram.}
\label{fig:comum}
\end{figure}   

We will remark that from the fact the relations compose it follows that
the existence of a relation implies a quasi-order on graphs that is related
to the homomorphism order. This order is studied more deeply in~\cite{Fiala2012}.

\subsection*{Structural properties preserved by relations}

In this subsection we investigate structural properties of $H$ that can be
derived from knowledge about certain properties of $G$ and the fact that
there is some relation $R$ such that $G\muls R=H$.

\subsubsection*{Connected components}

\begin{pro}\label{ccs}
  Let $G\muls R=H$ and denote by $H_1,\dots,H_k$ the connected components
  of $H$. Then there are relations $R_i\subseteq V_G\times V_{H_i}$ such
  that $G\muls R_i=H_i$ for each $1\leq i\leq k$ and $R=\bigcup_{i=1}^k
  R_i$. Furthermore, set $G_i=G[R^{-1}(V_{H_i})]$, then there are no edges
  between $G_i$ and $G_j$ for arbitrary $i\neq j$.
\end{pro}

\begin{proof}
  Define the restriction of $R$ to the connected components of $H$ as
  $R_i=\{(x,y)\in R\mid y\in V_{H_i}\}$. Clearly, $R$ is the disjoint union of
  the $R_i$ and $G\muls R_i\subseteq H_i$. The definition of $\muls$
  implies $H=G\muls R= \left(\bigcup_i R_i\right)^+ \circ G\circ
  \left(\bigcup_j R_j\right) = \bigcup_i\bigcup_j R_i^+ \circ G\circ R_j$.
  Since $R_i$ and $R_j$ relate vertices of $G$ to different connected
  components of $H$, we have $R_i^+ \circ G\circ R_j=\emptyset$. It follows
  that $H=\bigcup_i\bigcup_j R_i^+\circ G\circ R_j = \bigcup_i R_i^+\circ
  G\circ R_i = \bigcup_i G\muls R_i$. Hence $G\muls R_i=H_i$.

  Any edge between $G_i$ and $G_j$ would generate edges between $H_i$ and
  $H_j$, thus causing a contradiction to our assumptions.
\end{proof}

Denote by $b_0(G)$ the number of connected components of $G$, then from
Proposition~\ref{ccs} we arrive at:
\begin{cor}\label{cor:concomp}
  Suppose both $G$ and $H$ do not have isolated vertices. If $G\muls R=H$
  and $R$ has full domain, then $b_0(G)\geq b_0(H)$.
\end{cor}
\begin{proof}
  Our notations is the same as in Proposition~\ref{ccs}. We claim for arbitrary
  connected component $C$ of graph $G$, there exists a unique $i$, such that
  $C$ is a connected component of $G_i$. Otherwise one can find two
  vertices $x,y\in C$, $x$ and $y$ adjacent,
  such that $x\in V_{G_i}$ and $y\in V_{G_j}$, since $G$ has no isolated
  vertices, which contradicts
  $E(G_i,G_j)=\emptyset$. Thus it follows $b_0(G)\geq b_0(H)$.
\end{proof}

From corollary~\ref{cor:concomp}, we know that $H$ is connected whenever $G$
is connected. Conversely, the connectedness of $G$, however, cannot be deduced from the
connectedness of $H$. For example, consider $G=P_1\cup P_1$ with vertex set
$\{x_1,x_2,x_3,x_4\}$ and edges $\{x_1,x_2\}$ and $\{x_3,x_4\}$, and
$H=P_2$ with vertex set $\{v_1,v_2,v_3\}$. Set
$R=\{(x_1,v_1),(x_2,v_2),(x_3,v_2),(x_4,v_3)\}$. One can easily verify that
$G\muls R=H$. On the other hand, $H$ is connected but $G$ has 2 connected
components. The point here is, of course, that $R$ is not injective.

\subsubsection*{Colorings}
Graph homomorphisms of simple graphs can be seen as generalizations of
colourings. Thus, if $R$ is a
functional relation describing a vertex colouring, then $G\muls R\subseteq
K_k$. Conversely, if $G\muls R\subseteq K_k$, where $R$ has full domain,
then from Lemma~\ref{reho}, there exists a homomorphism from $G$ to
$K_k$, which is a colouring of $G$.
\begin{lemma} \label{colour} If $G$ is a simple graph and $R$ has full
  domain, then $\chi(G)\leq \chi(G\muls R)$.
\end{lemma}

\begin{proof}
  Suppose $G\muls R=H$ and the domain of $R$ is full, from Lemma~\ref{reho}
  we know $G\rightarrow H$, so $\chi(G)\leq \chi(G\muls R)$.
\end{proof}

\subsubsection*{Distances} \label{sub:dist}
\begin{obser} \label{path} If $P_k\muls R=G$, $G$ is a simple graph and the
  domain of $R$ is full, $P_k$ with the vertex set ${0,1,\dots,k}$, then
  there is a walk $[v_0,v_1,\dots,v_k]$ in $G$, where $(i,v_i)\in R$ for
  $0\leq i\leq k$.
\end{obser}

\begin{obser} \label{cycle} If $C_k\muls R=G$, $G$ is a simple graph and
  the domain of $R$ is full, then there is a closed walk
  $[v_0,v_1,\dots,v_{k-1}]$ in $G$, where $(i,v_i)\in R$ for $0\leq i\leq
  k-1$.
\end{obser}

Recall that $d_G(x,y)$ denote the \emph{(canonical) distance}\index{(canonical) distance} on graph $G$, i.e.,
$d_G(x,y)$ is the minimal length of a path in graph $G$ that connects
vertices $x$ and $y$; if there is no path connects vertices $x$ and $y$,
then the distance is infinite.

\begin{lemma}
  Suppose there exists a relation $R$ with full domain s.t.\ $G\muls R=H$,
  $x,y\in V_G$, $u,v\in V_H$ and $(x,u)\in R, (y,v)\in R$. If $x\neq y$,
  then $d_H(u,v)\leq d_G(x,y)$; If $x=y$ and $x$ is not an isolated vertex,
  then $d_H(u,v)\leq 2$.
\end{lemma}
\begin{proof}
  If $x=y$ and $x$ is not isolated, pick a vertex $z$ of graph $G$ which is
  adjacent to vertex $x$, and find a vertex $w\in H$ satisfying $(z,w)\in
  R$. Then $(w,u)\in E_H$ and similarly $(w,v)\in E_H$. So $d_H(u,v)\leq
  2$.

  If $x\neq y$, choose the shortest path $P=x,x_1,x_2,\dots, x_k,y$
  between $x$ and $y$, and find corresponding vertices
  $u_1,u_2,\dots,u_k\in H$ such that$(x_i,u_i)\in R$ for any $1\leq i\leq
  k-1$ it is easily seen that $(u,u_1)\in E_H$, $(u_i,u_{i+1})\in E_H$ and
  $(u_k,v)\in E_H$, then $d(u,v)\leq d(x,y)$.
\end{proof}

Hence we immediately get the following corollary about radius.

\begin{cor} \label{rad} Suppose $G\muls R=H$, $G$ and $H$ are connected
graphs, and $R$ has full domain, then $rad(H)\leq \max\{rad(G),2\}$.
\end{cor}
An analogous results holds for the diameters. In particular, if $G$
is not a complete graph, then $diam(G)\geq diam(G\muls R)$. As a result,
$k<l$ and $k\neq 1$ implies there is no relation from $P_k$ to $P_l$.
And as we state in the example section, $(P_1,P_2)$ is the only pair of paths
such that there is a relation from one to another and vice versa.

\label{subs:complete}

%The \emph{complement graph $\overline{H}$} of a simple graph $H$ has the
%same vertex set as $H$, and two vertices are connected in $\overline{H}$ if
%and only if they are not connected in $H$.
\subsubsection*{Complete graphs} 
Note that in this subsection we do not require that the domain of $R$ is
full.


\begin{pro}\label{prop:complete}

  Let $H$ be a simple graph. Then there exists a relation $R$ such that
  $K_k\muls R=H$ if and only if $H$ is a complete $m$-partite graph, where
  $m\leq k$.

\end{pro}

\begin{proof}
 We denote the vertices of $K_k$ by $1,\dots,k$.

 If $H$ is a complete $m$-partite graph, let $R=\{(i,u)\mid i=1,\dots,m,u\in U_i\}\}$, then
 for each $1\leq i\leq m$, all the vertices
  in $U_i$ are independent in $H$, and $u$ is adjacent to $v$ whenever
  $u\in U_i$ and $v\in U_j$ for distinct $i,j$. Hence it is easily
  seen that $K_k\muls R=H$.

   Conversely, if $K_k\muls R=H$, assume $\domain R=\{1,\dots,m\}$. We claim that $R$ is
  injective, otherwise $H$ would have loops. Thus $V_H$ is the disjoint union
  of $R(1),\dots,R(m)$. For any
  two distinct vertices $u,v$ in $R(i)$, $u$ and $v$ are independent in $H$,
  then $H$ is a $m$-partite graph.
  For distinct $i$ and $j$ every vertex in $R(i)$ are adjacent with every
  vertex in $R(j)$ whenever $R(i)\neq \emptyset$, which means $H$ a complete $m$-partite graph.
\end{proof}


%\begin{pro}
%  Let $H$ be a simple graph. Then there exists a relation $R$ such that
%  $K_k\muls R=H$ if and only if $\overline{H}$ is the disjoint union
%  of at most $k$ complete graphs.
%\end{pro}

\subsubsection*{Subgraphs} \label{sect:subgraph}

Relations between graphs intuitively imply relations between local
subgraphs. In this section we make this concept more precise. Recall $N[x]$ is denoted to be
the \emph{closed neighbourhood}\index{closed neighbourhood} of $x$ in $G$ and
$\overbar{N_G[x]}:= V_G\setminus N_G[x]$ \index{$\overbar{N_G[x]}$} be the set of vertices that are
not adjacent (or identical) to $x$ in $G$. Furthermore,
$\overbar{G_x}:=G-N_G[x]$\index{$\overbar{G_x}$}, which is the induced subgraph of $G$
obtained by removing the closed neighbourhood of a vertex $x$.
Analogously, for a subset $S\subseteq V_G$, $\overbar S$ is the induced subgraph obtained by removing all vertices in $S$ and their neighbours.

Then we have the following result about relations between local subgraphs.



\begin{pro} Suppose $G\muls R=H$ and $(x,u)\in R$. Suppose there is no isolated vertex in $G$. If there is no loops in
  $x$, then $\overbar{G_x}\muls \widetilde{R} = \overbar{G_u}$ where
  $\widetilde{R}\subseteq \overbar{N_G[x]}\times\overbar{N_H[u]}$ is the
  restriction of $R$.
\end{pro}

\begin{proof}
  We claim that the pre-image of any vertex in $\overbar H_u$ is not
    in $N_G(x)$. Otherwise, there is a vertex $v\in \overbar H_u$ and a
    vertex $y\in N_G(x)$ such that $(y,v)\in R$; from $(x,u)\in R$ we deduce
    that $v$ and $u$ are adjacent, which contradicts to $v\in \overbar
    H_u$. Next we claim that there is no vertex in $\overbar H_u$ whose
    pre-image is $x$. Suppose $v\in \overbar H_u$ and $R^{-1}(v)=\{x\}$.
    Since $v$ is not isolated in $\overbar H_u$, there exists a
    vertex $v'$ which is adjacent with $v$ in $\overbar H_u$. Thus
    $R^{-1}(v')\cap N(x)\neq \emptyset$, a contradiction. Hence
    for any edge $(v,v')$ in $\overbar H_u$, we can find
    an edge $(y,y')$ in $\overbar G_x$ such that $(y,v),(y',v')\in
    R$. Thus $\overbar G_x\muls \widetilde{R}=\overbar{G_y}$.
\end{proof}

%$(x,u)\in R$
%\TODO{
%if the vertex $x$ is isolated and $x$ duplicated.
%1.1 $u$ is also isolated, $u$ has only one preimage. then there is an isolated vertex
%after deleting. may have problem(if $G$ have no other isolated vertex, eg. two isolated vertex
%to two isolated vertex)

%1.2 $u$ is also isolated, and $x$ contracts.
%may have problem.



%1. if the vertex $x$ is isolated and been duplicated,

%1.1. if $u$ has only one preimage on $G$, then after deleting, there is a isolated vertex in %$H$.

%1.2. if it has more than one preimages, no impact.
%}

\begin{example}
Let us see an example. Let $G$ and $H$ are graphs as Figure~\ref{fige5}.
For a relation from graph $G$ to graph $H$, we consider the pre-image of
vertex $u$, because the domain of $R$ is full, and the symmetry of $P_4$, at least
either $(1,u)\in R$ or $(2,u)\in R$ holds. If $(1, u)\in R$, from the
above theorem, we know that there is an induced relation from $P_2$ to
$P_4$, but it is impossible. If $(2,u)\in R$ holds, also from above
theorem, there is an induced relation from $P_1$ to $P_4$, it also
cannot holds.

\begin{figure}[!ht]
\centering
\subfloat[$G$]{
%\label{fig:improved_subfig_a}
\begin{minipage}[c]{0.4\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{dupl1.eps}
\end{minipage}
}
\subfloat[$H$]{
%\label{fig:improved_subfig_b}
\begin{minipage}[c]{0.4\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{ex3.eps}
\end{minipage}
}
 \caption{There is no relation from $G$ to $H$.}
    \label{fige5}
\end{figure}
\end{example}


Note that from Corollary~\ref{rad}, the radius of $H$ is smaller than the radius of $G$, so there is no relation $R$ such that
$H\muls \widetilde{R}=G$. Therefore there is no relation from $G$ to $H$, neither from $H$ to $G$. Note that the two solutions can be different.



\begin{pro} \label{pro:subgraph}
  Suppose $G\muls R=H$ and $S$ and $D$ are subsets of $V_G$ and $V_H$,
  respectively, such that
  \begin{enumerate}
   \item $G[S] \muls R|_{(S\times D)}=H[D]$;
   \item $R|_{(S\times D)}$ has full domain on $S$;
   \item there is no isolated vertex in $\overbar D$.
  \end{enumerate}

  Then $\overbar S\muls\widetilde{R}=\overbar D$,
  where $\widetilde{R} = R|_{(\overbar S\times \overbar D)}$ is the
  corresponding restriction of $R$.
\end{pro}

\begin{proof}
  Obviously, $\overbar S\muls\widetilde{R}$ is an induced subgraph of $\overbar
  D$. We need to show the reverse inclusion. Given $u\in V_{\overbar{D}}$
  and $x\in R^{-1}(u)$, we first show that there are two possibilities:
  \begin{enumerate}
  \item $x$ is a vertex of $\overline{S}$.
  \item $x$ is an isolated vertex of $S$.
  \end{enumerate}
  Assume that is not the case, i.e., $x$ is either a non-isolated vertex of $S$ or $x$ is in the
  neighbourhood of some vertex of $S$. In both cases there is $y\in S$
  connected by an edge to $x$. Consequently there is a vertex $v\in D$, such
  that $v\in R(y)$, and $v$ is connected by an edge to $u$. It follows
  $u\notin V_{\overbar{D}}$, a contradiction.

  Now consider an arbitrary edge $(u,v)\in E_{\overbar{D}}$. We have
  $(x,y)\in E_G$ such that $u\in R(x)$ and $v\in R(y)$.
  If any of $x$ and $y$, say $x$, is an isolated vertex in $S$, then $y$ is not in $S$.
  Thus $y$ is in the neighbourhood of $S$, which contracts the two possibilities.
  So both $x$ and $y$ are not isolated in $S$, from the above deduction $x,y$ are in the case 1, i.e.,
  they are vertices of $\overline{S}$.
  Consequently $\overbar S\muls\widetilde{R}$ has precisely the same edges
  as $\overbar D$. Because $\overbar{D}$ has no isolated vertices and
  thus every vertex is an endpoint of some edge, we know that the vertex set
  of $\overbar S\muls\widetilde{R}$ is same as the vertex set of $\overbar D$. Hence
  $\overbar S\muls\widetilde{R}=\overbar D$.
\end{proof}
This result is of particular practical use in the special case where $S$
and $D$ consist of a single vertex. When looking for a relation $R$ such
that $G\muls R=H$ one can remove a vertex including its neighborhood from
$G$ as well as the prospective image including the neighborhood from $H$
and solve the problem on the subgraphs.



\section{Relational equivalence}
\label{sect:retract}
Recall that in Section~\ref{sec:hom-equ} we define graphs $G$ and $H$ are \emph{homomorphism equivalent}\index{homomorphism equivalent} (or
\emph{hom-equivalent}\index{hom-equivalent}) if there exists homomorphisms $G\to H$ and $H\to
G$. It is well known that every equivalence class of the homomorphism order
contains a minimal representative that is unique up to isomorphism: the
\emph{graph core}\index{graph core}~\cite{Hell2004}.

We define similar equivalences implied by the existence of
(special) relations between graphs. In this section, we require all
relations to have full domain unless explicitly stated otherwise. With
this condition we will show that these equivalences produce a rich structure
closely related to but distinct from the structure of homomorphism
equivalences.

This may come as a surprise: the equivalence implied by the existence of
surjective homomorphisms is not interesting. Consider two graphs $G$ and
$H$ and suppose there are surjective homomorphisms $f:G\to H$ and $g:H\to
G$. Since every vertex in $V_G$ has at most one image under $f$, we have
$|V_G|\geq |V_H|$. Analogously $|V_H|\geq |V_G|$, and hence
$|V_G|=|V_H|$. Thus $f$ and $g$ are both bijective, and $G$ is isomorphic
to $H$.

\subsection*{Reversible relations} \label{revers}

\begin{definition}
  A relation $R$ is \emph{reversible with respect to graph $G$}\index{reversible} if
  $(G\muls R)\muls R^+=G$.
\end{definition}

Recall that in Proposition~\ref{dec} we proved that $R$ can be decomposed.
Suppose $R=R_D\circ R_C$, where $R_D$ and $R_C$
are constructed as in the proof of Proposition~\ref{dec}.
Then we can get the following result with respect to reversible relation.

\begin{pro} \label{reve}   
$R$ is reversible with respect $G$ if and only if for every $\alpha$ and $\beta$
  satisfying $R_C(\alpha)=R_C(\beta)$ we have
  $N_{G\muls R_D}(\alpha)= N_{G\muls R_D}(\beta)$.
\end{pro}
\begin{proof}
  We set $G_1=G\muls R_D$, If $R_C(\alpha)=R_C(\beta)$ implies
  $N_{G_1}(\alpha)= N_{G_1}(\beta)$, then $H\muls R_C^+=G_1$.
  Therefore,
  \begin{align*}
     G\muls R\muls R^+ & = H\muls R^+ = H\muls (R_D\muls R_C)^+\\
                       & = H\muls R_C^+\muls R_D^+ = G_1\muls R_D^+ = G.
   \end{align*}

  The first equation is by assumption, the second is by Proposition~\ref{dec}, the third one
  is by the property of transpose, the fourth is from Lemma~\ref{lem:compo}.
  the last equation is by the property of $R_D$.
  Thus by definition, $R$ is reversible.

  Conversely, since $R$ is
  reversible, i.e., $H\muls R^+=G$, setting $G_2 = H\muls R_C^+$ gives
  $G_2\muls R_D^+=G$. Hence $G_1\muls R_C\muls R_C^+=G_2$ and $G_2\muls
  R_D^+\muls R_D=G_1$. From $I_{G_1}\subseteq R_C\muls R_C^+$ we conclude
  $G_1\subseteq G_2$, and similarly $I_{G_2}\subseteq R_D^+\muls R_D$ yields
  $G_1\supseteq G_2$. Hence $G_1=G_2$. $R_C^+$ is injective, hence
  $\alpha,\beta\in V_{G_2}=V_{G_1}$ has the same open neighbourhood whenever
  the pre-image of $\alpha$ and $\beta$ under $R_C^+$ coincide,
  i.e. $R_C(\alpha)=R_C(\beta)$.
\end{proof}

$R_D$ is an injective relation, hence one can easily get
$N_{G\muls R_D}(\alpha)=R_D(N_G(x))$ provided that $(x,\alpha)\in R_D$. On the
other hand, if we define $R$ to be the image of $R_D$ as in the proof of
Proposition~\ref{dec}, then $R_C(\alpha)=R_C(\beta)$ implies there are two
distinct vertices $x,y\in V_G$, s.t. $(x,u),(y,u)\in R$, where
$u=R_C(\alpha)=R_C(\beta)$, and verse visa. Using Proposition~\ref{reve}
we thus obtain
\begin{pro}
  A relation $R$ is reversible with respect to $G$ if and only if for every
  two vertices $x$ and $y$ such that $R(x)\cap R(y) \neq \emptyset$ we have
  $N_G(x)=N_G(y)$.
\end{pro}

\subsection*{Strong relational equivalence}

\begin{definition}
  Two graphs $G$ and $H$ are \emph{(strongly) relationally equivalent}, $G
  \backsim H$, if there is a relation $R$ such that $G\muls R=H$ and
  $H\muls R^+=G$.
\end{definition}

\begin{lemma}
  Relational equivalence is an equivalence relation on graphs.
\end{lemma}
\begin{proof}
  By definition $\backsim$ is symmetric. Because $G\muls I_G=G$, relation
  $\backsim$ is reflexive. Suppose $G\backsim G'$ and $G'\backsim
  G''$. Thus there are relations $R$, $S$, such that
  $G'=G\muls R$, $G''=G'\muls S$, $G=G'\muls R^{-1}$, and $G'=G''\muls S^{-1}$. By
  the composition law (Lemma~\ref{lem:compo}) it follows that
  $G''=G\muls(R\circ S)$ and $G=G''\muls(S^{-1}\circ R^{-1})=G''\muls(R\circ S)^{-1}$, i.e, $G\backsim
  G''$. Hence $\backsim$ is transitive.
\end{proof}


Recall that the \emph{thinness relation}\index{thinness relation} $S$ of $G$ is the equivalence relation on
  $V_G$ defined by $(x,y)\in S$ if and only if $N_G(x)=N_G(y)$.
  We denote by $\mathcal{S}$ the corresponding partition of $V_G$, and write
  $R_S\subseteq V_G\times\mathcal{S}$ that associates each vertex with its
  $S$-equivalence class, i.e., $(x,\beta)\in R_S$ if and only if $x\in\beta$.
In this context it is well known that $G$ can
be reconstructed from $G_{pd}$ and the knowledge of the $S$-equivalence
classes. In fact, we have
\begin{equation*}
\label{eq:thin-1}
  G_{pd}\muls R^+_S=G.
\end{equation*}




\begin{thm} \label{thm:equi}
  $G$ and $H$ are in the same equivalence class w.r.t.\ $\backsim$ if and
  only if their point-determining graphs are isomorphic.
\end{thm}
\begin{proof}
  Assume $G\backsim H$. From Equation(\ref{eq:thin-1}) we know that
  $G\backsim G_{pd}$, $H\backsim H_{pd}$, so $G_{pd}\backsim
  H_{pd}$.
  Now we claim that $G_{pd}$ and $H_{pd}$ are isomorphic.
  Suppose $G_{pd}\muls R=H_{pd}$, then the pre-image of $R$ is unique.
  Otherwise, there exist distinct vertices $x,y\in V_{G_{pd}}$ such that
  $R(x)=R(y)$, then $N_{G_{pd}}(x)=N_{G_{pd}}(y)$, contradicting
  thinness. Likewise, the pre-image of $R^{-1}$ is unique, i.e., the image
  of $R$ is unique. Hence $R$ is one-to-one.
\end{proof}

\begin{figure}[!ht]
\centering
\subfloat[$G$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
 \includegraphics[height=0.7\textwidth]{ex3.1.1.eps}
\end{minipage}}
\subfloat[$H$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
 \includegraphics[height=0.7\textwidth]{ex3.1.2.eps}
\end{minipage}}
\subfloat[$G_{pd}=H_{pd}$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
 \includegraphics[height=0.7\textwidth]{ex3.1.3.eps}
\end{minipage}}
\caption{Non-isomorphic graphs $G$ and $H$ with isomorphic point-determining graphs.}
\label{fig:thin}
\end{figure}

%\begin{figure}
%\begin{center}
 % \begin{tabular}{ccc}
  %  \includegraphics[height=0.2\textwidth]{ex3.1.1.eps} &
   % \includegraphics[height=0.2\textwidth]{ex3.1.2.eps} &
    %\includegraphics[height=0.2\textwidth]{ex3.1.3.eps} \\
    %$G$ & $H$ & $G_{thin}=H_{thin}$\\
  %\end{tabular}
%\end{center}
%\caption{Non-isomorphic graphs $G$ and $H$ with isomorphic thin graphs.}
%\label{fig:thin}
%\end{figure}

The example in Fig.~\ref{fig:thin} shows that point-determining graphs can be isomorphic
while $G$ and $H$ themselves are not isomorphic. Relational equivalence
thus is coarser than graph isomorphism (surjective homomorphic equivalence)
but stronger than homomorphic equivalence.

\subsection*{Weak relational equivalence} \label{sec:weakeq}

\begin{definition}
  Two graphs $G$ and $H$ are \emph{weak relationally equivalent}\index{weak relationally equivalent}, $G
  \backsim_w H$\index{$\backsim_w$}, if there are relations $R$ and $S$ such that $G\muls R=H$
  and $H\muls S=G$.
\end{definition}

\begin{lemma}
  Weak relational equivalence is an equivalence relation on graphs.
\end{lemma}
\begin{proof}
  By definition $\backsim_w$ is symmetric. Because $G\muls I_G=G$, relation
  $\backsim_w$ is reflexive. Suppose $G\backsim_w G'$ and $G'\backsim_w
  G''$. Thus there are relations $R$, $S$, $R'$, and $S'$, such that
  $G'=G\muls R$, $G''=G'\muls R'$, $G=G'\muls S$, and $G'=G''\muls S'$. By
  the composition law (Lemma~\ref{lem:compo}) it follows that
  $G''=G\muls(R\circ R')$ and $G=G''\muls(S'\circ S)$, i.e, $G\backsim_w
  G''$. Hence $\backsim_w$ is transitive.
\end{proof}

Strong relational equivalence implies weak relational equivalence. To see
this, simply observe that the definition of the weak form is obtained from
the strong one by setting $S=R^+$.

\begin{figure}[!ht]
\centering
\subfloat[$G$]{\label{figa:weak}
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{weak_nonstrong.eps}
\end{minipage}}
\subfloat[$H$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{weak_nonstrong2.eps}
\end{minipage}}
\caption{$G$ and $H$ are weakly relationally equivalent but have
  non-isomorphic  graphs.}
\label{fig:weak}
\end{figure}


%\begin{figure}[!ht]
%\begin{center}
 % \begin{tabular}{ccc}
  %  \includegraphics[height=0.25\textwidth]{weak_nonstrong.eps} &\qquad
   % \includegraphics[height=0.25\textwidth]{weak_nonstrong2.eps}\\
    %    $G$ & \qquad $H$ 
  %\end{tabular}
%\end{center}
%\caption{$G$ and $H$ are weakly relationally equivalent but have
 % non-isomorphic thin graphs.}
%\label{fig:weak}
%\end{figure}

The converse is not true, as shown by the graphs $G$ and $H$ in
Fig.~\ref{fig:weak}: It is easy to see that their point-determining graphs are different
and thus $G$ and $H$ are not strongly relationally equivalent. However,
they are relationally equivalent. To get relation from $G$ to $H$ contract
vertices 2 and 3 and keep other vertices on place, i.e.,
$$R=\{(1,1),(2,2),(3,2),(4,4),(5,5),(6,6),(7,7)\}.$$ To get relation
from $H$ to $G$, duplicate 5 and 7 and contract them together to 3,
$$S=\{(1,1),(2,2),(4,4),(5,5),(6,6),(7,7),(5,3),(7,3)\}.$$
Consequently, weak relational equivalence is coarser than strong relational
equivalence.

\subsection*{R-cores}

A graph is an \emph{R-core}\index{R-core}, if it is the smallest graph (in the number of
vertices) in its equivalence of $\backsim_w$.

This notion is analogous to the definition of graph cores. In this section
we show properties of R-cores that are similar to the properties of graph
cores. To this end we first need to develop a simple characterization of
R-cores.

Again we start from a decomposition of relations. Consider a relation
$R$ such that $G\muls R = H$. We seek for pair of relations $R_1$ and
$R_2$ such that $R=R_1\circ R_2$. In contrast to Lemma~\ref{dec}, however,
we now look for a decomposition so that the graph $G'=G\muls R_1$ is
smaller (in the number of vertices) than $G$.
%\begin{equation}
%\xymatrix{
%G \ar[dr]_{R_1}  \ar@{->}[rr]^{R=R_1\circ R_2} & & H \\
%  & G' \ar[ur]_{R_2} &
%}
%\end{equation}
  \begin{figure}[!ht]
  \centering
  \includegraphics[width=0.25\textwidth]{comum.eps} 
\caption{Communted diagram.}
\label{fig:comum2}
\end{figure}   

The existence of such a decomposition follows from a translation of
the well-known Hall Marriage Theorem~\cite{Schrijver2003} to the language of
relations. We say that the relation $R\subseteq A\times B$ satisfies the
\emph{Hall condition}, if for every $S\subseteq A$ we have $|S|\leq |R(S)|$.

\begin{thm}[\textbf{Hall's theorem}] \label{thm:hall}
  If $G\muls R = H$ and $R$ satisfies the Hall condition, then $R$
  contains a monomorphism $f:G\rightarrow H$.
\end{thm}

\begin{proof}
  The Hall Marriage Theorem is usually described on set systems. For set
  systems satisfying the Hall condition, the theorem guarantees the
  existence of a system of distinct representatives, see i.e.~\cite{Schrijver2003}. Relations can be seen as set systems (defined by
  the images of individual vertices). Furthermore, in our setting the
  system of distinct representatives directly corresponds to a monomorphism
  contained in the relation $R$.
\end{proof}

\begin{lemma} \label{lem:nohall} If $G\muls R = H$ and relation $R$ does
  not satisfy the Hall condition, then there are relations $R_1$ and $R_2$
  such that $R=R_1\circ R_2$, and the number of vertices of graph
  $G'=G\muls R_1$ is strictly smaller than the number of vertices of $G$.
\end{lemma}
\begin{proof}
  Without loss of generality assume that $V_G\cap V_H=\emptyset$. If $R$
  does not satisfy the Hall condition, then there exists a vertex set $S\subset
  V_G$ such that $|S|>|R(S)|$. Now we define relations $R_1$ and $R_2$ as
  follows:
  \begin{equation*}
    R_1(x)=
    \begin{cases} R(x) \text{   for $x\in S$,}\\
      x \text{   otherwise,}
    \end{cases}
\qquad\qquad\qquad
    R_2(x)=
    \begin{cases} x \text{   for $x\in R(S)$,}\\
      R(x) \text{   otherwise.}
    \end{cases}
  \end{equation*}
Obviously $R_1\circ R_2 = R$ and $|V_{G'}|=|V_G|-(|S|-|R(S)|)<|V_G|$.
\end{proof}

This immediately gives a necessary, but in general not sufficient,
condition for a graph to be an R-core.

\begin{cor}\label{cor:nohall2}
  If $G$ is an R-core, then every relation $R$ such that $G\muls R=G$
  satisfies the Hall condition and thus contains a monomorphism.
\end{cor}
\begin{proof}
  Assume that there is a relation $R$ that does not satisfy the Hall
  condition. Then there is a graph $G'$, $|V_{G'}|<|V_G|$, and relations
  $R_1$ and $R_2$ such that $G\muls R_1=G'$ and $G'\muls
  R_2=G$. Consequently $G'$ is a smaller representative of the equivalence
  class of $\backsim_w$, a contradiction with $G$ being R-core.
\end{proof}

To see that the condition of Corollary~\ref{cor:nohall2} is not sufficient
consider a graph $G$ consisting of two independent vertices. It is not an R-core,
because it can retract to an isolated vertex. However, the relation required
to be full, any relation from $G$ to itself satisfies the Hall condition.

Next we show that R-cores are, up to isomorphism, unique representatives of
the equivalence classes of $\backsim_w$.


  \begin{figure}[!ht]
  \centering
  \includegraphics[width=0.35\textwidth]{rcore.eps} 
\caption{Construction of an embedding from $G_\text{R-core}$ to $G$.}
\label{fig:rcore}
\end{figure}   

\begin{pro}\label{pro:iso}
  If both $G$ and $H$ are R-cores in the same equivalence class of
  $\backsim_w$, then $G$ and $H$ are isomorphic.
\end{pro}

\begin{proof}
  Because both $G$ and $H$ are R-cores, we know that $|V_G|=|V_H|$.

  Consider relations $R_1$ and $R_2$ such that $G\muls R_1=H$ and $H\muls
  R_2=G$. Applying Lemma~\ref{lem:nohall} we know that $R_1$ satisfies the
  Hall condition. Otherwise there would be a graph $G'$ with $|V_{G'}|<
  |V_G|$ so that $G'$ is relationally equivalent to both $G$ and $H$
  contradicting the fact that $G$ and $H$ are R-cores. Similarly, we can
  show that $R_2$ also satisfies the Hall condition.

  From Theorem~\ref{thm:hall} we know that there is a monomorphism $f$ from
  $G$ to $H$, and monomorphism $g$ from $H$ to $G$. It follows that number
  of edges of $G$ is not larger than the number of edges of $H$ and
  vice versa. Because $G$ and $H$ have the same number of edges and
  same number of vertices, $G$ and $H$ must be isomorphisms.
\end{proof}

It thus makes sense to define a construction analogous to the core of a graph.
\begin{definition}
  $H$ is an \emph{R-core of graph $G$}\index{R-core} if $H$ is an R-core and $H\backsim_w
  G$.
\end{definition}

All R-cores of graph $G$ are isomorphic as an immediate consequence of
Proposition~\ref{pro:iso}. We denote the  (up to isomorphism) unique R-core
of graph $G$ by $G_{\text{R-core}}$\index{$G_{\text{R-core}}$}.

\begin{lemma}
  $G_{\text{R-core}}$ is isomorphic to a (not necessarily induced) subgraph
  of $G$.
\end{lemma}

\begin{proof}
  Take any relation $R$ such that $G_{\text{R-core}}\muls R=G$. By the same
  argument as in Corollary~\ref{cor:nohall2}, there is a monomorphism
  $f:G_{\text{R-core}}\rightarrow G$ contained in $R$. Consider the image
  of $f$ on $G$.
\end{proof}

\begin{thm}
  \label{thm:Rcore}
  $G_{\text{R-core}}$ is isomorphic to an induced subgraph of $G$.
\end{thm}

\begin{proof}
%  We firstly prove that $G_{\text{R-core}}$ is isomorphic to a subgraph of $G$, i.e.,
%  there exists a mapping which maps every edge of $G_{\text{R-core}}$ to an edge of
%  $G$. We construct this mapping as follows:
  Fix $R_1$ and $R_2$ such that $G_{\text{R-core}}\muls R_1=G$ and
  $G\muls R_2=G_{\text{R-core}}$.

  $R=R_1\circ R_2$ is a relation such that $G_{\text{R-core}}\muls
  R=G_{\text{R-core}}$. By Corollary~\ref{cor:nohall2}, $R$ contains a
  monomorphism $f:G_{\text{R-core}}\rightarrow G_{\text{R-core}}$. Because
  such a monomorphism is a permutation, there exists $n$ such that $f^n$ is
  identity.

  Put $R_1'=R^{n-1}\circ R_1$. Because $R^{n}$ contains the identity and
  $R^{n}=R_1'\circ R_2$, it follows that for every
  $x\in V_{G_{\text{R-core}}}$, there is a vertex
  $I(x)\in V_G$ such that $I(x)\in R'_1(x)$ and $x\in R_2(I(x))$.
  In other words, $(x,I(x))\in R'_1(x)$ and $(I(x),x)\in R_2$.
  It is easily seen that $I$ is a mapping from vertex set of $G_{\text{R-core}}$
  to vertex set of $G$. We take the induced subgraph of $G$ induced by the image of $I$,
  denoted by $G'$, and claim that $I$ is an isomorphism of $G_{\text{R-core}}$ to $G'$.

  We first show that for two vertices $x\neq y$, we have $I(x)\neq I(y)$ and
  thus $I$ is vertex injective (thus both vertex and edge injective). Assume, that is not the
  case, i.e., that there are two vertices $x\neq y$ such that $I(x)=I(y)$.
  Consider an arbitrary vertex $z$ in the neighbourhood of $x$. It follows
  that $I(z)$ must be in the neighbourhood of $I(x)$ and consequently
  $z$ is in the neighbourhood of $y$. Thus the neighbourhoods of $x$ and $y$
  are the same. By Theorem~\ref{thm:equi}, however, we know that the
  R-core is a point-determining graph (because weak relational equivalence is coarser
  than strong relational equivalence), a contradiction.

  Then we claim that, $I$ is a homomorphism of $G_{\text{R-core}}$ to $G'$, i.e.,
  for every edge $(x,y)\in E_{G_{\text{R-core}}}$ we also have edge
  $(I(x),I(y))\in E_G$. This is because $I\subset R'_1$, then
  $G_{\text{R-core}}=G_{\text{R-core}}\muls I\subset G_{\text{R-core}}\muls R'_1=G$.
%  Hence we proved that $G_{\text{R-core}}$ is isomorphic to a subgraph of $G$.

  It is easily seen from the construction of $I$ that $I$ is vertex surjective.
  Finally we prove that $I$ is also a edge surjective homomorphism by claiming
  $I^{-1}$ is a homomorphism of $G'$ to $G_{\text{R-core}}$.
  We see $I^{-1}\subset R_2$ by observing $x \in R_2(I(x))$ implies $(I(x),x)\ in R_2$ for all $x\in$
  vertex set of $G_{\text{R-core}}$. Because $I$ as well as $I^{-1} $is one-to-one,
  $G'=G'\muls I^{-1}\subset G'\muls R_2=G_{\text{R-core}}$.
  $(I(x),I(y))\in G'$ corresponds to an edge $(x,y)\in
  G_{\text{R-core}}$.

  Hence we proved $I$ is bijective (both edge and vertex) homomorphism, thus $I$ is an isomorphism.
\end{proof}

We close the section with an algorithm computing the R-core of a graph. In
contrast to graph cores, where the computation is known to be NP-complete,
there is a simple polynomial algorithm for R-cores.

Observe that the R-core of a graph containing isolated vertices is isomorphic
to the disjoint union of the R-core of the same graph with the isolated
vertices removed and a single isolated vertex. The R-core of a graph without
isolated vertices can be computed by Algorithm~\ref{alg:Rcore}.

\begin{algorithm}[htb]
\caption{The R-core of a graph}
\label{alg:Rcore}
%\newcommand{\AND}{ $\wedge$ }
\begin{algorithmic}[1]
  \REQUIRE ~~\newline
  Graph $G$ with loops allowed and without isolated vertices,
  vertex set denoted by $V$, neighbourhoods $N_G(i)$, $i\in V$.
  \FOR {$i\in V$}
  \STATE $W(i)= \emptyset$
  \STATE found = FALSE
  \FOR {$j\in V\setminus \{i\}$}
  \IF {$N(j)\subseteq N(i)$}
  \STATE  $W(i):= W(i)\cup N(j)$
  \ENDIF
  \IF {$N(i)\subseteq N(j)$}
  \STATE found = TRUE
  \ENDIF
  \ENDFOR
  \IF {$W(i)=N(i)$ \AND found}
  \STATE delete $i$ from $V$
  \STATE $N(i)= \emptyset$
  \ENDIF
  \ENDFOR
\RETURN  The R-core $G[V]$ of $G$.

\end{algorithmic}
\end{algorithm}

The algorithm removes all vertices $v\in G$ such that (1) the neighborhood
of $v$ is union of neighbourhood of some other vertices $v_1,v_2,\dots, v_n$
and (2) there is vertex $u$ such that $N_G(v)\subseteq N_G(u)$.

It is easy to see that the resulting graph $H$ is relationally equivalent
to $G$. Condition (1) ensures the existence of a relation $R_1$ such that
$H\muls R_1=G$, while the condition (2) ensures the existence of a relation
$R_2$ such that $G\muls R_2=H$.

We need to show that $H$ is isomorphic to $G_{\text{R-core}}$. By Theorem
\ref{thm:Rcore} we can assume that $G_{\text{R-core}}$ is an induced
subgraph of $H$ that is constructed as an induced subgraph of $G$.

We also know that there are relations $R_1$ and $R_2$ such that
$G_{\text{R-core}}\muls R_1=H$ and $G\muls R_2=G_{\text{R-core}}$. By the
same argument as in the proof of Theorem~\ref{thm:Rcore} we can assume both
$R_1$ and $R_2$ to contain an (restriction of) identity.

Now assume that there is a vertex $v\in V_H\setminus
V_{G_{\text{R-core}}}$. We can put $u=R_2(v)$ and because $R_2$ contains an
identity we have $N_G(v)\subseteq N_G(u)$. We can also put
$\{v_1,v_2\ldots v_n\}$ to be the set of all vertices such that $v\in
R_1(v_i)$. It follows that the neighbourhood of $v$ is the union of
neighbourhoods of $v_1,v_2,\ldots, v_n$ and by the construction of $H$ we have $v\notin
V_H$, a contradiction.

\section{The partial order Rel\texorpdfstring{$(G,H)$}{Rel(G,H)}}
\label{sect:poset}

\subsection*{Basic properties}

For fixed graphs $G$ and $H$ we consider partial order $\mathrm{Rel}(G,H)$.
The vertices of this partial order are all relations $R$ such
that $G\muls R=H$. We put $R_1\leq R_2$ if and only if $R_1\subseteq R_2$.

This definition is motivated by Hom-complexes, see~\cite{Matousek2003}. In
this section we show the basic properties of this partial order and
concentrate on minimal elements in the special case of $\mathrm{Rel}(G,G)$.

\begin{pro}
  Suppose $G\muls R'=H$, $G\muls R''=H$ and $R'\subseteq R''$, then any
  relation $R$ with $R'\subseteq R\subseteq R''$ also satisfies $G\muls
  R=H$.
\end{pro}
\begin{proof}
  From $R'\subseteq R\subseteq R''$ we conclude $G\muls R'\subseteq G\muls
  R\subseteq G\muls R''$. Hence $G\muls R'=G\muls R''$ implies $G\muls
  R=H$.
\end{proof}

Hence it is possible to describe the partial order $\mathrm{Rel}(G,H)$ by
listing minimal and maximal solutions $R$ of $G\muls R=H$ w.r.t.\ set
inclusion.

For example, if $G$ is $P_3$ with vertices $v_0,v_1,v_2,v_3$ and $H$ is
$P_1$ with vertices $x_0,x_1$, it is easily seen that
$R''=\{(v_0,x_0),(v_2,x_0),(v_1,x_1),(v_3,x_1)\}$ is a maximal solution of
$G\muls R=H$ and $R'=\{(v_0,x_0),(v_1,x_1)\}$ is a minimal solution,
because $R'\subset R''$, then all the relations $R$ with $R'\subseteq
R\subseteq R''$ satisfy $G\muls R=H$. We note that minimal and maximal
solutions need not be unique.


\subsection*{Solutions of \texorpdfstring{$G\muls R = G$}{G* R = G}}


For simplicity, we say that a relation $R$ is an \emph{automorphism}\index{automorphism} of $G$
if it is of the form $R=\{(x,f(x))\mid x\in V_G\}$ and $f:V_G\to V_G$
is an automorphism of $G$.


We will see that conditions related to thinness again play a major role in
this context. Recall that $G$ is point-determining if no two vertices have the same
neighborhood, i.e., $N_G(x)=N_G(y)$ implies $x=y$. Here we need an even
stronger condition:
\begin{definition}
  A graph $G$ satisfies \emph{condition N}\index{condition N} if $N_G(x)\subseteq N_G(y)$
  implies $x= y$.
\end{definition}
In particular, graphs satisfying condition N are point-determining.

\begin{pro}
  For a given graph $G$, the set $\mathrm{Rel}(G,G)$ of all relations
  satisfying $G\muls R = G$ forms a monoid.
\end{pro}
\begin{proof}
  Firstly, because $G$ is a finite graph, the set $\mathrm{Rel}(G,G)$ is also
  finite. Furthermore, $R,S\in \mathrm{Rel}(G,G)$ implies $G\muls R=G$ and
  $G\muls S=G$ and thus $G\muls (R\circ S)=G$, so that $R\circ S\in
  \mathrm{Rel}(G,G)$. Finally, the identity relation $I_G$ is a left and right
  identity for relational composition: $I_G\circ R=R\circ I_G=R$.
\end{proof}

A relation $R\subset V_G\times V_G$ can be interpreted as a directed graph
$\vec R$ with vertex set $V_G$ and a directed edge $u\rightarrow v$ if and
only if $(u,v)\in R$. Note that $\vec R$ may have loops. We say that $v\in
V_G$ is \emph{recurrent}\index{recurrent} if and only if there exists a walk (of length at
least 1) from $v$ to itself. Let $S_G$ be the set of all the recurrent
vertices. Furthermore, we define an equivalence relation $\xi$ on $S_G$ by
setting $(u,v)\in\xi$ if there are both a walk in $\vec R$ from $u$ to $v$
and from $v$ to $u$. The equivalence classes w.r.t.\ $\xi$ are denoted by
$\vec R/\xi=\{D_1,D_2,\dots,D_m\}$. We furthermore define a binary
relation $\geq$ over $\vec R/\xi$ as follows: if there is a walk from a
vertex $u$ in $D_i$ to a vertex $v$ in $D_j$, then we say $u\geq v$. It is
easily seen that $\geq$ is reflexive, antisymmetric, and transitive, hence
$(\vec R/\xi,\geq)$ is a partially ordered set. W.l.o.g.\ we can assume
$\{D_1, D_2,\dots,D_s\}$ are the maximal elements w.r.t.\ $\geq$. Now let
$G_r=G[D_1\cup\dots\cup D_s]$ be the subgraph of $G$ induced by these
maximal elements.

\begin{lemma}\label{lem:aut1}
For arbitrary $x\in V_G$, there exist $l\in \mathbb{N}$ and a
recurrent vertex $v$ such that $(v,x)\in R^l$, where $R^l$ is $l$-times
composition of relation $R$.
\end{lemma}
\begin{proof}
Set $x_0=x$ and choose $x_i\in R^{-1}(x_{i-1})$ for all $i\ge1$. Since
$|V_G|<\infty$, there are indices  $j,k\in \mathbb{N}$, $j<k$,
$x_j=x_k$. Then $x_j$ is a recurrent vertex. The lemma follows by setting
$l=j$ and $v=x_i$.
\end{proof}

\begin{lemma}\label{lem:aut2}
For every $v\in V_{G_r}$, $R^{-1}(v)\subseteq V_{G_r}$.
\end{lemma}
\begin{proof}
  We prove this by two steps:

  First, we claim that for any $x\in R^{-1}(v)$, $x$ is recurrent.
  Suppose $x\in R^{-1}(v)$ is not recurrent. Lemma~\ref{lem:aut1} implies
  that there is $l\in \mathbb{N}$ and a recurrent vertex $w$ such that
  $(w,x)\in R^l$. Hence the definitions of $E$ and $\geq$ imply $[w]\geq
  [v]$, where $[v]$\index{$[v]$} denotes the equivalent class (w.r.t.\ $E$) containing
  the vertex $v$. Since $[v]$ is maximal w.r.t.\ $\geq$, we have
  $[v]=[w]$. Consequently, there exists an index $k\in \mathbb{N}$ such
  that $(v,w)\in R^k$. On the other hand, we have $(x,x)=(x,v)\circ
  (v,w)\circ (w,x)\in R^{k+l+1}$. Thus, $x$ is recurrent, a contradiction.
  Therefore, every vertex $x\in R^{-1}(v)$ is recurrent.

  Second, we prove $x$ is a maximal element in the partial order.
  Hence $[x]\geq
  [v]$ together with the maximality of $[v]$ gives $[x]=[v]$, and thus
  $x\in V_{G_r}$.
\end{proof}

\begin{lemma}\label{lem:aut3}
  For every $x\in V_G$, there is $l\in \mathbb{N}$ such that, for arbitrary
  $i\geq l$, there exists $u\in V_{G_r}$ satisfying $(u,x)\in R^i$.
\end{lemma}

\begin{proof}
  From Lemma~\ref{lem:aut1} and Lemma~\ref{lem:aut2} we conclude that it is
  sufficient to show that for an arbitrary recurrent vertex $v$ there is a
  $k\in \mathbb{N}$ and $w\in V_{G_r}$ such that $(w,v)\in R^k$. The lemma
  now follows easily from the finiteness of $V_G$.
\end{proof}


Now we introduce a lemma which connects relation $R$ and the neighborhood of vertex in a graph.
The lemma is of simple but very useful.
\begin{lemma}\label{lem:aut4}
 Suppose $G\muls R = H$. For any $u,v\in V_H$, if $R^{-1}(u)\subseteq R^{-1}(v)$, then $N_H(u)\subseteq N_H(v)$.
\end{lemma}

\begin{proof} 
 Suppose there exist $u,v\in V_H$, $R_{-1}(u)\subseteq R_{-1}(v)$ but $N_H(u)\nsubseteq N_H(v)$,
 then there exist a vertex $w$ of $H$, $w\in N_H(u)$ but $w\notin N_H(v)$. Because $(u,w)$ is an edge
 in $H$ and $G\muls R = H$, we can find $x,y\in V_G, x\in R_{-1}(w), y\in R_{-1}(u)$ and $(x,y)$ is an edge in $G$.
 $R_{-1}(u)\subseteq R_{-1}(v)$ implies $y\in R_{-1}(v)$. We already have $(x,w)\in R$ and $(x,y)$ is an edge in $G$,
 by the definition of $\muls$ we have $(v,w)$ is an edge of $H$, which contradicts to $w\notin N_H(v)$.
\end{proof}

%we need to change the prove for using the lemma.


From these lemmata we can deduce:
\begin{thm} \label{thm:auto1}
All solutions of $G\muls R=G$ are
automorphisms if and only if $G$ has property N.
\end{thm}
\begin{proof}
  Suppose there are distinct vertices $x,y\in V_G$ such that $N_G(x)\subseteq
  N_G(y)$. Then $R=I_G\cup(x,y)$, which is not functional, satisfies $G\muls
  R=G$. Thus $G\muls R=G$ is also solved by relations that are not
  automorphisms of $G$. This proves the `only if' part.

  Conversely, suppose $G$ has property N. \textbf{Claim:} There is a
  $k\in\mathbb{N}$ such that $R^k\cap (V_{G_r}\times V_{G_r})=I_{G_r}$.

  For each $v_i\in V_{G_r}$ there is a walk of length $s_i\ge1$ from $v_i$
  to itself. Hence $(v_i,v_i)\in R^{s_i}$. Let $s$ be the least common
  multiple of all the $s_i$. Then $(v_i,v_i)\in R^s$ for all $v_i\in V_{G_r}$.
  Define $Q:=R^s\cap(V_{G_r}\times V_{G_r})$. Thus $I_{G_r}\subseteq Q$ and
  moreover $Q^j\subseteq Q^{j+1}$ for all $j\in\mathbb{N}$. Since $V_{G_r}$
  is finite there is an $n\in\mathbb{N}$ such that $Q^{n+1}=Q^{n}$, and
  hence $Q^{2n}=Q^n$. Let us write $R^{-i}(v):=\{u\in V_G:(u,v)\in
  R^i\}$. For $v\in V_{G_r}$ we have $R^{-i}(v)\in V_{G_r}$ (from Lemma
 ~\ref{lem:aut2}) and hence $Q^{-n}(v)=R^{-sn}(v)$ for all $v\in V_{G_r}$.
  If $Q^n\neq I_{G_r}$, then there are two distinct vertices $u,v\in
  V_{G_r}$, such that $(u,v)\in Q^n$. From Lemma~\ref{lem:aut4} $N_G(u)\nsubseteq N_G(v)$ and $G=G\muls
  R^{sn}$ allows us to conclude that $R^{-sn}(u)\nsubseteq R^{-sn}(v)$ and
  $R^{-sn}(v)\nsubseteq R^{-sn}(u)$. Hence, there is a vertex $w$, such
  that $(w,u)\in Q^n$ and $(w,v)\notin Q^n$. From $(u,v)\in Q^n$ and
  $(w,u)\in Q^n$ we conclude $(w,v)\in Q^n\circ Q^n=Q^{2n}$, contradicting
  to $Q^{2n}=Q^n$. Therefore $Q^n=I_{G_r}$. Setting $k=sn$ now implies the
  claim.

  Finally, we show $V_{G_r}=V_G$. For any $v\in V_G\setminus V_{G_r}$,
  Lemma~\ref{lem:aut3} implies the existence of $w\in V_{G_r}$ and $m\in
  \mathbb{N}$ such that $(w,v)\in R^{mk}$. However, we have claimed
  $R^{-k}(w)=\{w\}$, hence $R^{-mk}(w)=\{w\}$. From Lemma \label{lem:auto4}, this, however, implies
  $N_G(w)\subseteq N_G(v)$ and thus contradicts property N. Therefore,
  $V_G=V_{G_r}$ and moreover $R^k=I_G$. This $R$ is an automorphism.
\end{proof}

\section{R-Retractions}
\label{sect:retraction}

Recall that a particularly important special case of ordinary graph homomorphisms are
homomorphisms to subgraphs, and in particular so-called retractions: Let
$H$ be a subgraph of $G$, a \emph{retraction}\index{retraction} of $G$ to $H$ is a
homomorphism $r: V_G\rightarrow V_H$ such that $r(x)=x$ for all $x\in
V_H$.

We introduced the graph cores in section~\ref{sect:retract} as minimal
representatives of the homomorphism equivalence classes. The classical and
equivalent definition is the following: A \emph{(graph) core}\index{core} is a graph
that does not retract to a proper subgraph. Every graph $G$ has a unique
core $H$ (up to isomorphism), hence one can speak of $H$ as \emph{the core
  of}\index{the core} $G$, see~\cite{Hell2004}.

Here, we introduce a similar concept based on relations between graphs.
Again to obtain a structure related to graph homomorphisms, in this section
we require all relations to have full domain unless explicitly stated
otherwise.

\begin{definition}
  Let $H$ be a subgraph of $G$. An \emph{R-retraction}\index{R-retraction} of $G$ to $H$ is a
  relation $R$ such that $G\muls R=H$ and $(x,x)\in R$ for all $x\in
  V_H$. If there is an R-retraction of $G$ to $H$ we say that $H$ is a
  \emph{retract}\index{retract} of $G$.
\end{definition}

\begin{lemma}\label{lem:ret}
  If $H$ is an R-retract of $G$ and $K$ is an R-retract of $H$, then $K$ is
  an R-retract of $G$.
\end{lemma}

\begin{proof}
  Suppose $T$ is an R-retraction of $H$ to $K$ and $S$ is an
  R-retraction of $G$ to $H$. Then $(G\muls S)\muls T=G\muls (S\circ
  T)=K$. Furthermore $(x,x)\in T$ for all $x\in V_K\subseteq V_H$, and
  $(u,u)\in S$ for all $u\in V_H$, hence $(x,x)\in S\circ T$ for all $x\in
  V_k$. Therefore $S\circ T$ is an R-retraction from $G$ to $K$.
\end{proof}

Hence, the following definition is meaningful.
\begin{definition}
  A graph is \emph{R-reduced}\index{R-reduced} if there is no R-retraction to a proper
  subgraph.
\end{definition}
Thus, we can also speak about `the R-reduced graph of a graph $G$' as the
smallest subgraph on which it can be retracted. We will see below that the
R-reduced graph of a graph is always unique up to isomorphism.

We remark that R-reduced graphs differs from R-cores introduced
in section~\ref{sect:retract}, thus we chose an alternative name used
also in homomorphism setting (cores are also called reduced graphs).

\begin{lemma}
  Let $G$ be a graph with loops and $o$ a vertex of $G$ with a loop on
  it. Then the R-reduced graph of $G$ is the subgraph induced by $\{o\}$.
\end{lemma}

\begin{proof}
  Let $O$ be the graph induced by $\{o\}$, and $R=\{(x,o)\mid x\in V_G\}$, then
  it is easily seen $R$ is an R-retraction of $G$ to $O$. Moreover, since
  $O$ has only one vertex, thus there is no R-retraction to its
  subgraphs. So $O$ is an R-reduced graph of $G$.

  Conversely, let $H$ be an R-reduced graph of $G$ and denote by $R$ the
  R-retraction from $G$ to $H$. Then a loop of $G$ must generate a loop of
  $H$ via $R$, denote it by $O$. Similarly to above, we see $O$ is an
  R-retract of $H$, hence it is also an R-retract of $G$ (by Lemma~\ref{lem:ret}).
  Therefore the definition of R-reduced graph implies
  $H=O$.
\end{proof}

In the remainder of this section, therefore, we will only consider graphs
without loops.

\begin{lemma} \label{lem:core}
  If $G$ is R-reduced, then $G$ has property N.
\end{lemma}
\begin{proof}
  Suppose there are two distinct vertices $x,y\in V_G$ with $N_G(x)\subseteq
  N_G(y)$ and consider the induced graph $G/x:=G[V_G\setminus\{x\}]$ obtained
  from $G$ by deleting the vertex $x$ and all edges incident with $x$. The
  relation $R=\left\{(z,z)\mid z\in V_G\setminus\{x\}\right\}\cup\{(x,y)\}$
  satisfies $G\muls R=G/x$: the first part is the identity on $G/x$ and
  already generates all necessary edges in $G/x$. The second part
  transforms edges of the form $(x,z)\in E_G$ to edges $(y,z)$. Since $R$
  has full domain and contains the identity relation restricted to
  $G/x$, it is an R-retraction of graph $G$, and hence $G$ is not R-reduced.
\end{proof}

\begin{pro} \label{pro:core}
  A graph $G$ is R-reduced if and only if it has no relation to a proper
  subgraph.
\end{pro}

\begin{proof}
  The `if' part is trivial. Now we suppose that $H$ is a proper induced
  subgraph of graph $G$ with the minimal number of vertices such that there
  is a relation $R$ satisfying $G\muls R=H$. Then $H$ does not have a
  relation to a proper subgraph of itself. We claim that $H$ has property
  N; otherwise, one can find a vertex $u\in V_H$ and construct a retraction
  from $H$ to $H/{u}$ as in Lemma~\ref{lem:core}, which causes a
  contradiction. Denote $\widetilde{R}=R\cap (V_H\times V_H)$, then
  $K=H\muls\widetilde{R}$ is a subgraph of $H$. From our assumptions on $H$ we
  obtain $K=H$. By virtue of Theorem~\ref{thm:auto1}, $\widetilde{R}$ is
  induced by an automorphism of $H$. Hence $R\circ \widetilde{R}^{+}$ is again
  a relation of $G$ to $H$ that contains the identity on $H$, i.e., it is
  an R-retraction.
\end{proof}

Since graph cores are induced subgraphs and retractions are surjective they
also imply relations. Proposition~\ref{pro:core} is also a consequence of
this fact. We refer to~\cite{Hell2004} for a formal proof.

\begin{figure}[!ht]
\centering
   \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{core.eps} \\
    \hspace{0.85cm}   $G$ \hspace{4cm} $G_\text{core}$
    \end{tabular}
\caption{A graph $G$ and its core.}
\label{fig:core}
\end{figure}

We call $R$ an \emph{minimal R-retraction}\index{minimal R-retraction} if there is no
R-retraction $R'$ such that $R\supset R'\supset I_H$.

\begin{lemma} \label{fun}
  Let $H$ be an R-retract of $G$. Then any minimal
  R-retraction of $G$ to $H$ is functional.
\end{lemma}
\begin{proof}
  Suppose $R$ is a minimal R-retraction of $G$ to $H$. If $R$ is not
  functional, then there exist distinct $x,y\in V_H$ such that
  $(u,x),(u,y)\in R$. Hence we could always pick a vertex from $\{x,y\}$
  which is different of $u$, w.l.o.g.\ suppose it is $x$. Then $R/(u,x)$ is
  an R-retraction, which contradicts minimality. To see this, set
  $R'=R/(u,x)$, then $R\supset R'\supset I_H$ and moreover $H=G\muls I_H
  \subseteq G\muls R'\subseteq G\muls R=H$, and thus $G\muls R'=H$.
\end{proof}


\begin{pro}
  A graph is R-reduced if and only if it is a graph core.
\end{pro}
\begin{proof}
  If $H$ is R-reduced from $G$ there is an R-retraction from $G$ to $H$
  which can be chosen minimal and hence by Lemma~\ref{fun} is functional
  and hence is a homomorphism retraction. Conversely, a homomorphism
  retraction is also an R-retraction. Hence the R-reduced graphs coincide
  with the graph cores.
\end{proof}

\begin{pro}
  Suppose $H$ is the core of graph $G$. If $H\muls R=K$ then there is a
  relation $R'$ such that $G\muls R'=K$. If $K\muls S=G$, then there is a
  relation $S'$ such that $K\muls S'=H$.
\end{pro}
\begin{proof}
  Since $H$ is the core of graph $G$, there is a relation $R_1$ such that
  $G\muls R_1=H$. If $H\muls R=K$ we have $G\muls R_1\muls R=K$ and
  $R'=R_1\circ R$ satisfies $G\muls R'=K$. If $K\muls S=G$ we have
  $K\muls S\muls R_1=H$ and $S'=S\circ R_1$ satisfies $K\circ S'=G$.
\end{proof}

\subsection*{Cocores}

In the classical setting of maps between graphs, one can only consider
retractions from a graph to its subgraphs, since graph homomorphisms of an
induced subgraph to the original graph are just the identity maps. In the
setting of relations between graphs, however, it appears natural to
consider relations with identity restriction between a graph and an induced
subgraph. This gives rise to notions of R-coretraction and R-cocore in
analogy with R-retractions and R-reduced graphs.

\begin{definition}
  Let $H$ be a subgraph of graph $G$. An \emph{R-coretraction}\index{R-coretraction} of $H$ to $G$ is
  a relation $R$ such that $H\muls R=G$ and $(x,x)\in R$ for all $x\in
  V_H$. We say that $H$ is an \emph{R-coretract}\index{R-coretract} of $G$.
\end{definition}

\begin{lemma}
  If $H$ is an R-coretract of graph $G$ and $K$ is an R-coretract of $H$, then
  $K$ is an R-coretract of $G$.
\end{lemma}
\begin{proof}
  Suppose $T$ is an R-coretraction of $K$ to $H$ and $S$ is an
  R-coretraction of $H$ to $G$. Then $(K\muls T)\muls S = K\muls(T\circ
  S)=G$. Furthermore $(x,x)\in T$ for all $x\in V_K\subseteq V_H$, and
  $(v,v)\in S$ for all $v\in V_H$, hence $(x,x)\in T\circ S$ for all $x\in
  V_K$. Therefore $T\circ S$ is an R-coretraction from $K$ to $G$.
\end{proof}

Hence, the following definition is meaningful.
\begin{definition}
  An R-coretract $H$ of a graph $G$ is an \emph{R-cocore of $G$}\index{R-cocore} if $H$
  does not have a proper subgraph that is an R-coretract of $H$ (and hence
  of $G$).
\end{definition}

\begin{figure}[!ht]
\centering
\subfloat[$G$]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.7\textwidth]{core1.eps}
\end{minipage}}
\subfloat[$\mathrm{cocore}(G)$ ]{
\begin{minipage}[c]{0.3\textwidth}
\centering
\includegraphics[width=0.7\textwidth]{cocore1.eps}
\end{minipage}}
 \caption{A graph and its cocore.}
  \label{fig:cocore}
\end{figure}



Clearly, the reference to $G$ is irrelevant: A graph $G$ is an
\emph{R-cocore}\index{R-cocore} if there is no proper subgraph of $G$ that is an
R-coretract of $G$. Similarly, we call $R$ to be a \emph{minimal
  R-coretraction}\index{minimal R-coretraction} of $H$ to $G$ if there exists no R-coretraction $R'$,
such that $R'\subset R$.

\begin{lemma}\label{lem:cocore}
  Let $H$ be an R-coretract of graph $G$, and let $R$ be a minimal
  R-coretraction of $H$ to $G$. Then the restriction of $R$ to $H$ equals
  $I_H$.
\end{lemma}
\begin{proof}
  Suppose $R\cap (V_H\times V_H)\neq I_H$ and define $R_1=R\setminus
  \{(x,y)\in R:x,y\in V_H,x\neq y\}$. Then $H\muls R_1\subseteq H\muls
  R=G$. We claim that $H\muls R_1=H\muls R$ and thus $R_1$ is an
  R-coretraction of $H$ to $R$, contradicting the minimality of $R$.

  To prove this claim, it is sufficient to show that any edge $e\in E_G$ is
  contained in $H\muls R_1$. If $e$ is not incident with any vertex in
  $V_H$ or $e\in E_H$, the conclusion is trivial. So we only need to
  consider $e=(z,u)$ with $z\in E_H$ and $u\in V_G\setminus V_H$. Since
  $G=H\muls R$, one can find $x_1,x_2\in V_H$ such that $(x_1,z),(x_2,u)\in
  R$ and $(x_1,x_2)\in E_H$. Because $H\subseteq H\muls\big(I_H\cup
  (x_1,z)\big)\subset H\muls\big(R\cap (V_H \times V_H)\big)=H$, we get
  $N_H(x_1)\subseteq N_H(z)$. It follows that $(z,x_2)\in E_H$ and
  hence $e=(z,u)\in G\muls R_1$.
\end{proof}

Like R-reduced graphs, R-cocores also satisfy a stringent condition on their
neighbourhood structure.

\begin{definition} \label{nei}
  A graph $G$ satisfies property N* if, for every vertex $x\in V_G$,
  there is no subset $U_x\subseteq V_G\setminus\{x\}$ such that
  \begin{equation*}
    N_G(x)=\bigcup_{y\in U_x} N_G(y)
  \end{equation*}
\end{definition}
In other words, no neighbourhood can be represented as the union of
neighbourhoods of other vertices of graph $G$.

\begin{pro} \label{cocore} $G$ is an R-cocore if and only if $G$ has
  property N*.
\end{pro}
\begin{proof}
  Consider a vertex set $U_x$ as in Definition~\ref{nei} and suppose
  that there is a vertex $x\in V_G$ such that $N_G(x)=\bigcup_{y\in U_x}
  N_G(y)$. Then the relation $R:=I\setminus(x,x)\cup\{(y,x):y\in U_x\}$ is an
  R-coretraction from $G/x$ to $G$. Thus $G$ is not an R-cocore.

  Conversely, suppose that $G$ is not an R-cocore, let $H$ be a coretract
  of $G$, and denote by $R$ a minimal R-coretraction of $H$ to $G$. Then,
  by Lemma~\ref{lem:cocore}, $R\cap (V_H\times V_H)=I_H$. Consider a
  vertex $v\in V_G\setminus V_H$ and set
  $R^{-1}(v)=\{x_1,\dots,x_i\}$. Then $N(v)=\bigcup_i N(x_i)$, contradicting
  property N*.
\end{proof}

\begin{lemma} \label{thin-cocore1}
 An R-cocore of graph $G$ is isomorphic to an R-cocore of $G_{\text{pd}}$.
\end{lemma}
\begin{proof}
 Suppose graph $H$ is an R-cocore of graph $G$, then there exists a coretraction $R$
 such that $H\muls R = G$. By the definition of $G_{\text{pd}}$, we know
 there exists an R-retraction $R'$ such that $G\muls R'=G_{\text{pd}}$.
 Then $H\muls (R\circ R') = G$. It is easily seen that $R\circ R'$ is a coretraction.
 And $H$ is the smallest subgraph of $G_{\text{pd}}$ which has a coretraction
 to $G_{\text{pd}}$, otherwise, suppose there are smaller graph $K$ such that $K$
 has a coretraction to $G_{\text{pd}}$, then $K$ also has a coretraction to $G$,
 which contradicts to the assumption that $H$ is an R-cocore.
 Therefore, $H$ is an R-cocore of $G_{\text{pd}}$.

 Conversely, if $H$ is an R-cocore of graph $G_{\text{pd}}$, then it is also
 an R-cocore of $G$.
\end{proof}

We call a subset $B$ of $V_G$ is a \emph{basis}\index{basis} of graph $G$, if for any $x\in V_G$, there
 exists a subset $U_x$ of $B$ such that $N_G(x)=\bigcup_{y\in U_x} N_G(y)$. Of course
 a basis of a graph always exists, because $V_G$ is a basis of $G$. We call a basis of graph $G$
 with minimal cardinality a \emph{minimal basis}\index{minimal basis}. Because we consider only finite graphs,
 a minimal basis always exists. Now we prove that minimal basis of a point-determining graph $G$ is unique.


\begin{lemma} \label{basis}
 Minimal basis of a point-determining graph $G$ is unique.
\end{lemma}


\begin{proof}
  Assume there are two distinct minimal basis $A,B$. Neither
  contains the other by their minimality. Because $A,B$ are distinct,
  there exists an element $a\in A$ and $a\notin B$.

  $B$ is a basis of graph $G$, by the definition, there is a set $U_a\subset B$ such that
  $N_G(a)=\bigcup_{b\in U_a} N_G(b)$, thus $|N_G(a)|\geq |N_G(b)|$
  for all $b\in U_a$. Since $G$ is a point-determining graph, any two vertices of $G$ do not
  have the same neighbourhood, thus $|N_G(a)|>|N_G(b)|$
  for all $b\in U_a$. Because $A$ is also a basis of graph $G$, then for any $b\in U_a$,
  $N_G(b)$ can be represented as the union of the neighbourhood of some elements of $A\setminus\{x\}$,
  $a$ is not contained since $|N_G(a)|>|N_G(b)|$. Thus $N_G(a)=\bigcup_{b\in U_a} N_G(b)$ can
  be represented as the union of the neighbourhood of some elements of $A\setminus\{x\}$, which contradicts
  to the minimality of $A$.
\end{proof}


\begin{lemma} \label{thin-cocore2}
 R-cocore of a point-determining graph is unique.
\end{lemma}

\begin{proof}
 From Lemma~\ref{basis}, we know basis of a point-determining graph is unique. We claim that the vertex set of
 any R-cocore of graph $G$ is the minimal basis of $G$. First,
 if $H$ is a R-cocore, then $V_H$ is a basis of graph $G$. Because by the definition of R-cocore,
 there is a coretraction $R$ such that $H\muls R = G$. For any vertex $x\in V_G$, we assign
 $U_x=R^{-1}\subset V_H$, it is easily seen that $N_G(x)=\bigcup_{y\in U_x} N_G(y)$.

 Then we prove $V_H$ is the minimal basis. Suppose there exists a subset $K$ of $V_G$ is a basis,
 and the cardinality of $K$ is smaller than $V_G$. By the definition of basis, for any $x\in V_G$
 we fix the set $U_x$, then there is an R-coretraction from $H$ to $G$, induced by $R(x)=\{y\in V_G\mid x\in U_y\}$.
 That is because for any vertex $x\in K$, we have $U_x=\{x\}$. It contradicts to the assumption that
 $H$ is a cocore.

 Therefore R-cocore of a point-determining graph is unique.
\end{proof}
% Now we prove that the subgraph $H$ induced by the minimal basis $B$ of thin graph $G$ is a R-cocore.
% Fix a set $U_x$ for each $x\in V_G$,
% then there is an R-coretraction from $H$ to $G$, induced by $R(x)=\{y\in V_G|x\in U_y\}$. That is because
% for any vertex $x\in B$, $U_x=\{x\}$. And it is easy to check that $H\muls R = G$.
% We claim $H$ is a minimal subgraph of $G$ which has an R-coretraction to $G$. Otherwise,




Because $G_{\text{pd}}$ is a point-determining graph, from lemma~\ref{thin-cocore2} that $G_{\text{pd}}$
has unique R-cocore for any graph $G$. And from lemma~\ref{thin-cocore1} we immediately get the
following proposition.

\begin{pro}
  R-cocore of $G$ is unique up to isomorphism.
\end{pro}
\iffalse
\begin{proof}
  We denote by $\mathcal{N}$ the collection of all open neighbourhoods of
  vertices in $G$, i.e.,
  $\mathcal{N}=\{N_G(x_1),N_G(x_2),\dots,N_G(x_k)\}$, where
  $V_G=\{x_1,x_2,\dots,x_k\}$. From the definition of the R-cocore we
  know that the subcollection $\mathcal{M}$ of $\mathcal{N}$ consisting of
  all the open neighbourhoods of vertices in R-cocore is a basis of
  $\mathcal{N}$, i.e., any set in $\mathcal{N}$ can be expressed by the
  union of some sets in $\mathcal{M}$. W.l.o.g., we denote the vertex set
  in an R-cocore $C$ of $G$ is $\{x_1,x_2,\dots,x_m\}$ where ${m\leq k}$,
  then $\mathcal{M}=\{N_G(x_1),N_G(x_2),\dots,N_G(x_m)\}$. We claim that
  any element in $\{N_G(x_1),N_G(x_2),\dots,N_G(x_m)\}$ cannot be
  expressed as the union of other elements, i.e., $\mathcal{M}$ is a
  minimal basis. Otherwise, w.l.o.g., suppose
  ${N_G(x_1)=\bigcup_{x_k}N_G(x_k)}$, ${x_k\in \{x_2,\dots,x_m\}}$. For any $1\leq
  k\leq m$, $N_G(x_k)=N_C(x_k)$ or $N_G(x_k)=N_C(x_k)+{\{x_i\mid (x_i,x_k)\in
  E_G, m+1\leq i\leq n\}}$, so either $N_C(x_1)=\cup_{x_k}N_C(x_k),{x_k\in
  \{x_2,\dots,x_m\}}$ or $N_C(x_1)=\cup_{x_k}N_C(x_k)+\{x_i\mid i\in 1,\dots,
  n\},{x_k\in \{x_2,\dots,x_m\}}$, the former contradicts to Proposition~\ref{cocore},
  which implies any element in
  ${\{N_C(x_1),N_C(x_2),\dots,N_C(x_m)\}}$ cannot be expressed as the union
  of other elements, the latter is impossible because $\{x_i\mid i\in 1,\dots,
  n\}\nsubseteq C$.

  Now we prove that this minimal basis is unique. Note that in
  $\mathcal{N}$ we view any vertex with the same neighbourhood as the same,
  since any vertex in R-cocore has different neighbourhoods. Let us
  consider two minimal sub-collections $\mathcal{A},\mathcal{B}$. Neither
  contains the other by their minimality. Since everything is finite, let
  $A\in \mathcal{A}/\mathcal{B}$ be an element of minimal size. Now
  $A$ can be expressed as a union of elements of $\mathcal{B}$, which all
  need to be of smaller cardinality than $A$ (or same but $A\notin
  \mathcal{B}$), but $\mathcal{A}$ then contains all of them, letting $A$
  be expressed by a union of elements of $\mathcal{A}$ contradicting the
  minimality of $\mathcal{A}$.
\end{proof}
\fi

These results allow us to construct an algorithm that computes the cocore
of given graph $G$ in polynomial time. First observe that the cocore of a
graph $G$ that contains isolated vertices is the disjoint union of cocore
of the graph $G'$ obtained from $G$ by removing isolated vertices and the
graph consisting of a single isolated vertex. It is thus sufficient to
compute cocores for graphs without isolated vertices in Algorithm
\ref{alg1}.

\begin{algorithm}[htb]
\caption{The cocore of a graph}
\label{alg1}
\begin{algorithmic}[1]
  \REQUIRE ~~\\
  Graph $G$ with loops and without isolated vertices specified by its
  vertex set $V$ and the neighbourhoods $N_G(i)$, $i\in V$.
  \FOR{$i\in V$}
    \STATE $W(i)= \emptyset$
    \FOR {$j\in V\setminus \{i\}$}
      \IF {$N(j)\subseteq N(i)$}
        \STATE  $W(i):= W(i)\cup N(j)$
      \ENDIF
     \ENDFOR
    \IF {$W(i)=N(i)$}
      \STATE delete $i$ from $V$
      \STATE $N(i)= \emptyset$
    \ENDIF
  \ENDFOR
\RETURN $G[V]$, the cocore of $G$.
\end{algorithmic}
\end{algorithm}

\begin{pro}
  Suppose $H$ is a cocore of $G$. If $K\muls R=H$, then there is a relation
  $R'$ such that $K\muls R'=G$. If $G\muls S=K$, then there is a relation
  $S'$ such that $H\muls S'=K$.
\end{pro}
\begin{proof}
  Since $H$ is a cocore of $G$, there exists an R-coretraction $R_1$ such
  that ${H\muls R_1=G}$. If $K\muls R=H$, then letting $R'=R\circ R_1$ implies
  $K\muls R'=G$. If $G\muls S=K$, we have $H\muls R_1\muls S=K$. Let
  $S'=R_1\circ S$, then $H\muls S'=K$.
\end{proof}


We can find a graph which is not an R-core, and at the same time it does not satisfy the
Hall condition. To see that, consider the graph $G$ in the example of Fig.~\ref{fig:weak}.
Obviously $R=\{(1,1),(2,2),(3,2),(4,4),(6,6),(5,3),(7,3),(5,5),(7,7)\}$
satisfies $G\muls R=G$. For the subset $S=\{2,3\}$ of $V(G)$, $R(S)=\{2\}$,
so $|R(S)|<|S|$, it does not satisfy the Hall condition. But not all graphs which
is not R-core does not satisfy the Hall condition, that means, the condition of
Corollary~\ref{cor:nohall2} is not sufficient. To see this, we
consider a graph consisting of two independent isolated vertices.

Note that relations from R-core or R-cocore to itself also satisfy the Hall condition.

\begin{pro}
If $G$ is an R-core, and relation $R$ satisfying $G\muls R = G$,
then any monomorphism $f\subset R$ satisfies $G\muls f = G$.
\end{pro}

\begin{proof}
From corollary~\ref{cor:nohall2} we know that $R$ which is a relation from
an R-core to itself satisfies the Hall condition
thus it contains a monomorphism. Suppose  $G\muls f \neq G$, then $G\muls f \subset G$.
By iteration we have $G\muls f^m \subset G$ for any $m$.
On the other hand, $f$ is a permutation, then there exists a $n$ such that $f^n$ is identity, thus
$G\muls f^n = G$. A contradiction.
\end{proof}

%\begin{pro}
% If $G\muls R = G$, and all solutions satisfy the Hall condition, then either of the two cases happens:
%\begin{enumerate}
 %\item $G$ is an $R$-core;
 %\item There is a solution contains a relation with non-full domain.
%\end{enumerate}
%\end{pro}

%\begin{proof}
%Suppose neither happens, then $G$ is not an $R$-core and all the relations are with full domain.
%Because $G$ is not an $R$-core, from the definition of $R$-core, we can find an induced subgraph $H$ of $G$ such that
%there is a relation $R_1$ satisfying $H\muls R_1 =G$
 % \begin{equation*}
  %  R(x)=
   % \begin{cases} R_1(x) \text{   for $x\in V_H$,}\\
    %  x \text{   otherwise,}
    %\end{cases}
    %\end{equation*}
    %thus $R$ is a non-full domain relation from
%$G$ to itself.

%It is easily seen that $R$ is a relation from $G$ to itself with full domain and it contains $R_1$.
%\end{proof}


Without the constraint of $R$ with full domain, we have:
\begin{pro}
All solutions of $G\muls R =G$ satisfy the Hall condition if and only if
$G$ is an R-cocore.
\end{pro}

\begin{proof}
If $G$ is an R-cocore, then all the solutions of $G\muls R = G$ are with full domain.
Note that $G$ is an R-cocore thus it is also an R-core,
from Corollary~\ref{cor:nohall2} we know that all solutions $R$ satisfy the
Hall condition.

Conversely, if all solutions satisfy the Hall condition, then all the solutions have full domains,
Hence $G$ is an R-cocore, otherwise we can find an induced subgraph $H$ of $G$ and a relation $R$
satisfying $H\muls R =G$. This relation $R$ is also the solution of $G\muls R = G$ in general (without constraint of
full domain) case.
\end{proof}

%Note that in the example(which?????), every relation contains a full relation.

Actually, it is very easy to get the following result which characterize the cases when all the solutions satisfy the Hall condition:
\begin{pro}
 If $G\muls R = G$, and all solutions satisfy the Hall condition, then either of the two cases happens:
\begin{enumerate}
 \item $G$ is an $R$-core;
 \item There is a solution contains a relation with non-full domain.
\end{enumerate}
\end{pro}

\subsection*{Inclusion relation}

Figure~\ref{fig:inclu} shows the inclusion relation of cores, R-cores, R-cocores, graphs with property N and point-determining graphs: the set of cores is a proper subset of the set of graphs with property N, which is a proper subset of R-cocores. The latter is a proper subset of R-cocores, the set of R-cores is a proper subset of the set of point-determining graphs.

  {\floatstyle{plain}\restylefloat{figure}%
   \begin{figure}[ht!]
   \centering
  \includegraphics[width=0.6\textwidth]{conclu.eps} 
\caption{Inclusion digram}
\label{fig:inclu}
   }{\end{figure}}


\begin{example}
We also give list of examples to illustrate the proper inclusion relations, some of the examples are already shown or been explained before:
\begin{enumerate}
\item $K_3$ is a core, then of course it has property N and is a R-core, R-cocore and point-determining graph.
\item $C_6$ has property N but is not a core. Its core is $P_2$.
\item $P_4$ is an R-cocore but not with property N.
\item The graph $H$ in Figure~\ref{fig:glo} is a R-core but not an R-cocore, its R-cocore is $P_4$.
\item The graph in Figure~\ref{figa:weak} is a point-determining graph but not an R-core.
\end{enumerate}
\end{example}


\subsection*{Lattice decomposition}

Recall that a \emph{lattice}\index{lattice} is a partially ordered set in which any two elements have a \emph{supremum}\index{superemums}
(also called a \emph{least upper bound}\index{least upper bound} or \emph{join}\index{join}) and an \emph{infimum}\index{infimum}
(also called a \emph{greatest lower bound}\index{greatest lower bound} or \emph{meet}\index{meet}).

Lattices structures are well studied in~\cite{Davey2002}. Generally the partial order $\mathrm{Rel}(G,H)$ is not a lattice, but in some case it is. In this subsection we will study the
structures of lattices in the partial order of $\mathrm{Rel}(G,H)$.

Note that graph homomorphism orders are lattice. And locally constrained homomorphism are semi-lattice.

\begin{obs}
There is some observations about $\mathrm{Rel}(G,G)$:
\begin{enumerate}
\item If $G$ is a rigid graph, i.e., a graph has identity as the only automorphism, then $\mathrm{Rel}(G,G)$ is a trivial lattice (a lattice with only one vertex).
\item If $G$ is with property N, then $G$ can be decomposed into $k$ trivial lattices, where $k$ is the number of automorphism of $G$.
\end{enumerate}
\end{obs}



\section{Computational complexity}
\label{sect:complexity}

In this section we briefly consider the complexity of computational
problems related to graph homomorphisms.
For the readers who do not familiar with computational complexity,
please refer to Appendix A. The \emph{homomorphism problem}\index{homomorphism problem}
$\Homo(H)$\index{$\Homo(H)$} takes as input some finite $G$ and asks whether there is a
homomorphism from $G$ to $H$. The computational complexity of the
homomorphism problem is fully characterized. It is known that $\Homo(H)$ is
NP-complete if and only if $H$ has no loops and contains odd cycles. All
the other cases are polynomial, see~\cite{Hell2004}.

The analogous problem for relations between graphs can be phrased as
follows: The \emph{full relation problem}\index{homomorphism problem} $\FulRel(H)$\index{$\FulRel(H)$} takes as input
some finite $G$ and asks whether there is a relation with full domain from
$G$ and asks whether there is a relation from $G$ to $H$. We show that
this problem can be easily converted to a related problem on surjective
homomorphisms. The \emph{surjective homomorphism problem}\index{surjective homomorphism problem} $\sHom(H)$\index{$\sHom(H)$}
takes as input some finite $G$ and asks whether there is a surjective
homomorphism from $G$ to $H$.

Let $\leq_\text{P}^\text{Tur}$ indicate polynomial time Turing reduction.

\begin{thm} \label{thm:complex}
For finite $H$ our relation problem sits in the following relationship.
\begin{equation}
  \Homo(H)\leq_\text{P}^\text{Tur} \FulRel(H)
  \leq_\text{P}^\text{Tur} \sHom(H)\,.
\end{equation}
\end{thm}

\begin{proof}
  First we show that $\Homo(H)$ is polynomially reducible to $\FulRel(H)$.
  If there is a homomorphism from $G$ $H$, then there is also a surjective
  homomorphism from $G+H$ to $H$. On the other hand, suppose $G$ has no
  homomorphism to $H$, from Lemma~\ref{reho} we conclude that $G+H$ has no
  relation to $H$ since $G$ has no relation to $H$.

  Now we show that the relation problem $\FulRel(H)$ is polynomially reducible to $\sHom(H)$.
  From Corollary~\ref{DeCo} we know $G\muls R = H$ if and only if there is
  a graph $G'=G\muls R_D$ which has a full homomorphism to $G$ and has a
  surjective homomorphism to $H$.

  We construct $G''$, by duplicating all the vertices of $G$ precisely
  $|V_H|$ times. We claim that $G'$ exists if and only if
  $G''$ has a full homomorphism to $G$, because we can put
  $G'=G''$ because the surjective homomorphism can easily undo the
  redundant duplications. This gives the polynomial reduction from $\FulRel(H)$ to
  $\sHom(H)$.
\end{proof}

To our knowledge, $\sHom(H)$ is not fully classified. A recent survey of
the closely related complexity problem concerning the existence of vertex
surjective homomorphisms~\cite{Bodirsky2012} provides some arguments why the
characterization of complexity is likely to be hard. We observe that the
existence of a homomorphism from $G$ to $H$ is equivalent to the existence
of a surjective homomorphism from $G+H$ to $H$. Thus $\sHom(H)$ is clearly
hard for all graphs for which $\Homo(H)$ is hard, i.e., for all loop-less
graphs with odd cycles.

Testing the existence of a homomorphism from a fixed $G$ to $H$ is
polynomial (there is only a polynomial number $|V_H|^{|V_G|}$ of possible
functions from $G$ to $H$). Similarly the existence of a relation from a fixed
$G$ to $H$ is also polynomial. In fact, an effective algorithm exists.
For fixed $G$ there are finitely many point-determining graphs $T$ which $G$ has relation
to. The algorithm thus first constructs the point-determining graph of $H$ and then, using
a decision tree recognizes all isomorphic copies of all point-determining graphs $G$ has
relation to.

\section{Weak relational composition}
\label{sect:weak}

In this section we will briefly discuss the `loop-free' version, i.e.,
equations of the form $G\mulw R=H$.

Most importantly, there is no simple composition law analogous to
Lemma~\ref{lem:compo}. The expression
\begin{equation*}
(G\mulw R)\mulw S = (S^+\circ (R^+\circ G\circ R)^{\iota}\circ S)^\iota
\end{equation*}
does not reduce to relational composition in general. For example, let
$G=K_3$ with vertex set $V=\{x,y,z\}$ and consider the relations
$R=\{(x,1),(z,1),(y,2)\}\subseteq \{x,y,z\}\times\{1,2\}$ and
$S=\{(1,x')(1,z')(2,y')\}\subseteq \{1,2\}\times \{x',y',z'\}$. One can easily
verify
\begin{equation*}
(G\mulw R)\mulw S = P_2 \ne G\mulw(R\circ S)= K_3
\end{equation*}
The most important consequence of the lack of a composition law is that
R-retractions cannot be meaningfully defined for the weak
composition. Similarly, the results related to R-equivalence heavily rely
on the composition law.

Nevertheless, many of the results, in particular basis properties derived
in section~\ref{sect:basic}, remain valid for the weak composition
operation. As the proofs are in many cases analogous, we focus here mostly
on those results where strong and weak composition differ, or where we need
different proofs. In particular, Lemma~\ref{dec} also holds for the weak
composition. Thus, we still have a result similar to Corollary~\ref{DeCo},
but the proof is slightly different.

\begin{cor}
Suppose $G\mulw R=H$. Then there is a set $C$, an injective relation
$R_D\subseteq \domain R\times C$, and a surjective relation
$R_C\subseteq C\times \image R$ such that
$G[\domain R]\mulw R_D\mulw R_C=H[\image R]$.
\end{cor}
\begin{proof}
From Proposition~\ref{dec} we know $R=I'\circ R_D\circ R_C\circ I''$.
And we know $G[\domain R]\mulw R_D=G[\domain R]\muls R_D$.
From the properties of $\mulw$, we have
\begin{align*}
G[\domain R]\mulw R &=(R^+\circ G[\domain R]\circ R)^l\\
&=((R_D\circ R_C)^+\circ G[\domain R]\circ R_D\circ R_C)^l\\
&=(R_C^+\circ R_D^+\circ G[\domain R]\circ R_D\circ R_C)^l\\
&=(R_C^+\circ (R_D^+\circ G[\domain R]\circ R_D)\circ R_C)^l\\
&=(R_C^+\circ G[\domain R]\muls R_D\circ R_C)^l\\
&=(R_C^+\circ G[\domain R]\mulw R_D\circ R_C)^l\\
&=G[\domain R]\mulw R_D\mulw R_C\\
&=H[\image R].\qedhere
\end{align*}
\end{proof}

Assume $G\mulw R=H$ and let $H_1,\dots,H_k$ the connected components of
$H$. From the definition of $\mulw$ and $\muls$, if we denote
$\widetilde{H}=G\muls R$, then $\widetilde{H}$ could be decomposed into the union
of connected components $\widetilde{H}_i$($1\leq i\leq k$), such that
$(\widetilde{H}_i)^\iota=H_i$. Hence the conclusion of the proposition
\ref{ccs} also holds true for weak relations.

Lemma~\ref{colour} does not hold for weak relations. For example, there is a
weak relation of $K_5$ to $K_3$, but $\chi(K_5)=5>\chi(K_3)=3$.

Lemma~\ref{path} and Lemma~\ref{cycle} do not hold for weak relations. For
example, if $G$ is a graph consisting of a single isolated vertex isolated,
then $P_3\mulw R=G$ and $C_3\mulw R=G$, but there are no walk in $G$.

With respect to complete graphs, weak relational composition also behaves
different from strong composition. If $K_k\mulw R=H$ then $R(i)$ can
contain more that one vertex in $V_H$. Compared to Proposition
\ref{prop:complete}, we also obtain a different result:

\begin{thm}
  There is a relation $R$ such that $K_k\mulw R = H$ if and only if every
  connected component of $\overline{H}$ is a complete graph, and the number
  of connected components of $\overline{H}$ containing at least 2 vertices
  is at most $k$.
\end{thm}

\begin{proof}
  If every connected component of $\overline{H}$ is a complete graph,
  denoted the vertex sets of the connected components containing at least
  $2$ vertices by $H_1,\dots, H_m$, $m\leq k$ and the vertices of $K_k$ by
  $1,\dots,k$. Let $R={\{(i,u)\mid i=1,\dots,k,u\in V_{H_i}\}}\cup
  \{(j,v):1\leq j\leq k,v\in V_H\setminus \bigcup_{i=1}^m V_{H_i}\}$. One
  easily checks that $K_k\mulw R=H$.

  Conversely, let $R$ be a relation satisfying $K_k\mulw R=H$. Consider
  the set $U_i=\{u\in V_H\mid R^{-1}(u)=\{i\}\}$. Then $u$ and $v$ are not
  adjacent for arbitrary $u,v\in U_i$, while $u$ is adjacent to $w$ for
  every $w\in V_H\setminus U_i$. Hence
  $\overbar{H}(U_i)$ is a connected component of $\overbar{H}$, which is
  also a complete graph. Given $w\in V_H\setminus \bigcup_{i=1}^m U_i$,
  $R^{-1}(w)$ must have at least 2 vertices in $K_k$, hence $w$ is adjacent
  to every vertex in $H$ except itself; in other words, $w$ is an
  isolated vertex in $\overbar{H}$. Therefore the number of connected
  components of $\overbar{H}$ containing at least 2 vertices is no more
  than $k$.
\end{proof}

The results in subsection~\ref{revers} also remain true for weak relations.


% ------------------------------------------------------------------------


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> Introduction/introduction_0303.tex <==
%%% Thesis Introduction --------------------------------------------------
\chapter{Introduction}
\ifpdf
    \graphicspath{{Introduction/IntroductionFigs/PNG/}{Introduction/IntroductionFigs/PDF/}{Introduction/IntroductionFigs/}}
\else
    \graphicspath{{Introduction/IntroductionFigs/EPS/}{Introduction/IntroductionFigs/}}
\fi



%%% ----------------------------------------------------------------------


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 

%\markboth{\MakeUppercase{\thechapter. Introduction}}{\thechapter. Introduction}


The subject of this thesis---graph relations and constrained homomorphism orders---belongs to the field of discrete mathematics, more specifically to graph theory. It has a close relationship to several other areas of mathematics stemming from algebra and mathematical structures via category theory and logic to computer science disciplines such as computational complexity.

The term `graph' was introduced by Sylvester in 1878~\cite{Sylvester1878}.
A {\em directed graph}\index{directed graph} $G$ is a pair $G=(V_G,E_G)$ such that $E_G$ is a subset of $V_G\times V_G$. We denote by $V_G$\index{$V_G$} {\em the set of vertices of $G$}\index{set of vertices} and by $E_G$ {\em the set of edges of $G$}\index{set of edges}. The class of all finite directed graphs is denoted by $\DiGraphs$\index{$\DiGraphs$}.
An {\em undirected graph} (or simply a {\em graph}\index{graph}) $G$ is a directed graph such that $(u,v)\in E_G$ if and only if $(v,u)\in E_G$. We thus consider undirected graphs to be a special case of directed graphs. Unless explicitly stated otherwise we allow loops on vertices. The class of all finite undirected graphs is denoted by $\Graphs$\index{$\Graphs$}.

Graphs are frequently employed to model natural or artificial systems.
Let us begin the introduction with two examples taken from the real world.

In social science we can use social networks to express the relationships between individuals, groups and organizations. For example, a friendship network shows the friendship relation among individuals in a community. At the same time, travelling is an important activity in modern society as people travel frequently, for business or for pleasure. If we consider all the places that people in a certain community have ever visited, we can define a network on places in the following natural way. 
Draw an edge between place $A$ and place $B$ if and only if we can find two people who are friends, one who has visited $A$, and the other $B$.
In this way we build a new network on places generated by the friendship network and the information about people and the places they visited. 


The research presented in this thesis was originally motivated by a generalization of concepts from bioinformatics. Consider protein-protein interaction networks (PPIs) in biology. Proteins contain domains that determine their function. Information on the domain content of proteins, which can be seen as a relation
$R\subseteq D\times P$ between domains and the proteins which contain them is readily available from biological databases. Candidates for interaction between domains can be derived from knowledge about the interacting proteins, i.e., a graph $G$ with vertex set $P$, and the relation $R$: If $(p,p')\in E_G$,
 $(d,p)\in R$, and $(d',p')\in R$, then the domains 
$(d,d')$ are putative interaction partners. 

In both examples, we use a network and a relation to create a new network. %The original network and that which is built upon it by using a relation are thus connected to one another. 
Conversely, given two networks, can we determine some meaningful relation between them? This is the idea behind the graph relations. 

More abstractly, let $G=(V_G,E_G)$ be a graph, $B$ a finite set, and
$R\subseteq V_G\times B$ a binary relation such that for every $b\in B$ there is $v \in V_G$ such that $(v,b)\in R$. Then
the graph $G\muls R$ has vertex set $B$ and edge set
\begin{equation*}
E_{G\muls R} = \left\{ (a,b)\in B\times B \mid \textrm{ there is }
      (u,v)\in E_G \textrm{ such that } (u,a),(v,b)\in R \right\}.
\end{equation*}
If there exists an $R$ satisfying the equation $G\muls R = H$, we say
there is a \emph{relation}\index{relation} from $G$ to $H$. The graphs $G$ and $H$
can be seen to be conjugates, i.e., $E_G=R^+\circ E_H\circ R$, where $R^+\subseteq B\times V_G$ is the transpose of the relation $R$ and $\circ$\index{$\circ$} denotes the \emph{composition}\index{composition} of binary relations, which is defined as follows: If $S\subseteq X\times Y$ and $T\subseteq Y\times Z$ are two binary relations, then $S\circ T=\{(x,z)\in X\times Z\mid  \textrm{ there is } y\in Y \textrm{ such that } (x,y)\in S \textrm{ and } (y,z)\in T\}$.


The concept of a relation between graphs turns out be closely related to the well-studied graph theory 
notion of a graph homomorphism. For given graphs $G=(V_G,E_G)$ and
$H=(V_H,E_H)$, a \emph{homomorphism}\index{homomorphism} $f:G\to H$ is a mapping $f:V_G\to
V_H$ such that $(u,v)\in E_G$ implies $(f(u),f(v))\in E_H$. If there is no homomorphism from $G$ to $H$, we write $G\nrightarrow H$\index{$G\nrightarrow H$}. 
Graph homomorphisms have been studied ever since the 1960s, originally as a generalization of graph colourings, with pioneering work by G.\ Sabidussi~\cite{Sabidussi1961}, Z.\ Hedrl\' in and A.\ Pultr~\cite{Hedrlin1964} subsequently seeing rapid development by P.\ Hell and J.\ Ne\v{s}et\v{r}il~\cite{Hell2004}. There is a lot of intensive research going on around this topic; for an extensive review of the subject, see~\cite{Hell2004}.

A homomorphism from a graph $G$ to a graph $H$ naturally defines a mapping $f^{1}:E_G\to E_H$ by setting
$f^{1}((u,v))=(f(u),f(v))$ for all $(u,v)\in E_G$. If both $f$ and $f^1$
are surjective, we call $f$ a \emph{surjective homomorphism}\index{surjective homomorphism}. Note that all
surjective homomorphisms $f:G\to H$ are (modulo representation) also
relations $G\muls R=H$, where $R=\{(u,f(u)) \mid u\in V_G\}$.

Obviously, relations that are not functional are not homomorphisms, but
correspond to multihomomorphisms, which in a sense are multifunctions. A \emph{multifunction}\index{multifunction} from a non-empty set $X$ to a non-empty set $Y$ is a function from $X$ to $P(Y)\setminus \emptyset$ where $P(Y)$ is the power set of $Y$~\cite{Nenthein2012}. Multifunctions between two topological spaces have been studied since 1960s~\cite{Whyburn1965}. Multifunctions were first studied in an algebraic sense in~\cite{Triphop2008}, in which they feature as multihomomorphisms from one group to another group. To the best of our knowledge, multihomomorphisms between graphs first appeared as building blocks of Hom-complexes, introduced by Lov{\'a}sz, and are related to recent exciting developments in topological combinatorics~\cite{Matousek2003}, in particular to deep results involved in a proof of the Lov{\'a}sz hypothesis~\cite{Babson2006}.

A relation with full domain thus can be regarded as a \textit{surjective multihomomorphism}, a multihomomorphism such that the pre-image of every vertex in $H$ is non-empty and for every edge $(x,y)$ in $H$ we can find an edge $(u,v)$ in $G$ satisfying $x\in f(u)$, $y\in f(v)$.

It appears that surjective multihomomorphisms between groups were first defined in~\cite{Triphop2008} and studied in~\cite{Nenthein2012}. However, surjective multihomomorphisms between graphs have not yet received attention.


\TODO{In this work, we show that even the notion of relations was not noticed by graph theorist, it has its own charm. Owing to omitted the constrains to be a mapping, it largely generalizes the situation which can happen in graph homomorphisms; it can ignore some part of original graphs, and/or maps one vertices to multiple vertices. Even the relations with full domains are a generalization of surjective homomorphisms. Every relation can be decomposed in a standard way into a surjective homomorphism and an injective relation, whose transpose can be seen as a full homomorphism. It derives many interesting notions of graph classes, such as R-cores, cores, reduced graphs and cocores. We show that core and reduced graph coincide, develop the characterization of cocore and R-core, and provide effective algorithms to compute them. We also give the implication relation of these notions and gives examples which can distinguish them. We also give a perhaps surprisingly simple characterization of those graphs $G$ for which all relations of $G$ to itself are automorphisms. For the computational complexity of testing for the existence of a relation, we describe the reduction of this problem to the corresponding problem for surjective homomorphisms.}



% 
% The study of relations, just as for the study of homomorphisms, involves investigating properties of general structures restricted to graphs.
% Surprisingly, we find that whereas the notion of a graph homomorphism originated in the other areas of mathematics, the notion of a constrained homomorphism arose instead from applied disciplines such as social science and electronics.

\mbox{}

\TODO{Inspired by relation,} we widen the scope of our study to investigate the properties of \emph{constrained homomorphisms}\index{constrained homomorphisms}, i.e., homomorphisms that satisfy further conditions such as surjectivity.
Partial orders induced by the existence of constrained homomorphisms and their properties form the second topic of this thesis. In particular we consider the following:

\begin{enumerate}
\item A homomorphism $f:G\to H$ is a {\em monomorphism}\index{monomorphism}\footnote{The name `monomorphism' originates from category theory.}, (also called \emph{injective homomorphism}\index{injective homomorphism}~\cite{Hell2004} or {\em \MonoHomo}) if it is injective.
\item A homomorphism $f:G\to H$ is a {\em full homomorphism}\index{full homomorphism}, or {\em \FullHomo}\index{\FullHomo}, if $(f(u),f(v))\in E_H$ implies $(u,v)\in E_G$.
\item A homomorphism $f:G\to H$ is an {\em embedding}\index{embedding}, or {\em \EmbedHomo}\index{\EmbedHomo} if it is both a monomorphism and a full homomorphism.
\end{enumerate}


For undirected graphs we also consider the following forms of locally constrained homomorphisms.
\begin{enumerate}
\item A homomorphism $f:G\to H$ is a {\em locally injective homomorphism}\index{locally injective homomorphism}, or {\em \LocInHomo}\index{\LocInHomo}, if for all $v\in V_G$, the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is injective.
\item A homomorphism $f:G\to H$ is a {\em locally surjective homomorphism}\index{locally surjective homomorphism}, or {\em \LocSurHomo}\index{\LocSurHomo}, if for all $v\in V_G$, the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is surjective.
\item A homomorphism $f:G\to H$ is a {\em locally bijective homomorphism}\index{locally bijective homomorphism}, or {\em \LocBiHomo}\index{\LocBiHomo}, if it is both a locally surjective and locally bijective homomorphism, that is, if the restrictions to the neighbourhoods are bijections.
\end{enumerate}


There are also other types of constrained homomorphism that have been studied. One example is that of a compaction~\cite{Kedem1984}.
A \emph{compaction}\index{compaction} of a graph $G$ to a graph $H$ is a homomorphism $f:G\to H$ such that for every vertex $x$ of $H$, there exists a vertex $v$ of $G$ with $f(v)=x$, and for every edge $(x,y)$ of $H$, $x\neq y$, there exists an edge $(u,v)$ of $G$ with $f(u)=x$ and $f(v)=y$. The computational complexity of compaction has been studied by Vikas~\cite{Vikas2002,Vikas2004}.

Constrained homomorphisms have been intensively studied in their structural and algorithmic aspects as well as in their applications. 
Each type of constrained homomorphism has its own history. For example, globally constrained homomorphisms have also been studied from the 1960s. The earliest literature we can find is what Hedetniemi published in 1966~\cite{Hedetniemi1966}. It is however surprising to learn from the survey paper~\cite{Fiala2008} that the notion of a locally bijective homomorphism was already well established in combinatorial topology as early as 1932~\cite{Reidemeister1932}.
The other types of locally constrained homomorphism received attention much later. Locally surjective homomorphisms were introduced by Everett and Borgatti in 1991~\cite{Everett1991} and locally injective homomorphisms by Ne\v set\v ril in 1971~\cite{Nesetril1971}.


There are many results that link graphs and orders, such as those concerning vertex-edge-face partial orders~\cite{Brightwell1997}, planar graphs, hypergraph colourings~\cite{Duffus1991}, and on-line algorithms~\cite{Kierstead1981}.
In a similar vein, the dimension of a partial order is analogous to the chromatic number of a graph~\cite{Kelly1982}.
See the survey paper~\cite{Trotter1996} by Trotter. We give another instance of partial orders on graphs.

For any fixed type of finite relational structure, homomorphisms induce an ordering of the set of all structures. In particular, given two (directed) graphs $G$ and $H$, we write $G\leq H$, or $G\to H$, if there is a homomorphism from $G$ to $H$. The relation $\leq$ is a quasi-order and so it induces an equivalence relation. 
For two (directed) graphs $G$ and $H$ such that $G\Hom H$ and $H\Hom G$, we write $G\Homeq H$ and say that {\em $G$ and $H$ are homomorphically equivalent}\index{homomorphically equivalent}. The homomorphism orders $(\Graphs,\leq)$ and $(\DiGraphs,\leq)$ are the partially ordered sets of all equivalence classes of finite undirected and directed graphs, respectively, ordered by the relation $\leq$. We shall abuse notation and follow the convenient practice of identifying an equivalence class in either of these homomorphism quasi-orders with one of its representatives, namely that (di)graph which is the core of all other (di)graphs equivalent to it. So by $(\Graphs,\leq)$, respectively $(\DiGraphs,\leq)$, we will actually be referring to the partially ordered sets induced by the quasi-ordered sets of all graphs (digraphs) on the set of graph (digraph) cores. (The notion of a graph core requires some preparation and will be defined in its proper place in Chapter~\ref{ch:homo}.)
%We will often abuse notation by replacing the classes that comprise $(\Graphs,\leq)$ and $(\DiGraphs,\leq)$ by their members (cores).

These orders are of particular interest. For example, each of the two orders forms a distributive lattice, with the disjoint union of graphs being the supremum and the categorical product being the infimum.

The homomorphism order has been a fruitful research topic for several decades.
One of the well studied properties of the homomorphism order is density. Both $(\Graphs,\leq)$ and $(\DiGraphs,\leq)$ are dense, the former shown by Welzl~\cite{Welzl1982} and the latter by Ne\v set\v ril and Tardif~\cite{Nesetril2000}.

The other property which is extensively studied is universality. Any countable partial order is isomorphic to a suborder of $(\DiGraphs,\leq)$. This result first appeared in the context of categories in 1969~\cite{Pultr1980}. \emph{Antichains}\index{antichain} are sets of elements which are pairwise incomparable. A characterization of finite maximal antichains was given in~\cite{Nesetril1978}.

Maximal antichains are particularly relevant because of their relationship to the notion of a \emph{homomorphism duality}\index{homomorphism duality}, introduced by Ne\v set\v ril and Pultr~\cite{Nesetril1978}. An ordered pair $(F,D)$ of graphs, or directed graphs, is a \emph{duality pair}\index{duality pair} if $\{G\mid F\to G\}=\{G\mid G\nrightarrow D\}$. Moreover, Ne\v set\v ril and Tardif obtain a correspondence between duality pairs and gaps in the homomorphism order~\cite{Nesetril2000a}.

\TODO{
In the second part of this work, we consider the analogous properties on the constrained homomorphism orders. We provide a systematical method to characterize the gaps and dualities in the constrained homomorphism orders, by analysis the properties of future-finite or past-finite order. Which simplified many of the existing results. We also give a method to build universal orders from future-finite or past-finite universal orders. Among other by realizing that oriented cycles are a new universal class in homomorphism order, we prove universality of the homomorphism order on the class of line graphs and of locally constrained homomorphism orders. 
}
 
\vspace{10pt}

This thesis consists of five chapters, including this introduction.

In Chapter~\ref{ch:graph} we describe notions that we require from graph theory and order theory.
In particular, we introduce basic graph-theoretic concepts and state their properties,
and define the main operations on graphs. We also give the fundamental properties of partial orders.
Chapter~\ref{ch:homo} gives a brief overview of graph homomorphisms and constrained homomorphisms. Moreover, we introduce the new notion of graph relation, and we compare it to the other well-studied types of constrained graph homomorphism. We provide the necessary background on the theory of computational complexity in Appendix A.


Further properties of relations are introduced in Chapter~\ref{ch:relation}.
We first show that every relation can be decomposed in a standard way into a surjective and an injective relation (Corollary~\ref{DeCo}). 
The equivalence classes of strong relational equivalence (Theorem~\ref{thm:equi}) and weak relational equivalence (Proposition~\ref{pro:iso}) are characterized. We then introduce the notion of R-cores, cores, reduced graphs and cocores. We show that core and reduced graph coincide, develop the characterization of cocore and R-core, and provide an effective algorithm to compute them. We also give a perhaps surprisingly simple characterization of those graphs $G$ for which all relations of $G$ to itself are automorphisms (Theorem~\ref{thm:auto1}). The computational complexity of testing for the existence of a relation between two graphs is briefly discussed. We describe the reduction of this problem to the corresponding problem for surjective homomorphisms. Finally, we briefly summarize the most important similarities and differences between weak and strong relational composition (Section~\ref{sect:weak}). Some of the results from this chapter have been published by J.~Hubi\v cka, J.~Jost, Y.~Long, P.~F.~Stadler, and L.~Yang in~\cite{Hubicka2012}. 


In Chapter~\ref{Ch:order} we review existing results on the homomorphism order (in Section~\ref{sec:homoorder}) and introduce the notion of constrained homomorphism orders. Moreover, after some discussion of universality, 
a new and significantly easier proof of universality of graph homomorphisms is given (Theorem~\ref{lem:cycles}), which simplifies the proof given in~\cite{Hubicka2005}.
As a new result, we show that graph homomorphisms are universal even on the class of oriented cycles. The notions of future-finite-universal and past-finite-universal partial order are introduced (in Section~\ref{sec:universality}) for later use. We survey existing results on constrained homomorphism orders and provide several new results about cores, universality, gaps and dualities in the context of constrained homomorphisms. We derive properties of these partial orders and identify their similarities and differences. At the same time we give a simple condition for the existence of dualities in future-finite and past-finite partial orders (in Section~\ref{sec:pastfinite}). 
In the full homomorphism order (Section~\ref{sec:fullhomo}) we characterize the gaps and give a new and simple proof of the existence of left duals (Theorem~\ref{thm:fulldual}) (simplifying results independently obtained by Feder and Hell~\cite{Feder2008} and Ball, Ne\v set\v ril, Pultr~\cite{Ball2007,Ball2010}).
For locally injective homomorphisms we prove universality on connected graphs (Theorem~\ref{thm:lochomouniv})
and give a partial characterization of gaps (Theorem~\ref{thm:locingap}). We also prove the universality of all three kinds of locally constrained homomorphisms on graphs. We apply the characterization of PR-cores and FR-cores which are derived in Chapter~\ref{ch:relation} and carry over most results on the surjective homomorphism order. 
We prove that for every $d\geq 3$ the homomorphism order on the class of line graphs with maximum degree $d$ is universal (Theorem~\ref{thm:main}).
Some of the results from this chapter have been submitted~\cite{Fiala2014} or are in preparation~\cite{Fiala2012}.





==> Introduction/introduction_beforeAndrew.tex <==
%%% Thesis Introduction --------------------------------------------------
\chapter{Introduction}
\ifpdf
    \graphicspath{{Introduction/IntroductionFigs/PNG/}{Introduction/IntroductionFigs/PDF/}{Introduction/IntroductionFigs/}}
\else
    \graphicspath{{Introduction/IntroductionFigs/EPS/}{Introduction/IntroductionFigs/}}
\fi



%%% ----------------------------------------------------------------------


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 

%\markboth{\MakeUppercase{\thechapter. Introduction}}{\thechapter. Introduction}


The subject of this thesis---graph relations and constrained homomorphism orders---belongs to the field of discrete mathematics, in particular graph theory. It has close relationship to several other fields of mathematics stemming from algebra and mathematical structures via category theory and logic to computer science disciplines like the field of computational complexity.

The term `graph' was introduced by Sylvester in 1878~\cite{Sylvester1878}.
A {\em directed graph}\index{directed graph} $G$ is a pair $G=(V_G,E_G)$ such that $E_G$ is a subset of $V_G\times V_G$. We denote by $V_G$ {\em the set of vertices of $G$}\index{set of vertices} and by $E_G$ {\em the set of edges of $G$}\index{set of edges}. The class of all finite directed graphs is denoted by $\DiGraphs$.
An {\em undirected graph} (or simply a {\em graph}\index{graph}) $G$ is a directed graph such that $(u,v)\in E_G$ if and only if $(v,u)\in E_G$. We thus consider undirected graphs to be a special case of directed graphs. Unless explicitly stated otherwise we allow loops on vertices. The class of all finite undirected graphs is denoted by $\Graphs$.

Graphs are frequently employed to model natural or artificial systems.  
Let us start the introduction with two examples in the real world.

In social science we can use social network to express the relationships between individuals, groups, organizations. For example, friendship network shows the friendship relation in a society. At the same time, traveling is a important activity in modern society, people travel frequently, for business or for pleasure. If we consider all the places that people in a certain society have ever visited, we can define a network on places naturally in the following way. 
Draw an edge between place $A$ and place $B$ if and only if we can find two people who are friends, one has visited $A$, and the other $B$.
In this way we build a new network on places generated by the friendship network and the information on people und the places they visited. 


Research presented in this thesis was originally motivated by a generalization of concepts from bioinformatics. Consider protein-protein interaction networks (PPIs) in biology. Proteins contain domains that determine their function. Information on the domain content of proteins, which can be seen as a relation
$R\subseteq D\times P$ between domains and the proteins which contain them is readily available from biological databases. Candidates for interaction between domains can be derived from knowledge on the interacting proteins, i.e., a graph $G$ with vertex set $P$, and the relation $R$: If $(p,p')\in P$, $(d,p)\in R$, and $(d',p')\in R$, then the domains 
$(d,d')$ are putative interaction partner. 

In both examples, we use a network and a relation to create a new network. Obviously, these two networks are connected by the relation reflection. Conversely, given two networks, can we determine some meaningful relation between them? This is the idea behind the graph relations. 

More abstractly, let $G=(V_G,E_G)$ be a graph, $B$ a finite set, and
$R\subseteq V\times B$ a binary relation, so that, for every element
$b\in B$, we can find an element $v \in V_G$ such that $(v,b)\in R$. Then
the graph $G\muls R$ has vertex set $B$ and edge set
\begin{equation*}
E_{G\muls R} = \left\{ (u,v)\in B\times B \mid \textrm{ there is }
      (x,y)\in E_G \textrm{ and } (x,u),(y,v)\in R \right\}.
\end{equation*}
If there exists an $R$ satisfying the equation $G\muls R = H$, we say
there is a \emph{relation} from $G$ to $H$. Note that graphs $G$ and $H$
can be seen to be conjugate, i.e., $G=R^+\circ H\circ R$.


This concept turns out to have a close relation to a well studied graph theory
concept: graph homomorphism.  For given graphs $G=(V_G,E_G)$ and
$H=(V_H,E_H)$ a \emph{homomorphism}\index{homomorphism} $f:G\to H$ is a mapping $f:V_G\to
V_H$ such that $(u,v)\in E_G$ implies $(f(u),f(v))\in E_H$. If there is no homomorphims from $G$ to $H$, we write $G\nrightarrow H$\index{$G\nrightarrow H$}.
As a generalization of graph colourings, graph homomorphisms is studied from 1960s. It was pioneered by G.\ Sabidussi~\cite{Sabidussi1961},  Z.\ Hedrl\' in and A.\ Pultr~\cite{Hedrlin1964}, and rapidly developed by P.\ Hell and J.\ Ne\v{s}et\v{r}il~\cite{Hell2004}. There is a lot of intensive research going on in this topic, for an extensive review of the subject, see~\cite{Hell2004}.

A homomorphism of graph $G$ to graph $H$ naturally defines a mapping $f^{1}:E_G\to E_H$ by setting
$f^{1}((x,y))=(f(x),f(y))$ for all $(x,y)\in E_G$. If both $f$ and $f^1$
are surjective, we call $f$ a \emph{surjective homomorphism}\index{surjective homomorphism}. Note that all
surjective homomorphisms $f:G\to H$ are (modulo representation) also
relations $G\muls R=H$ where $R=\{(u,f(u)),x\in V_G\}$.

Obviously, relations that are not functional are not homomorphisms, but
correspond to multihomorphisms, which in a sense is multifunction. A \emph{multifunction} from a non-empty set $X$ into a non-empty set $Y$ is a function from $X$ into $P(Y)\setminus \emptyset$ where $P(Y)$ is the power set of $Y$~\cite{Nenthein2012}. Multifunctions between two topological spaces have been studied since 1960s~\cite{Whyburn1965}. In~\cite{Triphop2008} multifunctions were first studied in an algebraic sense, which is called multihomomorphisms from a group into another group. To our best knowledge, multihomomorphisms between graphs first appeared as building blocks of Hom-complexes, introduced by Lov{\'a}sz, and are related to recent exciting
developments in topological combinatorics~\cite{Matousek2003}, in particular to deep results involved in a proof of the Lov{\'a}sz hypothesis~\cite{Babson2006}.

A relation with full domain thus can be regarded as a \textit{surjective multihomomorphism}, a multihomomorphism such that pre-image of every vertex in $H$ is non-empty and for every edge $(u,v)$ in $H$ we can find an edge $(x,y)$ in $G$ satisfying $u\in f(x)$, $v\in f(y)$.

It appears that surjective multihomomorphisms between groups were first defined in~\cite{Triphop2008} and studied in~\cite{Nenthein2012}. However, surjective multihomomorphisms between graphs have never been studied yet.


The study of relations, the same as the study of homomorphisms, is to investigate properties of general structures restricted to graphs.
Surprisingly, we find that the graph homomorphism is originated in the other fields of mathematics, however, constrained homomorphisms arose from applied disciplines such as social science and electronics, etc.

\mbox{}

We further widen the scope to study the properties of homomorphism-like mappings in general. we use \emph{constrained homomorphism} as a generic term for these special homomorphisms. The properties of partial orders induced by the existence of constrained homomorphisms are the second topic of this thesis. In particular we consider the following:


\begin{enumerate}
\item A homomorphism $f:G\to H$ is {\em a monomorphism}\index{monomorphism}\footnote{The name `monomorphism' is from category theory.}, (also called \emph{injective homomorphism}\index{injective homomorphism}~\cite{Hell2004} or {\em \MonoHomo}) if it is injective.
\item A homomorphism $f:G\to H$ is {\em a full homomorphism}, or {\em \FullHomo}, if $(f(u),f(v))\in E_H$ implies $(u,v)\in E_G$.
\item A homomorphism $f:G\to H$ is {\em an embedding}, or {\em \EmbedHomo} if it is both a monomorphism and a full homomorphism.
\end{enumerate}


For undirected graphs we also consider the following forms of locally constrained homomorphisms.
\begin{enumerate}
\item A homomorphism $f:G\to H$ is {\em locally injective homomorphism}, or {\em \LocInHomo}, if the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is injective.
\item A homomorphism $f:G\to H$ is {\em locally surjective homomorphism}, or {\em \LocSurHomo}, if the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is surjective.
\item A homomorphism $f:G\to H$ is {\em locally bijective homomorphism}, or {\em \LocBiHomo}, if it is both a locally surjective and locally bijective homomorphism, that is, if the restriction on neighbourhoods is a bijection.
\end{enumerate}


Note that there are also other constrained homomorphisms which were studies. One of the examples is compaction~\cite{Kedem1984}.
A \emph{compaction} of graph $G$ to graph $H$ is a homomorphism of $G$ to $H$ such that for every vertex $x$ of $H$, there exists a vertex $v$ of $G$ with $c(v)=x$, and for every edge $(h,h')$ of $H$, $h\neq h'$, there exists an edge $(g,g')$ of $G$ with $c(g)=h$ and $c(g')=h'$. The computational complexity of compaction was studied by Vikas~\cite{Vikas2002,Vikas2004}.

Structural and algorithmic aspects as well as applications of constrained homomorphisms have been intensively studied.
Each constrained homomorphism has its own history. For example the global constrained homomorphism were also studied from 1960s. The earliest literature we can find is what Hedetniemi published in 1966~\cite{Hedetniemi1966}. It is however surprising that, based on a survey paper~\cite{Fiala2008}, locally bijective homomorphism was already well established in combinatorial topology in 1932~\cite{Reidemeister1932}.
The other locally constrained homomorphisms have been started much later. Locally surjective homomorphisms were introduced by Everett and Borgatti in 1991~\cite{Everett1991} and locally injective homomorphisms by Ne\v set\v ril in 1971~\cite{Nesetril1971}.


Many results link graphs and orders, like the study of vertex-edge-face partial orders~\cite{Brightwell1997}, and
planar graphs, hypergraph colourings~\cite{Duffus1991}, on-line algorithms~\cite{Kierstead1981}.
Also note that dimension of partial order is analogous to the chromatic number of graph~\cite{Kelly1982}.
See a survey paper by Trotter~\cite{Trotter1996}. We give another instance of partial orders on graphs.

For any fixed type of finite relational structure, homomorphisms induce an ordering of the set of all structures. In particular, give two (directed) graphs $G$ and $H$, we write $G\leq H$ or $G\to H$ provided that there is a homomorphism from $G$ to $H$. Then the relation $\leq$ is a quasi-order and so it induces an equivalence relation:
For two (directed) graphs $G$ and $H$ such that $G\Hom H$ and $H\Hom G$, we write $G\Homeq H$ and say that {\em $G$ and $H$ are homomorphically equivalent}. The homomorphism order $\Graphs$ and $\DiGraphs$ are the partially ordered sets of all equivalence classes of finite undirected and directed graphs, respectively, ordered by the $\leq$. We will often abuse notation by replacing the classes that comprise $\Graphs$ and $\DiGraphs$ with their members.

These orders are of particular interests. For example, the two orders are actually a distributive lattice, with the disjoint union of graphs being the supremum and the categorical product being the infimum.

The homomorphism order has been fruitful research topic for several decades.
One of the well studied properties of homomorphism order is density. Both $\Graphs$ and $\DiGraphs$ are dense, the former shown by Welzl~\cite{Welzl1982} and the latter, by Ne\v set\v ril and Tardif~\cite{Nesetril2000}.

The other property which is extensively studied is universality. That is, any countable partial order is isomorphic to a suborder of $\DiGraphs$. This result first appeared in the context of categories in 1969~\cite{Pultr1980}. Antichains are sets of element which is not comparable. The characterization of finite maximal antichains was given in~\cite{Nesetril1978}.

Maximal antichains are particularly relevant because of their relationship to the notion of a \emph{homomorphism duality}, introduced by Ne\v set\v ril and Pultr~\cite{Nesetril1978}: an ordered pair $(F,D)$ of graphs, or directed graphs, is a \emph{duality pair} if $\{G\mid F\to G\}=\{G\mid G\nrightarrow D\}$. Moreover, Ne\v set\v ril and Tardif obtain a correspondence between duality pairs and gaps in the homomorphism order~\cite{Nesetril2000a}.
%  
% \vspace{10pt}
% 
% One of the aims of this thesis is to introduce a new notion `graph relation' which is a variant of graph homomorphism. The concept of `relation' is very natural and at the same time relatively general.
% Moreover, some of the properties of relations coincide with the properties of a well defined notion `graph homomorphism' and its variants. On the other hand, it also owns specific properties. These properties are of interest not only in the theory of structural and algorithmic graph theory, but also in application. Furthermore, it gives birth to many interesting theoretical notions and results.
% 
% The second purpose of the thesis is to provide a systematic survey on constrained homomorphisms orders, which are partial orders with graphs as elements and ordered by the existence of the corresponding constrained homomorphisms, such as monomorphisms, surjective homomorphisms, full homomorphisms, relations and locally constrained homomorphisms. 
% While the homomorphism order has been fruitful research topic for several decades, relatively little effort has been put into the study of orders induced by the constrained homomorphisms. Our goal is to show the properties of these partial orders, and to identify their similarities and differences. We survey existing results and provide several new results about cores, universality, gaps and dualities in the context of constrained homomorphisms. 
% 
% 
% Another goal is to provide a systematic summary on the results of graph homomorphisms and various of constrained homomorphisms. These constrained homomorphisms are motivated respectively from different fields in the past 60 years. Each of them has its own properties and applications. We compare them and give better understandings. 
% 
% To give an idea how other disciplines such as biology motivates combinatorics is also considered as an effect of this thesis.

\vspace{10pt}

This thesis consists of five Chapters.

In Chapter 2 we provide the main concepts of graph theory and order theory.
In particular, we introduce basic graph theoretic concepts and state their properties,
and define the main operations on graphs. We also give the fundamental properties of partial orders.  
Chapter 3 gives a brief overview of graph homomorphism and constrained homomorphisms, i.e., monomorphism, surjective homomorphism, full homomorphism and 
locally bijective, injective, surjective homomorphism. Moreover, we introduce a new notion of graph relation, which is a new variant of homomorphism and can be seen as a generalized surjective homomorphism. We compare it to the other well studied constrained graph homomorphisms. We provide the necessary background on the theory of computational complexity in Appendix A.


%In Chapter 5 we introduce the fundamental concepts in partial order theory, and moreover we discuss a concrete the partial order, homomorphism order, that is, graphs ordered by the existence of homomorphisms. We discuss the density, duality and gaps, the maximum antichain for the category of simple graphs and directed graphs respectively. We also introduce the universality of homomorphism order. The methods of investigate the universality of order are introduced systematically.


More properties of relations are introduced in Chapter 4.
We first show that every relation can be decomposed in a standard way into a surjective and an injective relation (Corollary~\ref{DeCo}). 
Equivalent classes of strong relational equivalence (Theorem~\ref{thm:equi}) and weak relational equivalence (Proposition~\ref{pro:iso}) are characterized. We then introduce the notion of R-cores, cores, reduced graphs and cocores. We figure out that core and reduced graph coincide, develop the characterization of cocore and R-core, and provide an effective algorithm respectively to compute them. We also give a, perhaps surprisingly simple, characterization of those graphs $G$ for which all relations of $G$ to itself are automorphisms (Theorem~\ref{thm:auto1}). The computational complexity of testing for the existence of a relation between two graphs is briefly discussed. We describe the reduction of this problem to the problem of surjective homomorphism. Finally, we briefly summarize the most important similarities and differences between weak and strong relational composition (Section~\ref{sect:weak}). Some of the results from this chapter has been published by J.~Hubi\v cka, J.~Jost, Y.~Long, P.~F.~Stadler, and L.~Yang in~\cite{Hubicka2012}. 


In Chapter 5 we review existing results of homomorphism order and introduce the notion of constrained homomorphism orders. Moreover, more discussion about the universality
and a new and significantly easier proof of universality of graph homomorphisms are given, which simplifies the proof given in~\cite{Hubicka2005}.
As a new result, we show that the graph homomorphisms are universal even on the class of oriented cycles. The notions of future-finite-universal and past-finite-universal partial order are introduced for later use. We survey existing results on constrained homomorphism orders and provide several new results about cores, universality, gaps and dualities in the context of constrained homomorphisms. We show the properties of these partial orders and identify their similarities and differences. At the same time we give a simple condition for the existence of dualities in future-finite and past-finite partial orders. 
In full homomorphism order we characterize the gaps and give a new and simple proof of existence of left duals (simplifying results independently obtained by Feder and Hell \cite{Feder2008} and Ball, Ne\v set\v ril, Plutr \cite{Ball2007,Ball2010}).
For locally injective homomorphisms we prove the universality on connected graphs
and give a partial characterization of gaps. We also prove the universality of all three kinds of locally constrained homomorphisms on graphs. We apply the characterization of PR-cores and FR-cores which are discovered in Chapter 4 and carry over most results on the surjective homomorphism order. 
We prove that for every $d\geq 3$ the homomorphism order on class of line graphs with maximal degree $d$ is universal.
Some of the results from this chapter has been submitted~\cite{Fiala2014} or in preparation~\cite{Fiala2012}.





==> Introduction/introduction_old.tex <==
%%% Thesis Introduction --------------------------------------------------
\chapter{Introduction}
\ifpdf
    \graphicspath{{Introduction/IntroductionFigs/PNG/}{Introduction/IntroductionFigs/PDF/}{Introduction/IntroductionFigs/}}
\else
    \graphicspath{{Introduction/IntroductionFigs/EPS/}{Introduction/IntroductionFigs/}}
\fi



%%% ----------------------------------------------------------------------


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 

\section{introduction}




The \emph{complement} $\overline{G}$ of simple graph $G$ is the graph on $V$
with edge set $[V]^2/E$.

The \emph{underlying graph} $G_{sim}$ of multigraph $G$ is the
simple graph having the same vertex set $V_G$, and there is a edge
between two vertices in $G_{sim}$ if and only if there is at least
an edge between them in $G$.

A \emph{graph homomorphism} $f$ from a graph $G = (V_G,E_G)$ to a
graph $H = (V_H,E_H)$, written $f:G \rightarrow H$, is a mapping
$f:V_G \rightarrow V_H$ from the vertex set of $G$ to the vertex set
of $H$ such that $\{x,y\}\in E_G$ implies $\{f(x),f(y)\}\in E_H$.

An \emph{isomorphism} of graphs $G$ and $H$ is a bijection between
the vertex sets of $G$ and $H$ $ f \colon V_G \to V_H \,\!$ such
that any two vertices $u$ and $v$ of $G$ are adjacent in $G$ if and
only if $f(u)$ and $f(v)$ are adjacent in $H$.





A graph $G$, if it holds the property that the neighborhood of any two vertices are not equal, i.e. $N(x)\neq N(y)$ for $\forall x,y\in G$
 we call the graph is \emph{thin graph}.







Closure
For all $a, b$ in $S$, the result of the operation $a\circ b$ is also in $S$.
Associativity
For all $a, b$ and $c$ in $S$, the equation $(a\circ b) \circ c$ = $a \circ (b \circ c)$ holds.
Identity element
There exists an element $e$ in $S$, such that for all elements $a$ in $S$, the equation $e\circ a = a \circ e = a$ holds.



A \emph{reflexive graph} is a pseudograph such that each vertex has an associated graph loop.


\section{Preliminary}
In this section I will give a list of basic concepts of graph theory which is used in the dissertation.

\subsection{Basic concepts in graph theory}

A \emph{graph} is an ordered pair of disjoint sets $(V,E)$

A \emph{directed graph} \index{directed graph} $G$ is a pair $G=(V_G,E_G)$ such that $E_G$ is a
subset of $V_G\times V_G$. We denote by $V_G$ \index{$V_G$} the \emph{set of vertices
of $G$} \index{vertices, vertex} and by $E_G$ \index{$E_G$}\emph{the set of edges of $G$} \index{edge}.
We consider only finite graphs and allow loops on vertices.

An \emph{undirected graph} \index{undirected graph}(or simply a \emph{graph} \index{graph}) $G$ is any
directed graph such that $(u,v)\in E_G$ if and only if $(v,u)\in E_G$. We
thus consider undirected graphs to be special case of directed graphs and
we still allow loops on vertices.  A \emph{simple graph} is an undirected
graph without loops.


A \emph{multigraph} $G$ is an ordered pair $G:=(V, E)$ with $V$ a
set of vertices. $E$, a multiset of unordered pairs of vertices,
called \emph{edges}. Denote vertex set by $V_G$ and edge set by $E_G$. We
allow multigraphs to have \emph{loops}, that are, the edges that
connect a vertex to itself.

As opposed to a multigraph, a \emph{simple graph} is a undirected
graph with no loops and no more than one edge between different
vertices.

A \emph{pseudograph} is a non-simple graph in which both graph loops and multiple edges are permitted.

If $(x,y)\in E(G)$, then $x$ and $y$ are \emph{adjacent} \index{adjacent}.

We say that $G'=(V',E')$ is a \emph{subgraph} \index{subgraph} of $G=(V,E)$ if $V'\subset V$ and $E'\subset E$.
In this case we write $G'\subset G$ \index{$\subset$}.
If $G'$ contains all edges of $G$ that join two vertices in $V'$ then $G'$ is said to be the
subgraph \emph{induced} by $V'$ and is denoted by $G[V']$ \index{$G[V']$}.

In other words, $G'$ is an
\emph{induced subgraph} \index{induced subgraph} of $G$ if it has all the edges that appear
in $G$ over the same vertex set.


The set of vertices adjacent to a vertex $x\in G$, the \emph{(open) neighborhood} of $x$ in $G$, is denoted by $N_G(x)$.
we denote $N_G[x]=N_G(x)\cup \{x\}$ \index{$N_G[x]$}, call it \emph{closed neighborhood} of $x$ in $G$.


path and cycle
directed path and cycle, denote the vertices.
A \emph{walk} \index{walk} in a graph $G$ is a sequence of vertices $v_0,v_1,\ldots,v_k$ of $G$ such that $v_{i-1}$ and $v_i$ are adjacent for each
$i=1,2,\dots,k$.

oriented path

The graph with vertices 0,1,$\dots$,$k$ and edges (0,1),(1,2),$\dots$,$((k-1,k))$ is called the path $P_k$. Note that $P_k$ has $k+1$
vertices and $k$ edges.

close walk
 
The \emph{distance} \index{distance} between two vertices $u,v$ in a graph is the number of edges
in a shortest path connecting them, denoted by $d(u,v)$ \index{$d(u,v)$}. The \emph{eccentricity}
$\epsilon$ of a vertex $v$ is the greatest distance between $v$ and any other vertex.
The \emph{radius} \index{radius} of a graph $G$, denoted by $rad(G)$ index{$rad(G)$}, is the minimum eccentricity
of any vertex. The \emph{diameter} \index{diameter} of a graph $G$, denoted by $diam(G)$ \index{$diam(G)$}, is the
maximum eccentricity of any vertex in the graph. That is, it is the greatest distance between any pair of vertices.


cycle

We often construct new graphs from old ones by deleting or adding some vertices and edges.
If $W\subset V_G$, then $G-W=G[V\\W]$ is the subgraph of $G$ obtained by deleting the vertices
in $W$ and all edges adjacent with them.

contraction
duplication
The \emph{chromatic number} $\chi$, of a graph $G$, is defined as the smallest $k$ such that $G$ admits a $k-$colouring.

\TODO{

A \emph{partitioning} $P$ of the vertices set $V_G$ is a division
of them into disjoint subsets: $P=(V_1,\cdots ,V_k)$. The
\emph{quotient graph} induced by the partitioning, written $G/P$,
is the graph $\tilde{G}=(\tilde{V},\tilde{E})$ is defined by
shrinking each part into a single node, i.e.

$ \tilde{V}= \{V_1,\cdots,V_k\}$ and

$ (V_i,V_j)\in \tilde{E} $ if and only if $ i\neq j \text{ and } \exists v \in V_i, w\in V_j\ (v,w) \in E.$}

\subsection{Basic concept in other fields}

The \emph{(binary) relation} $R$ is defined as a subset of $V_G
\times V_H$: $x\in V_G$ and $u\in V_H$ has a relation if and only if
$(x,u) \in R$. The \emph{transitive relation} $R^T$ of $R$ is a subset of $V_H \times V_G$. $g\in V_G$ and $h\in V_H$,
$(h,g) \in R^T$ if and only if $(g,h) \in R$.

A \emph{monoid} is a set, $S$, together with a binary operation $“\circ”$ that satisfies the following three axioms:





==> Introduction/introduction_temp.tex <==
%%% Thesis Introduction --------------------------------------------------
\chapter{Introduction}
\ifpdf
    \graphicspath{{Introduction/IntroductionFigs/PNG/}{Introduction/IntroductionFigs/PDF/}{Introduction/IntroductionFigs/}}
\else
    \graphicspath{{Introduction/IntroductionFigs/EPS/}{Introduction/IntroductionFigs/}}
\fi



%%% ----------------------------------------------------------------------


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 

%\markboth{\MakeUppercase{\thechapter. Introduction}}{\thechapter. Introduction}


The subject of this thesis---graph relations and constrained homomorphism orders---belongs to the field of discrete mathematics, more specifically to graph theory. It has a close relationship to several other fields of mathematics stemming from algebra and mathematical structures via category theory and logic to computer science disciplines such as  computational complexity.

The term `graph' was introduced by Sylvester in 1878~\cite{Sylvester1878}.
A {\em directed graph}\index{directed graph} $G$ is a pair $G=(V_G,E_G)$ such that $E_G$ is a subset of $V_G\times V_G$. We denote by $V_G$ {\em the set of vertices of $G$}\index{set of vertices} and by $E_G$ {\em the set of edges of $G$}\index{set of edges}. The class of all finite directed graphs is denoted by $\DiGraphs$.
An {\em undirected graph} (or simply a {\em graph}\index{graph}) $G$ is a directed graph such that $(u,v)\in E_G$ if and only if $(v,u)\in E_G$. We thus consider undirected graphs to be a special case of directed graphs. Unless explicitly stated otherwise we allow loops on vertices. The class of all finite undirected graphs is denoted by $\Graphs$.

Graphs are frequently employed to model natural or artificial systems.  
Let us begin the introduction with two examples taken from the real world.

In social science we can use social networks to express the relationships between individuals, groups and organizations. For example, a friendship network shows the friendship relation among individuals in a community. At the same time, travelling is an important activity in modern society as people travel frequently, for business or for pleasure. If we consider all the places that people in a certain community have ever visited, we can define a network on places in the following natural way. 
Draw an edge between place $A$ and place $B$ if and only if we can find two people who are friends, one who has visited $A$, and the other $B$.
In this way we build a new network on places generated by the friendship network and the information about people and the places they visited. 


The research presented in this thesis was originally motivated by a generalization of concepts from bioinformatics. Consider protein-protein interaction networks (PPIs) in biology. Proteins contain domains that determine their function. Information on the domain content of proteins, which can be seen as a relation
$R\subseteq D\times P$ between domains and the proteins which contain them is readily available from biological databases. Candidates for interaction between domains can be derived from knowledge about the interacting proteins, i.e., a graph $G$ with vertex set $P$, and the relation $R$: If $(p,p')\in E_G$,
 $(d,p)\in R$, and $(d',p')\in R$, then the domains 
$(d,d')$ are putative interaction partners. 

In both examples, we use a network and a relation to create a new network. %The original network and that which is built upon it by using a relation are thus connected to one another. 
Conversely, given two networks, can we determine some meaningful relation between them? This is the idea behind the graph relations. 

More abstractly, let $G=(V_G,E_G)$ be a graph, $B$ a finite set, and
$R\subseteq V_G\times B$ a binary relation such that for every $b\in B$ there is $v \in V_G$ such that $(v,b)\in R$. Then
the graph $G\muls R$ has vertex set $B$ and edge set
\begin{equation*}
E_{G\muls R} = \left\{ (a,b)\in B\times B \mid \textrm{ there is }
      (u,v)\in E_G \textrm{ such that } (u,a),(v,b)\in R \right\}.
\end{equation*}
If there exists an $R$ satisfying the equation $G\muls R = H$, we say
there is a \emph{relation} from $G$ to $H$. The graphs $G$ and $H$
can be seen to be conjugates, i.e., $E_G=R^+\circ E_H\circ R$, where $R^+\subseteq B\times V_G$ is the transpose of the relation $R$ and $\circ$ denotes the composition of binary relations. % ($E_H\subseteq V_H\times V_H$ a binary relation). 
The \emph{composition} of binary relations $S\subseteq X\times Y$ and $T\subseteq Y\times Z$ is defined to be the relation $S\circ T=\{(x,z)\in X\times Z\mid  \textrm{ there is } y\in Y \textrm{ such that } (x,y)\in S \textrm{ and } (y,z)\in T\}$.


The concept of a relation between graphs turns out be closely related to the well-studied graph theory 
notion of a graph homomorphism.  For given graphs $G=(V_G,E_G)$ and
$H=(V_H,E_H)$, a \emph{homomorphism}\index{homomorphism} $f:G\to H$ is a mapping $f:V_G\to
V_H$ such that $(u,v)\in E_G$ implies $(f(u),f(v))\in E_H$. If there is no homomorphism from $G$ to $H$, we write $G\nrightarrow H$\index{$G\nrightarrow H$}. 
Graph homomorphisms have been studied ever since the 1960s, originally as a generalization of graph colourings, with pioneering work by G.\ Sabidussi~\cite{Sabidussi1961},  Z.\ Hedrl\' in and A.\ Pultr~\cite{Hedrlin1964} subsequently seeing rapid development by P.\ Hell and J.\ Ne\v{s}et\v{r}il~\cite{Hell2004}. There is a lot of intensive research going on  around this topic; for an extensive review of the subject, see~\cite{Hell2004}.

A homomorphism from a graph $G$ to a graph $H$ naturally defines a mapping $f^{1}:E_G\to E_H$ by setting
$f^{1}((u,v))=(f(u),f(v))$ for all $(u,v)\in E_G$. If both $f$ and $f^1$
are surjective, we call $f$ a \emph{surjective homomorphism}\index{surjective homomorphism}. Note that all
surjective homomorphisms $f:G\to H$ are (modulo representation) also
relations $G\muls R=H$, where $R=\{(u,f(u)) \mid u\in V_G\}$.

Obviously, relations that are not functional are not homomorphisms, but
correspond to multihomomorphisms, which in a sense are multifunctions. A \emph{multifunction} from a non-empty set $X$ to a non-empty set $Y$ is a function from $X$ to $P(Y)\setminus \emptyset$ where $P(Y)$ is the power set of $Y$~\cite{Nenthein2012}. Multifunctions between two topological spaces have been studied since 1960s~\cite{Whyburn1965}. Multifunctions were first studied in an algebraic sense in~\cite{Triphop2008}, in which they  feature as multihomomorphisms from one group to another group. To the best of our knowledge, multihomomorphisms between graphs first appeared as building blocks of Hom-complexes, introduced by Lov{\'a}sz, and are related to recent exciting developments in topological combinatorics~\cite{Matousek2003}, in particular to deep results involved in a proof of the Lov{\'a}sz hypothesis~\cite{Babson2006}.

A relation with full domain thus can be regarded as a \textit{surjective multihomomorphism}, a multihomomorphism such that the pre-image of every vertex in $H$ is non-empty and for every edge $(x,y)$ in $H$ we can find an edge $(u,v)$ in $G$ satisfying $x\in f(u)$, $y\in f(v)$.

It appears that surjective multihomomorphisms between groups were first defined in~\cite{Triphop2008} and studied in~\cite{Nenthein2012}. However, surjective multihomomorphisms between graphs have not yet received attention.


The study of relations, just as for the study of homomorphisms, involves investigating properties of general structures restricted to graphs.
Surprisingly, we find that whereas the notion of a graph homomorphism originated in the other fields of mathematics, the notion of a constrained homomorphism arose instead from applied disciplines such as social science and electronics.

\mbox{}

We widen the scope of our study to investigate the properties of \emph{constrained homomorphisms}, i.e., homomorphisms that satisfy further conditions such as surjectivity.
Partial orders induced by the existence of constrained homomorphisms and their properties form the second topic of this thesis. In particular we consider the following:

\begin{enumerate}
\item A homomorphism $f:G\to H$ is a {\em monomorphism}\index{monomorphism}\footnote{The name `monomorphism' originates from category theory.}, (also called \emph{injective homomorphism}\index{injective homomorphism}~\cite{Hell2004} or {\em \MonoHomo}) if it is injective.
\item A homomorphism $f:G\to H$ is a {\em full homomorphism}, or {\em \FullHomo}, if $(f(u),f(v))\in E_H$ implies $(u,v)\in E_G$.
\item A homomorphism $f:G\to H$ is an {\em embedding}, or {\em \EmbedHomo} if it is both a monomorphism and a full homomorphism.
\end{enumerate}


For undirected graphs we also consider the following forms of locally constrained homomorphisms.
\begin{enumerate}
\item A homomorphism $f:G\to H$ is a {\em locally injective homomorphism}, or {\em \LocInHomo}, if the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is injective.
\item A homomorphism $f:G\to H$ is a {\em locally surjective homomorphism}, or {\em \LocSurHomo}, if the restriction of the mapping $f$ to the domain $N_G(v)$ and range $N_H(f(v))$ is surjective.
\item A homomorphism $f:G\to H$ is a {\em locally bijective homomorphism}, or {\em \LocBiHomo}, if it is both a locally surjective and locally bijective homomorphism, that is, if the restriction to the neighbourhood of a vertex is a bijection.
\end{enumerate}


There are also other types of constrained homomorphism that have been studied. One example is that of a compaction~\cite{Kedem1984}.
A \emph{compaction} of a graph $G$ to a graph $H$ is a homomorphism $f:G\to H$ such that for every vertex $x$ of $H$, there exists a vertex $v$ of $G$ with $f(v)=x$, and for every edge $(x,y)$ of $H$, $x\neq y$, there exists an edge $(u,v)$ of $G$ with $f(u)=x$ and $f(v)=y$. The computational complexity of compaction has been studied by Vikas~\cite{Vikas2002,Vikas2004}.

Constrained homomorphisms have been intensively studied in their structural and algorithmic aspects as well as in their applications. 
Each type of constrained homomorphism has its own history. For example, globally constrained homomorphisms have also been studied from the 1960s. The earliest literature we can find is what Hedetniemi published in 1966~\cite{Hedetniemi1966}. It is however surprising to learn from the survey paper~\cite{Fiala2008} that the notion of a locally bijective homomorphism was already well established in combinatorial topology as early as 1932~\cite{Reidemeister1932}.
The other types of locally constrained homomorphism received attention much later. Locally surjective homomorphisms were introduced by Everett and Borgatti in 1991~\cite{Everett1991} and locally injective homomorphisms by Ne\v set\v ril in 1971~\cite{Nesetril1971}.


There are many results that link graphs and orders, such as those concerning vertex-edge-face partial orders~\cite{Brightwell1997}, planar graphs, hypergraph colourings~\cite{Duffus1991}, and on-line algorithms~\cite{Kierstead1981}.
In a similar vein, the dimension of a partial order is analogous to the chromatic number of a graph~\cite{Kelly1982}.
See the survey paper~\cite{Trotter1996} by Trotter. We give another instance of partial orders on graphs.

For any fixed type of finite relational structure, homomorphisms induce an ordering of the set of all structures. In particular, given two (directed) graphs $G$ and $H$, we write $G\leq H$, or $G\to H$, if there is a homomorphism from $G$ to $H$. The relation $\leq$ is a quasi-order and so it induces an equivalence relation. 
For two (directed) graphs $G$ and $H$ such that $G\Hom H$ and $H\Hom G$, we write $G\Homeq H$ and say that {\em $G$ and $H$ are homomorphically equivalent}. The homomorphism orders $(\Graphs,\leq)$ and $(\DiGraphs,\leq)$ are the partially ordered sets of all equivalence classes of finite undirected and directed graphs, respectively, ordered by the relation $\leq$. We will often abuse notation by replacing the classes that comprise $\Graphs$ and $\DiGraphs$ by their members.

These orders are of particular interest. For example, each of the two orders forms a distributive lattice, with the disjoint union of graphs being the supremum and the categorical product being the infimum.

The homomorphism order has been a fruitful research topic for several decades.
One of the well studied properties of the homomorphism order is density. Both $\Graphs$ and $\DiGraphs$ are dense, the former shown by Welzl~\cite{Welzl1982} and the latter by Ne\v set\v ril and Tardif~\cite{Nesetril2000}.

The other property which is extensively studied is universality. Any countable partial order is isomorphic to a suborder of $\DiGraphs$. This result first appeared in the context of categories in 1969~\cite{Pultr1980}. Antichains are sets of elements which are pairwise incomparable. A characterization of finite maximal antichains was given in~\cite{Nesetril1978}.

Maximal antichains are particularly relevant because of their relationship to the notion of a \emph{homomorphism duality}, introduced by Ne\v set\v ril and Pultr~\cite{Nesetril1978}. An ordered pair $(F,D)$ of graphs, or directed graphs, is a \emph{duality pair} if $\{G\mid F\to G\}=\{G\mid G\nrightarrow D\}$. Moreover, Ne\v set\v ril and Tardif obtain a correspondence between duality pairs and gaps in the homomorphism order~\cite{Nesetril2000a}.
 
\vspace{10pt}

This thesis consists of five chapters, including this introduction.

In Chapter 2 we describe notions that we require from graph theory and order theory.
In particular, we introduce basic graph-theoretic concepts and state their properties,
and define the main operations on graphs. We also give the fundamental properties of partial orders.  
Chapter 3 gives a brief overview of graph homomorphisms and constrained homomorphisms, i.e., monomorphisms, surjective homomorphisms, full homomorphisms and 
locally bijective, injective, surjective homomorphisms. Moreover, we introduce the new notion of graph relation, which is a new variant of homomorphism and can be seen as a generalized surjective homomorphism. We compare it to the other well-studied types of constrained graph homomorphism. We provide the necessary background on the theory of computational complexity in Appendix A.


Further properties of relations are introduced in Chapter 4.
We first show that every relation can be decomposed in a standard way into a surjective and an injective relation (Corollary~\ref{DeCo}). 
The equivalence classes of strong relational equivalence (Theorem~\ref{thm:equi}) and weak relational equivalence (Proposition~\ref{pro:iso}) are characterized. We then introduce the notion of R-cores, cores, reduced graphs and cocores. We show that core and reduced graph coincide, develop the characterization of cocore and R-core, and provide an effective algorithm to compute them. We also give a perhaps surprisingly simple characterization of those graphs $G$ for which all relations of $G$ to itself are automorphisms (Theorem~\ref{thm:auto1}). The computational complexity of testing for the existence of a relation between two graphs is briefly discussed. We describe the reduction of this problem to the corresponding problem for surjective homomorphisms. Finally, we briefly summarize the most important similarities and differences between weak and strong relational composition (Section~\ref{sect:weak}). Some of the results from this chapter have been published by J.~Hubi\v cka, J.~Jost, Y.~Long, P.~F.~Stadler, and L.~Yang in~\cite{Hubicka2012}. 


In Chapter 5 we review existing results on the homomorphism order and introduce the notion of constrained homomorphism orders. Moreover, after some discussion of universality, 
a new and significantly easier proof of universality of graph homomorphisms is given, which simplifies the proof given in~\cite{Hubicka2005}.
As a new result, we show that graph homomorphisms are universal even on the class of oriented cycles. The notions of future-finite-universal and past-finite-universal partial order are introduced for later use. We survey existing results on constrained homomorphism orders and provide several new results about cores, universality, gaps and dualities in the context of constrained homomorphisms. We derive properties of these partial orders and identify their similarities and differences. At the same time we give a simple condition for the existence of dualities in future-finite and past-finite partial orders. 
In the full homomorphism order we characterize the gaps and give a new and simple proof of the existence of left duals (simplifying results independently obtained by Feder and Hell~\cite{Feder2008} and Ball, Ne\v set\v ril, Pultr~\cite{Ball2007,Ball2010}).
For locally injective homomorphisms we prove universality on connected graphs
and give a partial characterization of gaps. We also prove the universality of all three kinds of locally constrained homomorphisms on graphs. We apply the characterization of PR-cores and FR-cores which are derived in Chapter 4 and carry over most results on the surjective homomorphism order. 
We prove that for every $d\geq 3$ the homomorphism order on the class of line graphs with maximum degree $d$ is universal.
Some of the results from this chapter have been submitted~\cite{Fiala2014} or are in preparation~\cite{Fiala2012}.





==> Introduction/left.tex <==

\subsection*{Basic concept in other fields}


The \emph{complement} \index{complement} $\overline{G}$ \index{$\overline{G}$} of simple graph $G$ is the graph on $V$
with edge set $[V]^2/E$.

The \emph{underlying graph} \index{underlying graph} $G_{sim}$ \index{$G_{sim}$} of multigraph $G$ is the
simple graph having the same vertex set $V_G$, and there is a edge
between two vertices in $G_{sim}$ if and only if there is at least
an edge between them in $G$.

A \emph{graph homomorphism} \index{graph homomorphism} $f$ from a graph $G = (V_G,E_G)$ to a
graph $H = (V_H,E_H)$, written $f:G \rightarrow H$ \index{$G \rightarrow H$}, is a mapping
$f:V_G \rightarrow V_H$ from the vertex set of $G$ to the vertex set
of $H$ such that $\{x,y\}\in E_G$ implies $\{f(x),f(y)\}\in E_H$.

An \emph{isomorphism} \index{isomorphism} of graphs $G$ and $H$ is a bijection between
the vertex sets of $G$ and $H$ $ f \colon V_G \to V_H \,\!$ such
that any two vertices $u$ and $v$ of $G$ are adjacent in $G$ if and
only if $f(u)$ and $f(v)$ are adjacent in $H$.





A graph $G$, if it holds the property that the neighborhood of any two vertices are not equal, i.e. $N(x)\neq N(y)$ for $\forall x,y\in G$
 we call the graph is \emph{thin graph} \index{thin graph}.



The \emph{chromatic number} \index{chromatic number} $\chi$ \index{$\chi$}, of a graph $G$, is defined as the smallest $k$ such that $G$ admits a $k$-colouring.

For simplicity, we say that a relation $R$ is an \emph{automorphism} \index{automorphism} of $G$
if it is of the form $R=\{(x,f(x))|x\in V_G\}$ and $f:V_G\to V_G$
is an automorphism of $G$.

Closure
For all $a, b$ in $S$, the result of the operation $a\circ b$ is also in $S$.
Associativity
For all $a, b$ and $c$ in $S$, the equation $(a\circ b) \circ c$ = $a \circ (b \circ c)$ holds.
Identity element
There exists an element $e$ in $S$, such that for all elements $a$ in $S$, the equation $e\circ a = a \circ e = a$ holds.


Denote vertex set by $V_G$ and edge set by $E_G$. We
allow multigraphs to have \emph{loops} \index{loops}, that are, the edges that
connect a vertex to itself.

As opposed to a multigraph, a \emph{simple graph} \index{simplge graph} is a undirected
graph with no loops and no more than one edge between different
vertices.

A \emph{pseudograph} \index{pseudograph} is a non-simple graph in which both graph loops and multiple edges are permitted.

A \emph{reflexive graph} \index{reflexive graph} is a pseudograph such that each vertex has an associated graph loop.



The \emph{(binary) relation} \index{binary relation} \index{relation} $R$ is defined as a subset of $V_G
\times V_H$: $x\in V_G$ and $u\in V_H$ has a relation if and only if
$(x,u) \in R$. The \emph{transitive relation} \index{transitive relation} $R^T$ \index{$R^T$} of $R$ is a subset of $V_H \times V_G$. $g\in V_G$ and $h\in V_H$,
$(h,g) \in R^T$ if and only if $(g,h) \in R$.

A \emph{monoid} \index{monoid} is a set, $S$, together with a binary operation $“\circ”$ that satisfies the following three axioms:

For relation $R\subseteq X\times Y$ we define by 
$R(x)=\{p\in Y|(x,p)\in R\}$ \index{$R(x)$} the \emph{image of $x$ under $R$} \index{image} and 
$R^{-1}(p)=\{x\in X|(x,p)\in R\}$ \index{$R^{-1}(p)$} the 
\emph{pre-image of $p$ under $R$} \index{pre-image}. 

==> Macros/MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 


==> dissdocuments/declarations.tex <==
\newpage
\begin{center}{\Large \bf Erkl\"arungen }\end{center}

\begin{itemize}
\item Ich erkenne die Promotionsordnung der Fakult\"at f\"ur Mathematik und Informatik der Universit\"at Leipzig vom 22.7.2009 in der Fassung der Ersten \"Anderungssatzung vom 4. Juli 2011 an. \vspace{0.2cm}

\item Die eingereichte Arbeit wurde nicht in gleicher oder \"ahnlicher Form einer anderen Pr\"ufungsbeh\"orde zum Zwecke einer Promotion oder eines anderen Pr\"ufungsverfahrens vorgelegt. \vspace{0.2cm}

\item Es haben keine fr\"uheren erfolglosen Promotionsversuche stattgefunden. 
\vspace{0.2cm}

\end{itemize}

\vspace*{1.5cm}
\begin{flushleft}
...............................................\\
(\me)
\end{flushleft}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "dissdocuments"
%%% End: 


==> dissdocuments/lettertodean.tex <==
\begin{flushleft}
\me        \hfill
\selectlanguage{german}
Leipzig, den \myformat\today \\
\mystreet\\ 
\mycity \\
Tel.: \mytel \\
Email: \myemail

\end{flushleft}
\vspace*{0.2cm}
\begin{flushleft}
An den\\
Dekan der Fakult\"at f\"ur\\ 
Mathematik und Informatik\\
Universit\"at Leipzig\\
\facultystreet\\ 
\facultycity
\end{flushleft}

{\bf Betreff: Durchf\"uhrung meines Promotionsverfahrens}\\

Sehr geehrter Herr Prof.\ Dr.\ \thedean,

hiermit m\"ochte ich die Durchf\"uhrung meines Promotionsverfahrens im Fachgebiet \department zur Erlangung des Doktorgrades Doctor rerum naturalium (Dr.\ rer.\ nat.) an der Fakult\"at f\"ur Mathematik und Informatik der Universit\"at Leipzig beantragen. \\[.2cm]
Die Anfertigung der Dissertation wurde von \mysupervisor\ betreut. \\

Mit freundlichen Gr\"u\ss en,
\vspace{2cm}

\me \\
 
{\bf Anlagen:} Dissertation (3 gebundene Exemplare), Zusammenfassung
der Dissertation (30 Exemplare), beglaubigte Kopie meiner Diplomurkunde,
tabellarischer Lebenslauf, Erkl\"arungen nach \textsection 6 1.5 der
Promotionsordnung, Verzeichnis der wissenschaftlichen Ver\"offentlichungen und Vortr\"age, Gutachtervorschl\"age.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "dissdocuments"
%%% End: 


==> dissdocuments/pubsandtalks.tex <==
\begin{center}
{\Large {\bf Ver\"offentlichungen und Vortr\"age}} \vspace{0.5cm}
\end{center}

{\large\bf Begutachtete Artikel}

\begin{itemize}
\item {\it Constrained Homomorphism Orders}, joint with J. Fiala, J. Hubi\v cka, extended abstract, Proceedings of Bordeaux Graph Workshop 2012.

\item {\it Relations between Graphs}, joint with J. Hubi\v cka, J. Jost, P. Stadler, L. Yang, Ars Mathematica Contemporanea, (2012), Volume 6, no. 2.

\item {\it The Correspondence between Zero-divisor Graphs with 6 Vertices and Their Semigroups}, joint with Y. Huang,
Journal of Algebra and its Applications.6 (2007), no. 2, 287--290. 13-04.

\end{itemize}

{\large\bf Eingereicht Artikel}


\begin{itemize}

\item {\it Universality of intervals of line graph order}, joint with J. Fiala, J. Hubi\v cka, submitted to European Journal of Combinatorics. ArXiv:1402.3736


\end{itemize}


{\large\bf Vortr\"age}



\begin{itemize}
\item {\it Relations between Graphs}, Bordeaux Graph Workshop, (Bordeaux, FR.), November 2012
\end{itemize}

\begin{itemize}

\item {\it Some interesting notions from Relations between Graphs}, Shanghai Conference on Algebraic Combinatorics, (Shanghai, CN.), August 2012

\end{itemize}

\begin{itemize}

\item {\it Relations between Graphs}, Workshop on Graph Theory and Combinatorics/Symposium for Young Combinatorists, National Sun Yat-sen University, (Kaohsiung, TW.), August 2012
\end{itemize}

\begin{itemize}
 \item{\it The Full Homomorphism and Surjective Homomorphism Orders}, (Leipzig, DE.), International Max Planck Research School Workshop, June 2012
\end{itemize}

\begin{itemize}

\item {\it Graph relations and graph homomorphisms}, Workshop on graph homomorphisms and related topics, (Nova Louka, CZ.), December 2011
\end{itemize}


\begin{itemize}

\item {\it Relations between Graphs}, Workshop on Algebraic Combinatorics, Shanghai Jiao Tong University, (Shanghai, CN.), September 2011
\end{itemize}


\begin{itemize}

\item {\it Relations between Complex Networks}, Complex System Summer School, Sante Fe Insitute, (Santa Fe, US.), June 2011
\end{itemize}

\begin{itemize}

\item {\it Graph relations, a concept from biology}, Autumn seminar Bioinformatics 2010, (Vysoka Lipa, CZ.), October 2010

\end{itemize}

%\cite{Englitz:2008p1,Tolnai:2008p1980,Tolnai:2008p713,Haustein:2008p1533}

%\bibliography{Literature/Papers}
%\bibliographystyle{apalike}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "DissDocuments"
%%% End: 

==> dissdocuments/reviewersuggestions.tex <==
\newpage
\begin{center}
{\Large \bf 
Gutachtervorschl"age}\vspace{0.5cm}
\end{center}

Folgende Personen w\"aren aufgrund ihrer fachlichen Kompetenz als Gutachter f\"ur diese Dissertation besonders geeignet:
\begin{itemize}
\item Prof.\ Dr.\ J\"urgen Jost\\
  Max-Planck-Institut f"ur Mathematik in den Naturwissenschaften\\
  Inselstr.\ 22-26\\
  D-04103 Leipzig\\
  email: jjost@mis.mpg.de\\
  Tel: 0341 9959 552\\
  Fax: 0314 9959 555\\

\item Prof.\ Dr.\ Peter F. Stadler\\
  Professur f\"ur Bioinformatik, Institut f\"ur Informatik\\
  Universit\"at Leipzig\\
  H\"artelstr.\ 16-18\\
  D-04107 Leipzig\\
  email: Peter.Stadler@bioinf.uni-leipzig.de\\
  Tel: +49 341 97-16690\\
  Fax: +49 341 97-16679\\

\item Prof.\ Dr.\ Pavol Hell\\ 
 School of Computing Science\\
 Simon Fraser University\\
 BURNABY, B.C., Canada V5A 1S6 \\
 email: pavol@sfu.ca\\
 Tel: +1 778-782-3391\\
 Fax: +1 778-782-3045\\

\item Prof.\ Dr.\ Wilfried Imrich\\
 Department Mathematics and Information Technology\\
 Montanuniversit{\"a}t Leoben\\
 Franz Josef-Stra\ss e 18\\
 8700 Leoben, Austria\\
 email: imrich@unileoben.ac.at\\
 Tel: +43 3842 402 1717\\
 Fax: +43 3842 402 1702\\

\item Prof.\ Dr.\ Jaroslav Ne{\v{s}}et{\v {r}}il\\
Department of Applied Mathematics\\
Charles University\\
Malostransk{\'e} n{\'a}m. 25\\
118 00 Praha 1, Czech Republic \\
email: nesetril@kam.mff.cuni.cz\\
Tel: +420 221 914 230\\
Fax: +420 257 531 014\\
\end{itemize}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "dissdocuments"
%%% End: 


==> dissdocuments/selbstaendig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Selbst\"andigkeitserkl\"arung
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\begin{center}
{\bf Selbstst\"andigkeitserkl\"arung}
\end{center}
Hiermit erkl\"are ich, die vorliegende Dissertation selbst\"andig und ohne
unzul\"assige fremde Hilfe angefertigt zu haben. Ich habe keine anderen
als die angef\"uhrten Quellen und Hilfsmittel benutzt und s\"amtliche 
Textstellen, die w\"ortlich oder sinngem\"a{\ss} aus ver\"offentlichten oder unver\"offentlichten Schriften entnommen wurden, und alle Angaben, die auf m\"undlichen Ausk\"unften beruhen, als solche kenntlich gemacht. 
Ebenfalls sind alle von anderen Personen bereitgestellten Materialien 
oder erbrachten Dienstleistungen als solche gekennzeichnet.\\
\\
\begin{flushleft}
\selectlanguage{german}
Leipzig, den \myformat\today 
\end{flushleft}
\vspace*{0.5cm}
\begin{flushleft}
$\ldots\ldots\ldots\ldots\ldots\ldots\ldots\ldots\ldots$\\
{\small(\me)}
\end{flushleft}

==> dissdocuments/shortcv.tex <==
\begin{flushleft}{\Large \bf Short CV} \\\rule{145mm}{0.2mm}\end{flushleft}

\begin{tabbing} \hspace*{4.5cm}\=\kill 

Name: \> Yangjing Long\\[0.5cm]

Date of birth: \> 08.07.1985 \\

\end{tabbing}

\vspace{-1cm}

\begin{tabbing} \hspace*{4.5cm}\=\kill 

09/2004 - 02/2008 \> Bachelor in Mathematics and Applied Mathematics\\
\> Shanghai Jiao Tong University (China) \\[0.5cm]

05/2008-10/2009 \> Graduate student at the Max Planck Institute \\
                 \>  for Mathematics in the Sciences (Germany)\\ [0.5cm]

since 11/2009 \> PhD student at the Max Planck Institute\\  
             \> for Mathematics in the Sciences (Germany)\\ 

\end{tabbing}


\hspace{3cm}


\begin{flushleft}{\Large \bf Daten zum Autor} \\\rule{145mm}{0.2mm}\end{flushleft}

\begin{tabbing} \hspace*{4.5cm}\=\kill 

Name: \> Yangjing Long\\[0.5cm]

Geburtsdatum: \> 08.07.1985  \\

\end{tabbing}

\vspace{-1cm}

\begin{tabbing} \hspace*{4.5cm}\=\kill 

09/2004 - 02/2008 \> Mathematikstudium\\
\> Universit\"at Shanghai Jiao Tong \\[0.5cm]

05/2008-10/2009 \> Studentin am Max-Planck-Institut f{\"u}r Matematik \\
\> in den Naturwissenschaften Leipzig\\ [0.5cm]

seit 11/2009 \> Doktorandin am Max-Planck-Institut f{\"u}r Matematik \\
\> in den Naturwissenschaften Leipzig\\ 

\end{tabbing}

